Homotopy (co)limits via homotopy (co)ends in general combinatorial model categories

We prove and explain several classical formulae for homotopy (co)limits in general (combinatorial) model categories which are not necessarily simplicially enriched. Importantly, we prove versions of the Bousfield-Kan formula and the fat totalization formula in this complete generality. We finish with a proof that homotopy-final functors preserve homotopy limits, again in complete generality.

==> _commands/_commands_1.tex <==
\makeatletter

%\input{_commands/objectmath/_objectmath_6008}

\input{_commands/automath/_automath_5022}

\input{_commands/basics/_basics_1}

\input{_commands/maps/maps_11}

\input{_commands/operators/operators_1}

\input{_commands/smalloperators/_smalloperators_1}

%Smaller versions of \otimes, \oplus, and \times, to be used in expressions concerning elements (a\sotimes b as apposed to A\otimes B)



\input{_commands/catlimits/_catlimits_3}


%\newcommand\comp{^{\scriptscriptstyle\bullet}}

%\newcommand\bicomp{^{\scriptscriptstyle\bullet\bullet}}


\input{_commands/arrows/_arrows_1}

\input{_commands/categories/_categories_2}

%\input{_commands/lie/_lie_1}

\input{_commands/abbreviations/_abbreviations_1}

\input{_commands/index/_index_1}

\input{_commands/page/_page_1}


\input{_commands/derivatives/_derivatives_1}



\input{_commands/slots/_slots_1}

\input{_commands/tuples/_tuples_2}

\input{_commands/delims/_delims_3}


\input{_commands/homology/_homology_1000}

\input{_commands/alg_geo/_alg_geo_1}


\input{_commands/intervals/_intervals_1}


\input{_commands/wraptext/_wraptext_1}
	

	
\input{_commands/widebar/_widebar_1}

%\makeatother

==> _commands/abbreviations/_abbreviations_1.tex <==
%Abbreviations:

\ExplSyntaxOn
\cs_new:Npn\newabbreviation#1#2#3{
	\cs_new:cpn { an#1 }{#2#3\xspace}
	\cs_new:cpn { An#1 }{\uppercase{#2}#3\xspace}
	\cs_new:cpn { an#1s }{#2#3s\xspace}
	\cs_new:cpn { An#1s }{\uppercase{#2}{#3}s\xspace}
}
\ExplSyntaxOff

\newabbreviation{hau}{H}{ausdorff}
\newabbreviation{rep}{r}{epresentation}
\newabbreviation{subrep}{s}{ubrepresentation}
\newabbreviation{irr}{i}{rreducible}
\newabbreviation{irrep}{i}{rreducible representation}
\newabbreviation{indec}{i}{ndecomposable}
\newabbreviation{coho}{c}{ohomology}
\newabbreviation{homal}{h}{omological}
\newabbreviation{homy}{h}{omology}
\newabbreviation{rhs}{r}{ight-hand side}
\newabbreviation{lhs}{l}{eft-hand side}
\newabbreviation{ses}{s}{hort exact sequence}
\newabbreviation{les}{l}{ong exact sequence}
\newabbreviation{cech}{\v{C}}{ech}

==> _commands/alg_geo/_alg_geo_1.tex <==
% for \reg etc, to be ed later.

%\input{_alg_geo/sheaf/sheaf_1}

\newmapclass{sheaf}[
	parent=map,
	%command=\mathscr,
	singlekeys={
		{sheafify} { upper={+} },
%		{*} { n=* },
		{dual}{upper=\vee},
	},
	keyvals={
		{stalk}{ci={\keyvalue}},
		%{res}{i=\vert\keyvalue},
		{twist}{symbolputright={(\keyvalue)}},
		{equivar}{upper={\keyvalue}},
	},
	output=alg,
]

%\newhomtype{Sheaf}[
%	singlekeys={
%		{sheafify} { upper={+} },
%		{*} { n=* },
%	},
%	keyvals={
%		{stalk}{ci={\inputvar}},
%		{res}{i=\vert\inputvar},
%	},
%]

%\newcotype

\newcommand\affineA{\mathbb{A}}
\newcommand\projectiveP{\mathbb{P}}
\newcommand\aff[2][]{
	\affineA^{\!\!#2}
	\ifblank{#1}
	{
		% do nothing
	}
	{
		_{#1}
	}
}
\newcommand\pspace[2][]{
	\projectiveP^{#2}
	\ifblank{#1}
	{
		% do nothing
	}
	{
		_{\!\!#1}
	}
}

\DeclareMathOperator\Specproto{Spec}

\newmap{\Spec}{\Specproto}
\let\spec=\Spec

\DeclareMathOperator\Projproto{Proj}

\newmap{\Proj}{\Projproto}
\let\proj=\Proj

%\let\sheaf=\mathscr

%\newcommand\shF{\sheaf{F}}
%\newcommand\shG{\sheaf{G}}
%\newcommand\shH{\sheaf{H}}
%\newcommand\shO{\sheaf{O}}
%\newcommand\shC{\sheaf{C}}
%\newcommand\shZ{\sheaf{Z}}
%\newcommand\shB{\sheaf{B}}

\newsheaf{\shF}{\mathscr{F}}
\newsheaf{\shG}{\mathscr{G}}
\newsheaf{\shH}{\mathscr{H}}
\newsheaf{\shO}{\mathscr{O}}
\newsheaf{\shC}{\mathscr{C}}
\newsheaf{\shZ}{\mathscr{Z}}
\newsheaf{\shB}{\mathscr{B}}

%\newcommand\reg[1]{ % regular functions
%	\shO
%	\ifblank{#1}
%	{
%		% do nothing
%	}
%	{
%		_{#1}
%	}
%}

%\newcommand\Reg{\shO} % regular functions without subscript

\newcommand\shhomsymbol{\mathscr{H\!\!{\scriptscriptstyle O\!\!\!M}}}


\newsheaf{\reg}{\mathscr{O}}

\newmap{\shhom}{\shhomsymbol}[parent=Hom,output=sheaf]


%\newoptcohomology\shhom{\shHom}
%\newhomologytheory{sh}{\shH}{\shC}{\shZ}{\shB}

%\newoptcohomology\sections{\Gamma}

==> _commands/arrows/_arrows_1.tex <==
\newcommand\isoto{\xrightarrow{ %isomorphism arrow
		\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}}}

\newcommand\medisoto{\xrightarrow{ %isomorphism arrow
		\,\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}\,}}

\newcommand\longisoto{\xrightarrow{ %isomorphism arrow
		\;\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}\;}}

\newcommand\isofrom{\xleftarrow{ %isomorphism arrow
		\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}}}

\newcommand\medisofrom{\xleftarrow{ %isomorphism arrow
		\,\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}\,}}

\newcommand\longisofrom{\xleftarrow{ %isomorphism arrow
		\;\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}\;}}
		


\providecommand*{\twoheadrightarrowfill@}{%
  \arrowfill@\relbar\relbar\twoheadrightarrow
}
\providecommand*{\twoheadleftarrowfill@}{%
  \arrowfill@\twoheadleftarrow\relbar\relbar
}
\providecommand*{\xtwoheadrightarrow}[2][]{%
  \ext@arrow 0579\twoheadrightarrowfill@{#1}{#2}%
}
\providecommand*{\xtwoheadleftarrow}[2][]{%
  \ext@arrow 5097\twoheadleftarrowfill@{#1}{#2}%
}


\newcommand\xto[1]{
	\xrightarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\xinto[1]{
	\xhookrightarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\xonto[1]{
	\xtwoheadrightarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\xfrom[1]{
	\xleftarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\xinfrom[1]{
	\xhookleftarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\xonfrom[1]{
	\xtwoheadleftarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\from{\leftarrow}
\newcommand\longto\longrightarrow
\newcommand\longfrom{\longleftarrow}

\newcommand{\hooklongrightarrow}{\lhook\joinrel\longrightarrow}
\newcommand{\twoheadlongrightarrow}{\relbar\joinrel\twoheadrightarrow}

\newcommand{\hooklongleftarrow}{\longleftarrow\joinrel\rhook}
\newcommand{\twoheadlongleftarrow}{\twoheadleftarrow\joinrel\relbar}

\newcommand\into{\hookrightarrow}
\newcommand\longinto{\hooklongrightarrow}

\newcommand\onto{\twoheadrightarrow}
\newcommand\longonto{\twoheadlongrightarrow}

\newcommand\infrom{\hookleftarrow}
\newcommand\longinfrom{\hooklongleftarrow}
\newcommand\onfrom{\twoheadleftarrow}
\newcommand\longonfrom{\twoheadlongleftarrow}

==> _commands/automath/_automath_5022.tex <==
\ExplSyntaxOn


\msg_new:nnnn { automath } { keyval_not_found } { Unknown~key~#1~passed~to~object~#2~on~input~line~\msg_line_number: } {}

\msg_new:nnnn { automath } { arg_keyval_not_found } { Unknown~argument~key~#1~passed~to~object~#2~on~input~line~\msg_line_number: } {}

\msg_new:nnnn { automath } { tl_not_found } { Unknown~data~#1~passed~to~object~#2~on~input~line~\msg_line_number: } {}
%IM should be changed so that this is passed to the actual object, not 
%IM the parent object, e.g., by having a third argument containing the
%IM actual object in \g_automath_tl_get:nn


\msg_new:nnnn { automath } { parent_not_found } { Unknown~class~#1~set~as~parent~of~object~#2~on~input~line~\msg_line_number: } {}

% Extra cs variants we need:

\cs_generate_variant:Nn \keyval_parse:NNn { cco }
\cs_generate_variant:Nn \tl_if_blank:nTF { vTF }

\tl_set:Nn \automath_bullet_tl {\raisebox{-0.25ex}{\scalebox{1.2}{$\cdot$}}}
\tl_set:Nn \automath_double_bullet_tl {\automath_bullet_tl\automath_bullet_tl}

%IM make a command \automathrender that is a frontend to _render:nn,
%IM accessible from non-expl3 settings
%IM Similarly, \newobject and \newclass
%IM Similarly, \automathifdotTF (tests if equal to .) and
%IM \automathifblankTF (??).

%IM allow things like | |_\infty and -^2, e.g. \var{slot}[g=2]
%IM this could for instance be accomplished by allowing passing
%IM options to the output class. In order for this to work,
%IM we need a new interface for output classes, e.g. \var[opt1]{sym}[opt2]
%IM
%IM Better: make two commands, \var and \varwithoptions{opt1}{sym}[opt2]

%IMplement notation \var[\big]

%IM output=self requires functions taking only one argument.

%IM new class type: flextuple or simply tuple

%IM allow setup of slots

%IM Currently, \Set has unwanted behaviour; running \Set without arguments produces { } rather than
%IM nothing. Probably, this is a bad implementation of \arg

%IM need \mathopen and \mathclose for non-scaled pars, and also a new implementation
%IM with ifpars=true|false and partype=(), for instance. Also allow dot, like, partype=.) or /.

% This package is supposed to allow a kind of object-oriented
% mathematics. All objects are created as instances of some
% specific CLASS, and hence classes must be created before objects.
%
% The fundamental form of all output made with this system is of the
% form
%		symbol ^ { upper index } _ { lower index } ( argument )
% (though in one of the types of classes, the argument is meant to be
% empty).
%
% There are (currently) three types of classes with slightly different
% input interfaces
%	* VARIABLES, simple commands that do not take argument, like
%	  x, y_0, X^*, etc.
%	  The standard syntax is
%	  \command[options]
%	* MAPS, function-like commands that do take arguments, like
%	  f(x), g_1'(x), Hom_A(x,y), End(Z), etc.
%	  The standard syntax is
%	  \command[options]{optional argument in braces}
%	* COHOMOLOGIES, function-like commands that take two arguments,
%	  an index and an argument in parentheses, like H^0(X),
%	  Z_0(X), etc.
%	  The standard syntax is
%	  \command[options]{mandatory index argument}{optional argument in braces}

%IMPLEMENT COMPLEXES
%IMPLEMENT changes to allow notation { ! } { ... } instead of {!} { ... }

%IM Maybe the difference between \map{f} and \var[arg=f,output=map] should be removed

% Consequently, there are three different "new class" commands.
% All three of them make heavy use of the command
% \g_automath_new_object:nn, to be defined below, which is the
% low-level command for creating new objects of any class.

% Whenever you create a new class, named ⟨myclass⟩, you will get
% two commands with names based on ⟨myclass⟩ (so make sure
% that these are free):
% 		* \new⟨myclass⟩, which creates a new instance of the
%		  class ⟨myclass⟩.
%		* \⟨myclass⟩, a command to create a quick instance of
%		  ⟨myclass⟩ on the go; it will take an extra initial argument
%		  corresponding to the symbol. So if it has, say, map type,
%		  you can write \⟨myclass⟩{f}[options]{x} to get a ⟨myclass⟩
%		  object with symbol f and argument x.

% The two first of these classes go through great lengths to implement
% a way to write primes the classical way, like \varx' for x',
% since I assume that this is a feature most classical TeX users will
% appreciate. The last class, cohomology, goes to equal lengths to allow notations like \co*{X} for the *'th cohomology of X




\DeclareDocumentCommand\newvariableclass{mO{}} % new variable-type class
{
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } { #2 }
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}t{'}t{'}}{
		% the actual \#1 command
		\IfBooleanTF{ ##3 }
		{
			\IfBooleanTF { ##4 }
			{ \automathrenderclass { #1 } { symbol = { ##1 }, ##2, prime, prime } }
			{ \automathrenderclass { #1 } { symbol = { ##1 }, ##2, prime } }
		}
		{	\automathrenderclass { #1 } { symbol = { ##1 }, ##2 }	}
	}
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmO{}t{'}t{'}}{
		\IfBooleanTF{ ##4 }
		{
			\IfBooleanTF { ##5 }
			{ \automathrenderclass { #1 } { symbol = { ##2 }, ##1, ##3, prime, prime } }
			{ \automathrenderclass { #1 } { symbol = { ##2 }, ##1, ##3, prime } }
		}
		{	\automathrenderclass { #1 } { symbol = { ##2 }, ##1, ##3 }	}
	}
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } ##1 { parent = #1, symbol = { ##2 }, ##3 }
		% create the object with name ##1
		\DeclareDocumentCommand{##1}{O{}t{'}t{'}}{
		% the actual \##1 command
			\IfBooleanTF{ ####2 }
			{
				\IfBooleanTF { ####3 }
				{ \automathrenderobject { ##1 } { ####1, prime, prime } }
				{ \automathrenderobject { ##1 } { ####1, prime } }
			}
			{	\automathrenderobject { ##1 } { ####1 }	}
		}
	}
}

%IM Consider using \automathIfNoValueOrDotTF on the argument

\DeclareDocumentCommand\newmapclass{mO{}} % new map-type class
{
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } { #2 }
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}t{'}t{'}G{}}{
		% the actual \#1 command
			\IfBooleanTF{ ##3 }
			{
				\IfBooleanTF { ##4 }
				{ \automathrenderclass { #1 } { symbol={##1}, ##2, prime, prime, arg={##5} } }
				{ \automathrenderclass { #1 } { symbol={##1}, ##2, prime,arg={##5} } }
			}
			{	\automathrenderclass { #1 } { symbol={##1}, ##2,arg={##5} }	}
	}
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmO{}t{'}t{'}G{}}{
			\IfBooleanTF{ ##4 }
			{
				\IfBooleanTF { ##5 }
				{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3, prime, prime, arg={##6} } }
				{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3, prime,arg={##6} } }
			}
			{	\automathrenderclass { #1 } { symbol={##2}, ##1, ##3,arg={##6} }	}
	}
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } ##1 { parent = #1, symbol = { ##2 }, ##3 }
		% creates the object with name ##1
		\DeclareDocumentCommand{##1}{O{}t{'}t{'}G{}}{
		% the actual \##1 command
			\IfBooleanTF{ ####2 }
			{
				\IfBooleanTF { ####3 }
				{ \automathrenderobject { ##1 } { ####1, prime,prime, arg={####4} } }
				{ \automathrenderobject { ##1 } { ####1, prime, arg={####4} }
				}
			}
			{	\automathrenderobject { ##1 } { ####1, arg={####4} }	}
		}
	}
}

\DeclareDocumentCommand\newcohomologyclass{mO{}} % new cohomology-type class
{
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } { #2 }
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}mG{}}{
		% the actual \#1 command
		\automathifeqTF { ##3 }{ * }
		{	\automathrenderclass { #1 } { symbol={##1}, ##2, *, arg={##4} }	}
		{
			\automathifeqTF { ##3 }{ ** }
			{	\automathrenderclass { #1 } { symbol={##1}, ##2, **, arg={##4} }	}
			{
				\automathifblankordotTF { ##3 }
				{ \automathrenderclass { #1 } { symbol={##1}, ##2, arg={##4} } }
				{ \automathrenderclass { #1 } { symbol={##1}, ##2, degreedefault={##3}, arg={##4} } }
			}
		}
	}
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmO{}mG{}}{
		\automathifeqTF { ##4 }{ * }
		{	\automathrenderclass { #1 } { symbol={##2}, ##1, ##3, *, arg={##5} }	}
		{
			\automathifeqTF { ##4 }{ ** }
			{	\automathrenderclass { #1 } { symbol={##2}, ##1, ##3, **, arg={##5} }	}
			{
				\automathifblankordotTF { ##4 }
				{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3, arg={##5} } }
				{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3, degreedefault={##4}, arg={##5} } }
			}
		}
	}
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } { ##1 }{ parent = #1, symbol = { ##2 }, ##3 }
		% creates the object with name ##1
		\DeclareDocumentCommand{##1}{O{}mG{}}{
			% the actual \##1 command
			\automathifeqTF { ####2 } { * }
			{	\automathrenderobject { ##1 } {  ####1, *, arg={ ####3 } }	}
			{
				\automathifeqTF { ####2 } { ** }
				{	\automathrenderobject { ##1 } {  ####1, **, arg={ ####3 } }	}
				{
					\automathifblankordotTF { ####2 }
					{ \automathrenderobject { ##1 } {  ####1, arg={ ####3 } } }
					{ \automathrenderobject { ##1 } {  ####1, degreedefault={ ####2 }, arg={ ####3 } } }
				}
			}
		}
	}
}

\DeclareDocumentCommand\newcomplexclass{mO{}} % new cohomology-type class
{
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } { #2 }
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}g}{
		% the actual \#1 command
		\automathifeqTF { ##3 }{ * }
		{	\automathrenderclass { #1 } { symbol={##1}, ##2, * }	}
		{
			\automathifeqTF { ##3 }{ ** }
			{	\automathrenderclass { #1 } { symbol={##1}, ##2, ** }	}
			{
				\IfValueTF { ##3 }
				{
					\automathifblankordotTF { ##3 }
					{ \automathrenderclass { #1 } { symbol={##1}, ##2 } }
					{ \automathrenderclass { #1 } { symbol={##1}, ##2, degreedefault={##3} } }
				}
				{
					\automathrenderclass { #1 } { symbol={##1}, ##2 }
				}
			}
		}
	}
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmO{}g}{
		\automathifeqTF { ##4 }{ * }
		{	\automathrenderclass { #1 } { symbol={##2}, ##1, ##3, * }	}
		{
			\automathifeqTF { ##4 }{ ** }
			{	\automathrenderclass { #1 } { symbol={##2}, ##1, ##3, ** }	}
			{
				\IfValueTF { ##4 }
				{
					\automathifblankordotTF { ##4 }
					{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3 } }
					{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3, degreedefault={##4} } }
				}
				{
					\automathrenderclass { #1 } { symbol={##2}, ##1, ##3 }
				}
			}
		}
	}
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } { ##1 }{ parent = #1, symbol = { ##2 }, ##3 }
		% creates the object with name ##1
		\DeclareDocumentCommand{##1}{O{}g}{%
			% the actual \##1 command
			\automathifeqTF { ####2 } { * }
			{	\automathrenderobject { ##1 } {  ####1, * }	}
			{
				\automathifeqTF { ####2 } { ** }
				{	\automathrenderobject { ##1 } {  ####1, ** }	}
				{
					\IfValueTF { ####2 }
					{
						\automathifblankordotTF { ####2 }
						{ \automathrenderobject { ##1 } {  ####1 } }
						{ \automathrenderobject { ##1 } {  ####1, degreedefault={ ####2 } } }
					}
					{
						\automathrenderobject { ##1 } {  ####1 }
					}
				}
			}
		}
	}
}

%
\DeclareDocumentCommand\newtupleclass{mO{}} % new tuple-type class
{
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } { #2 }
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}m}{
		% the actual \#1 command
		\automathrenderclass { #1 }{ symbol = { ##1 }, ##2, arg = { ##3 } }
	}
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmmO{}}{
		\automathrenderclass { #1 }{ symbol = { ##2 }, ##1, ##3, arg = { ##4 } }
	}
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmmmmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } { ##1 } % creates the object with name ##1
		{ parent = #1, leftpar = { ##2 }, argsep = { ##3 }, rightpar = { ##4 }, argdots = { ##5 }, ##6 }
		\DeclareDocumentCommand{##1}{O{}G{}}{
		% the actual \##1 command
			\IfNoValueTF { ####2 }
			{	\automathrenderobject { ##1 } { ####1 } }
			{	\automathrenderobject { ##1 } { ####1, arg = { ####2 } } }
		}
	}
}

\DeclareDocumentCommand\newdelimiterclass{mO{}} % new delimiter-type class
{
	%IM this needs updating: We need an option not to use the arg keyvals,
	%IM for right now, autopars do not work for \Set
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } {
		keyvals={
			{arg}{argwithoutkeyval=\keyvalue},
			%Currently, no braces around \keyvalue is necessary for \automathdelimsize to work
			% with par=auto
		},
		#2
	}
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}m}
	{ \automathrenderclass { #1 } { symbol = { ##1 }, ##2, arg = { ##3 } } }
	% the actual \#1 command
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmO{}m}
	{ \automathrenderclass { #1 } { symbol = { ##2 }, ##1, ##3, arg = { ##4 } } }
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } { ##1 }{ parent = #1, leftpar = { ##2 }, rightpar = { ##3 }, ##4 }
		% creates the object with name ##1
		\DeclareDocumentCommand{##1}{O{}G{}}{
		% the actual \##1 command
			\IfNoValueTF { ####2 }
			{	\automathrenderobject { ##1 } { ####1 }	}
			{	\automathrenderobject { ##1 } { ####1, arg = { { ####2 } } } }
		}
	}
}

\cs_generate_variant:Nn \tl_if_eq:nnTF { xnTF }

\cs_generate_variant:Nn \tl_if_eq:nnF { xnF }

\cs_generate_variant:Nn \tl_if_eq:nnT { xnT }

\DeclareDocumentCommand{\automathifblankordotTF}{mmm}
{
	\tl_if_blank:nTF { #1 }
	{	#2	}
	{
		\tl_if_eq:xnTF { \tl_trim_spaces:n { #1 } } { . } { #2 } { #3 }
	} 
}

\DeclareDocumentCommand{\automathifblankordotT}{mm}
{
	\tl_if_blank:nTF { #1 }
	{	#2	}
	{
		\tl_if_eq:xnT { \tl_trim_spaces:n { #1 } } { . } { #2 }
	} 
}

\DeclareDocumentCommand{\automathifblankordotF}{mm}
{
	\tl_if_blank:nF { #1 }
	{
		\tl_if_eq:xnF { \tl_trim_spaces:n { #1 } } { . } { #2 }
	} 
}

\cs_set_eq:NN\automathifeqTF\tl_if_eq:nnTF

\cs_set_eq:NN\automathifeqT\tl_if_eq:nnT

\cs_set_eq:NN\automathifeqF\tl_if_eq:nnF



\cs_new:Npn \g_automath_new_class:nn#1#2{
	% create a new class
	% #1 = name of class
	% #2 = standard keyval setup; the parent class by default is automathvariable
	\g_automath_new_object:nnn { automathvariable } { #1 } { #2 }
}


\cs_set_eq:NN\automathnewclass\g_automath_new_class:nn

\seq_new:N \automath_all_objects_seq


\seq_put_right:Nn \automath_all_objects_seq { automathvariable }



\cs_new:Npn \g_automath_new_object:nnn#1#2#3{ % create new object
	% #1 = class of command
	% #2 = name of command, without backslash
	% #3 = standard keyval setup

	\g_automath_tl_provide:nn { #2 } { parent }

	\tl_set:cn { g_automath_#2_parent } { automathvariable }


	\cs_set:cpn { g_automath_#2_keyval:nn } ##1##2 % command controlling keyvals
	{ \g_automath_keyval:nnnn { ##2 } { ##1 } { #1 } { #2 } }

	\cs_set:cpn { g_automath_#2_singlekey:n } ##1 % command controlling singlekeys
	{ \g_automath_singlekey:nnn { ##1 } { #1 } { #2 } }
	

	% Now a similar collection of keyval commands for the *argument*
	
	\cs_set:cpn { g_automath_#2_arg_keyval:nn } ##1##2
	{ \g_automath_arg_keyval:nnnn { ##2 } { ##1 } { #1 } { #2 } }
	
	\cs_set:cpn { g_automath_#2_arg_singlekey:n } ##1
	{ \g_automath_arg_singlekey:nnn { ##1 } { #1 } { #2 } }

	
	% initially sets up the keyval interface of the object
	\g_automath_keys_set:nn { #2 } { parent=#1, #3 }
	
	\seq_put_right:Nx \automath_all_objects_seq { #2 }
}




% Get-type commands:
%IM All of this data should have g_ removed and get _tl

\cs_new:Npn \g_automath_tl_get:nn#1#2% maybe should be PROTECTED??
{
	% #1 = name of object
	% #2 = the data to get
	%\exp_args:Nnno
	\tl_if_exist:cTF { g_automath_#1_#2 }%IM replace by check for if_provided
	%\bool_if_exist:cTF { g_automath_#1_#2_if_provided }
	{%
		%\bool_if:cTF { g_automath_#1_#2_if_provided }
		%{ \use:c { g_automath_#1_#2 } }
		%{ \g_automath_tl_get:nn{\g_automath_tl_get:nn{#1}{parent}}{#2} }
		\use:c { g_automath_#1_#2 }
	}%
	{%
		%\exp_args:No
		%\exp_args:No
		%\tl_if_eq:nnTF { #1 } { automathvariable }
		%{
			%\msg_error:nnnn { automath } { data_not_found } { #2 } { #1 }
		%}
		%{
			%\g_automath_tl_get:nn{\g_automath_tl_get:nn{#1}{parent}}{#2}%
			\g_automath_tl_get:cn { g_automath_#1_parent } { #2 }
		%}
	}%
}

\cs_new:Npn \g_automath_tl_get_exp_not:nn#1#2% maybe should be PROTECTED??
{
	% #1 = name of object
	% #2 = the data to get
	%\exp_args:Nnno
	\tl_if_exist:cTF { g_automath_#1_#2 }%IM replace by check for if_provided
	%\bool_if_exist:cTF { g_automath_#1_#2_if_provided }
	{%
		%\bool_if:cTF { g_automath_#1_#2_if_provided }
		%{ \use:c { g_automath_#1_#2 } }
		%{ \g_automath_tl_get:nn{\g_automath_tl_get:nn{#1}{parent}}{#2} }
		%\use:c { g_automath_#1_#2 }
		\exp_not:v { g_automath_#1_#2 }
		%\exp_not:n { \use:c { g_automath_#1_#2 } }
	}%
	{%
		%\exp_args:No
		%\exp_args:No
		%\tl_if_eq:nnTF { #1 } { automathvariable }
		%{
			%\msg_error:nnnn { automath } { data_not_found } { #2 } { #1 }
		%}
		%{
			%\g_automath_tl_get:nn{\g_automath_tl_get:nn{#1}{parent}}{#2}%
			\g_automath_tl_get:cn { g_automath_#1_parent } { #2 }
		%}
	}%
}

\cs_generate_variant:Nn \g_automath_tl_get:nn { cn }



\cs_new:Npn \g_automath_tl_get_store:nnN#1#2#3% maybe should be PROTECTED??
{
	% #1 = name of object
	% #2 = the data to get
	% #3 = where to store it
	%\exp_args:Nnno
	\tl_if_exist:cTF { g_automath_#1_#2 }%IM replace by check for if_provided
	{%
		%\use:c { g_automath_#1_#2 }%
		\tl_set_eq:Nc #3 { g_automath_#1_#2 }
		%\tl_set:Nn#3 { automathvariable }
	}%
	{%
		%\exp_args:No
		%\exp_args:No
%		\tl_if_eq:nnTF { #1 } { automathvariable }
%		{
%			\msg_error:nnnn { automath } { data_not_found } { #2 } { #1 }
%		}
%		{
			%\g_automath_tl_get_store:nnN{\g_automath_tl_get:nn{#1}{parent}}{#2}#3%
			\g_automath_tl_get_store:cnN { g_automath_#1_parent } { #2 } #3
%		}
	}%
}

\cs_generate_variant:Nn \g_automath_tl_get_store:nnN { cnN, nnc, cnc }

\cs_new:Npn\g_automath_tl_provide:nn#1#2
{
	%\tl_if_exist:cF { g_automath_#1_#2 } { \tl_new:c { g_automath_#1_#2 } }
	%\bool_if_exist:cF { g_automath_#1_#2_if_provided } { \bool_new:c { g_automath_#1_#2_if_provided } }
	%\bool_set_true:c { g_automath_#1_#2_if_provided }
	\tl_if_exist:cF { g_automath_#1_#2 } { \tl_set:cn { g_automath_#1_#2 } {} }
}

%\cs_new:Npn\g_automath_tl_unprovide:nn#1#2
%{
	%\tl_if_exist:cF { g_automath_#1_#2 } { \tl_new:c { g_automath_#1_#2 } }
	%\bool_if_exist:cF { g_automath_#1_#2_if_provided } { \bool_new:c { g_automath_#1_#2_if_provided } }
	%\bool_set_true:c { g_automath_#1_#2_if_provided }
%}

\cs_new:Npn\g_automath_tl_inherit:nn#1#2
{
	\tl_if_exist:cF { g_automath_#1_#2 }
	{
		\g_automath_tl_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
	}
	{
		\g_automath_tl_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
		%IM could be replaced by simply { #1 } { #2 } once the check is made
		%IM based on "if_provided"
	}
}

\cs_new:Npn\g_automath_tl_inherit_x:nn#1#2
{
	\tl_if_exist:cF { g_automath_#1_#2 }
	{
			\g_automath_tl_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
	}
	{
		\g_automath_tl_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
		%IM could be replaced by simply { #1 } { #2 } once the check is made
		%IM based on "if_provided"
	}
}




\cs_new:Npn \g_automath_seq_get_store:nnN#1#2#3{% maybe should be PROTECTED??
	% #1 = name of object
	% #2 = the sequence to get
	% #3 = the command to store it in
	%\seq_if_exist:cTF { g_automath_#1_#2 }%
	\bool_if_exist:cTF { g_automath_#1_#2_if_provided }
	{%
		%\seq_set_eq:Nc#3 { g_automath_#1_#2 }
		\bool_if:cTF { g_automath_#1_#2_if_provided }
		{ \seq_set_eq:Nc#3 { g_automath_#1_#2 } }
		{ \g_automath_seq_get_store:cnN{ g_automath_#1_parent }{#2}#3 }
	}%
	{%
		%\exp_args:No
		%\exp_args:No
		%\tl_if_eq:nnTF { #1 } { automathvariable }
		%{
		%	\msg_error:nnnn { automath } { data_not_found } { #2 } { #1 }
		%}
		%{
			\g_automath_seq_get_store:cnN{ g_automath_#1_parent }{#2}#3%
		%}
	}%
}

\cs_generate_variant:Nn \g_automath_seq_get_store:nnN { cnN, nnc, cnc }

\cs_new:Npn\g_automath_seq_inherit:nn#1#2
{
	\bool_if_exist:cTF { g_automath_#1_#2_if_provided }
	{
		\bool_if:cF { g_automath_#1_#2_if_provided }
		{
			\g_automath_seq_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
			\bool_set_true:c { g_automath_#1_#2_if_provided }
		}
	}
	{
		\bool_new:c { g_automath_#1_#2_if_provided }
		\bool_set_true:c { g_automath_#1_#2_if_provided }
		\seq_if_exist:cF { g_automath_#1_#2 } { \seq_new:c { g_automath_#1_#2 } }
		\g_automath_seq_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
	}
}





\cs_new:Npn \g_automath_prop_provide:nn#1#2
{
	% #1 = name of the object
	% #2 = name of the prop
	\prop_if_exist:cF { g_automath_#1_#2 } { \prop_new:c { g_automath_#1_#2 } }
}


\cs_new:Npn \g_automath_keyval_get:nnNTF#1#2#3#4#5{%
	% #1 = name of the object
	% #2 = keyval data to get
	% #3 = command to store possible data in
	% #4 = if true (not to be used)
	% #5 = if false
	\prop_get:cnNTF { g_automath_#1_custom_keyvals } { #2 }#3%\l_automath_keyval_get_temp
	{	#4	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{ #5 }
		{ \g_automath_keyval_get:vnNTF { g_automath_#1_parent } { #2 } #3 { #4 } { #5 } }
	}
}

\cs_generate_variant:Nn \g_automath_keyval_get:nnNTF { vnNTF }

\cs_new:Npn \g_automath_singlekey_get:nnNTF#1#2#3#4#5{%
	% #1 = name of the object
	% #2 = singlekey data to get
	% #3 = command to store possible data in
	% #4 = if true (not to be used)
	% #5 = if false
	\prop_get:cnNTF { g_automath_#1_custom_singlekeys } { #2 } #3
	{	#4	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{ #5 }
		{ \g_automath_singlekey_get:vnNTF { g_automath_#1_parent } { #2 } #3 { #4 } { #5 } }
	}
}

\cs_generate_variant:Nn \g_automath_singlekey_get:nnNTF { vnNTF }

%\cs_new:N\l_automath_arg_keyval_get_parent_temp

\cs_new:Npn \g_automath_arg_keyval_get:nnNTF#1#2#3#4#5{%
	% #1 = name of the object
	% #2 = keyval data to get
	% #3 = command to store possible data in
	% #4 = if true (not to be used)
	% #5 = if false
	\prop_get:cnNTF { g_automath_#1_custom_arg_keyvals } { #2 }#3%\l_automath_keyval_get_temp
	{	#4	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{ #5 }
		{ \g_automath_arg_keyval_get:vnNTF { g_automath_#1_parent } { #2 } #3 { #4 } { #5 } }
	}
}

\cs_generate_variant:Nn \g_automath_arg_keyval_get:nnNTF { vnNTF }

\prop_new:N\l_automath_arg_keyval_get_temp

\cs_new:Npn \g_automath_arg_singlekey_get:nnNTF#1#2#3#4#5{%
	% #1 = name of the object
	% #2 = singlekey data to get
	% #3 = command to store possible data in
	% #4 = if true (not to be used)
	% #5 = if false
	\prop_get:cnNTF { g_automath_#1_custom_arg_singlekeys } { #2 } #3
	{	#4	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{ #5 } { \g_automath_arg_singlekey_get:vnNTF { g_automath_#1_parent } { #2 } #3 { #4 } { #5 } }
	}
}

\cs_generate_variant:Nn \g_automath_arg_singlekey_get:nnNTF { vnNTF }

\cs_new:Npn\g_automath_bool_get:nnTF#1#2#3#4
{
	% #1 = name of the object
	% #2 = boolean to get
	% #3 = if true
	% #4 = if false
	\bool_if_exist:cTF { g_automath_#1_if_#2_if_provided }
	{
		\bool_if:cTF { g_automath_#1_if_#2_if_provided }
		{
			\bool_if:cTF { g_automath_#1_if_#2 } { #3 } { #4 }
		}
		{
			\tl_if_eq:nnTF { #1 } { automathvariable }
			{ #4 } { \g_automath_bool_get:vnTF { g_automath_#1_parent } { #2 } { #3 } { #4 } }
		}
	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{ #4 } { \g_automath_bool_get:vnTF { g_automath_#1_parent } { #2 } { #3 } { #4 } }
	}
}

\cs_generate_variant:Nn \g_automath_bool_get:nnTF { xnTF, cnTF, vnTF }

\cs_new:Npn\g_automath_bool_provide:nn#1#2
{
	% #1 = name of the object
	% #2 = boolean to provide
	\bool_if_exist:cTF { g_automath_#1_if_#2_if_provided }
	{
		\bool_if:cF { g_automath_#1_if_#2_if_provided }
		{	\bool_set_true:c { g_automath_#1_if_#2_if_provided }	}
	}
	{
		\bool_new:c { g_automath_#1_if_#2 }
		\bool_new:c { g_automath_#1_if_#2_if_provided }
		\bool_set_true:c { g_automath_#1_if_#2_if_provided }
	}
}

\cs_new:Npn\g_automath_cs_get:nnn#1#2#3
{
	% #1 = name of the object
	% #2 = command sequence to get
	% #3 = what to apply said sequence to
	\cs_if_exist:cTF { g_automath_#1_#2:n }
	{	\use:c { g_automath_#1_#2:n } { #3 }	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{
			% should probably throw an error by now, but later!
		}
		{
			\g_automath_cs_get:xnn { \g_automath_tl_get:nn{#1}{parent} } { #2 } { #3 }
		}
	}
}

\cs_generate_variant:Nn \g_automath_cs_get:nnn { xnn }


%\cs_set_eq:NN \automathnewobject \g_automath_new_object:nnn

\cs_generate_variant:Nn \g_automath_new_object:nnn { nxn }

\cs_set:Npn \automathnewobject#1#2#3
{	\g_automath_new_object:nxn { #1 }{ \cs_to_str:N #2 } { #3 }	}


%Now everything that has to do with creation of new objects


\cs_new:Npn \g_automath_keys_set:nn#1#2
{
	% #1 = object
	% #2 = keys
	\keyval_parse:cco %IM think about wthether o-type is really necessary.
	{ g_automath_#1_singlekey:n }
	{ g_automath_#1_keyval:nn }
	{ #2 }
}

\cs_new:Npn \g_automath_arg_keys_set:nn#1#2
{
	% #1 = object
	% #2 = keys
	\keyval_parse:cco %IM -||-
	{ g_automath_#1_arg_singlekey:n }
	{ g_automath_#1_arg_keyval:nn }
	{ #2 }
}

\DeclareDocumentCommand\setupclass{mm}{ % a user-level command for setting up the object
	% #1 = class
	% #2 = setup
	%\exp_args:Nx
	%\use:c { g_automath_#1_keys_set:n }
	\g_automath_keys_set:nn { #1 }{ #2 }
}

\DeclareDocumentCommand\setupobject{mm}{%
	% #1 = object
	% #2 = setup
	%\use:c { g_automath_\cs_to_str:N#1_keys_set:n }
	\g_automath_keys_set:nn { \cs_to_str:N #1 } { #2 }
}




\cs_new_protected:Npn \g_automath_render:nn#1#2
{
	%IM Render and return should be merged; return could be equivalent to the keys {render, clearstuff}
	%IM No reason to have the same code twice
	% the main command for rendering the command corresponding to the object #2 of class #1 with options #3
	\group_begin:
		%\use:c{ g_automath_#1_keys_set:n } { #2 } % set up the keyval interface
		\g_automath_keys_set:nn { #1 } { #2 }
		\tl_set:Nx\l__automath_symbol_temp { \g_automath_tl_get:nn { #1 } { symbol } } %IM chang to "store" solution
		%\g_automath_tl_get_store:nnN { #1 } { symbol } \l__automath_symbol_temp
		\g_automath_seq_get_store:nnN { #1 } { commands_sequence } \l__automath_commands_sequence_temp_seq
		%\seq_map_inline:cn { g_automath_#1_commands_sequence }
		\seq_map_inline:Nn\l__automath_commands_sequence_temp_seq
		{
			\tl_set:Nx \l__automath_symbol_temp
			{
				\exp_not:n { ##1 } { \exp_not:V \l__automath_symbol_temp }
			}
		}
		\tl_set:Nx\l__automath_render_temp
		{ % set a temporary command that contains the entire output
				%IM should test if symbol, index etc. are non-empty,
				%IM hen assign one by one. The same at return.
				\exp_not:V \l__automath_symbol_temp
%				% Setup indices:
				\exp_not:N\g_automath_upper_index:n
				{
					\g_automath_tl_get:nn { #1 } { upper_index }
				}
				\exp_not:N\g_automath_lower_index:n {
					\g_automath_tl_get:nn { #1 } { lower_index }
				}
		}%
		\g_automath_bool_get:nnTF { #1 } { par }
		{
			\tl_put_right:Nx \l__automath_render_temp
			{
				\exp_not:N
				\g_automath_parentheses:nnnn
				{ \g_automath_tl_get:nn { #1 } { par_size } }
				{ \g_automath_tl_get:nn { #1 } { par_open } }
				{ \g_automath_tl_get:nn { #1 } { par_close } }
				{ \g_automath_tl_get:nn { #1 }{ arg } } % apply argument command to argument
			}
		}
		{
			\tl_put_right:Nx \l__automath_render_temp
			{	\g_automath_tl_get:nn { #1 }{ arg }	}
		}
		\g_automath_bool_get:nnTF { #1 } { output } %IM p-q tests show that this does not work
		{
			\tl_set:Nx \l__automath_render_temp
			{
				\exp_not:c { \g_automath_tl_get:nn { #1 } { output }withoptions } { \g_automath_tl_get:nn { #1 } { output_options } } { \exp_not:V 
				\l__automath_render_temp }
			}
		}
		{
			% if false; do nothing
		}
	\exp_last_unbraced:NV
	\group_end:
	\l__automath_render_temp
}

\cs_set_eq:NN\automathrenderclass\g_automath_render:nn % a front-end command

\cs_set:Npn\automathrenderobject#1#2
{
	\g_automath_render:nn { \cs_to_str:N #1 } { #2 }
}




\cs_generate_variant:Nn \tl_put_right:cn { cf }

\cs_new:Npn\g_automath_primitive_singlekey_return:n#1
{
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\g_automath_seq_inherit:nn { #1 } { commands_sequence }
	\seq_map_inline:cn { g_automath_#1_commands_sequence }
	%IM must do the same as for the symbol, also to upper index etc.
		{
			\tl_set:cx { g_automath_#1_symbol }
			{
				\exp_not:n {\exp_not:N ##1}  { \exp_not:v { g_automath_#1_symbol } }
				%IM no idea why we needed and extra \exp_not:n
			}
		}
	\g_automath_tl_inherit_x:nn { #1 } { upper_index }
	\g_automath_tl_inherit_x:nn { #1 } { lower_index }
	\g_automath_tl_inherit_x:nn { #1 } { arg }
	%IMPLEMENT THIS!!!
	\tl_set:cx { g_automath_#1_symbol }
	{
		%\g_automath_tl_get:nn { #1 }{ symbol }
		\exp_not:v { g_automath_#1_symbol }
		% Setup indices:
		\exp_not:N\g_automath_upper_index:n
		{
			%\exp_not:f { \g_automath_tl_get:nn { #1 } { upper_index } }
			%IM for unknown reasons, :f did the trick here
			\exp_not:v { g_automath_#1_upper_index }
		}
		\exp_not:N\g_automath_lower_index:n {
			%\exp_not:v { g_automath_#1_lower_index }
			%\exp_not:f { \g_automath_tl_get:nn { #1 } { lower_index } }
			%\exp_not:x { \exp_not:n { \g_automath_tl_get:nn { #1 } { lower_index } }}
			%IM for unknown reasons, :f did the trick here
			\exp_not:v { g_automath_#1_lower_index }
		}
	}
	\g_automath_bool_get:nnTF { #1 } { par }
	{
		%\g_automath_tl_inherit:nn { #1 } { par_size }
		\g_automath_tl_get_store:nnN { #1 } { par_size } \l__automath_render_par_size_temp
		\tl_put_right:cn { g_automath_#1_symbol }
		{
			\exp_not:N
			\g_automath_parentheses:nnnn
		}
		\tl_put_right:cx { g_automath_#1_symbol }
		{
			%{ \exp_not:v { g_automath_#1_par_size } }
			{ \exp_not:V \l__automath_render_par_size_temp }
			{ \g_automath_tl_get:nn { #1 } { par_open } }
			{ \g_automath_tl_get:nn { #1 } { par_close } }
			{ \exp_not:v { g_automath_#1_arg } }
		}
	}
	{
		\tl_put_right:cx { g_automath_#1_symbol }
		{	\exp_not:v { g_automath_#1_arg }	}
	}
	\tl_clear:c { g_automath_#1_upper_index }
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\bool_set_true:c { g_automath_#1_if_first_upper }
	\tl_clear:c { g_automath_#1_lower_index }
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\bool_set_true:c { g_automath_#1_if_first_lower }
	\tl_clear:c { g_automath_#1_arg }
	\g_automath_bool_provide:nn { #1 } { first_arg }
	\bool_set_true:c { g_automath_#1_if_first_arg }
	\seq_clear:c { g_automath_#1_commands_sequence }
	%IM maybe one should enclose the new symbol in another group
	%IM should also reset stuff like par size
	%IM reset leftpar, rightpar, parsize etc. also
}


%Commands for rendering the argument:



\cs_new:Npn \g_automath_lower_index:n #1{
	% controls rendering of lower indices
	\tl_if_blank:nF { #1 } { \sb{#1} }
}




\cs_new:Npn \g_automath_upper_index:n #1{
	% controls rendering of upper indices
	\tl_if_blank:nF { #1 } { \sp{#1} }
}





\tl_new:N\automathdelimsize


%\cs_generate_variant:Nn \g_automath_parentheses:nnnn { vnnn, vvvn }

\cs_new:Npn \g_automath_parentheses:nnnn#1#2#3#4
{
	\tl_if_blank:nF { #4 }
	{
		\str_case:nnF { #1 }
		{
			{ normal } {
				\group_begin:
				\mathopen#2 #4 \mathclose#3
				\group_end:
			}
			{ auto } {
				\group_begin:
				\tl_set:Nn\automathdelimsize{\middle}
				\left#2 #4 \right#3
				\group_end:
			}
			{ * } {
				\group_begin:
				\tl_set:Nn\automathdelimsize{\middle}
				\left#2 #4 \right#3
				\group_end:
			}
%			{ \big } {
%				\group_begin:
%				\tl_set_eq:NN\automathdelimsize\big
%				\mathopen\big#2 #4 \mathclose\big#3
%				\group_end:
%			}
%			{ \Big } {
%				\group_begin:
%				\tl_set_eq:NN\automathdelimsize\Big
%				\mathopen\Big#2 #4 \mathclose\Big#3
%				\group_end:
%			}
%			{ \bigg } {
%				\group_begin:
%				\tl_set_eq:NN\automathdelimsize\bigg
%				\mathopen\bigg#2 #4 \mathclose\bigg#3
%				\group_end:
%			}
%			{ \Bigg } {
%				\group_begin:
%				\tl_set_eq:NN\automathdelimsize\Bigg
%				\mathopen\Bigg#2 #4 \mathclose\Bigg#3
%				\group_end:
%			}
		}
		{
			\group_begin:
			\tl_set_eq:NN\automathdelimsize#1
			\mathopen#1#2 #4 \mathclose#1#3
			\group_end:
		}
	}
}

\cs_new:Npn \g_automath_symbol_parentheses:nnnn#1#2#3#4
{
	\tl_if_blank:nF { #4 }
	{
		\str_case:nnF { #1 }
		{
			{ normal } { \mathopen#2 #4 \mathclose#3 }
			{ auto } { \left#2 #4 \right#3 }
			{ * } { \left#2 #4 \right#3 }
		}
		{ \mathopen#1#2 #4 \mathclose#1#3 }
	}
}


% Now for the commands that implement the keyval interface.
% These commands are used by the command \g_automath_#1_keys_set, see
% above.
% There is a fixed collection of primitive commands.
% Furthermore, the user has the option to create a collection
% of new commands, which are all stored in the token list
% called \g_automath_#1_custom_keyvals
% These keyvals contain code that must be executable by other keys
% (e.g., primitive ones)
% The key value is accessible to the user via the temporary command
% \keyvalue



\cs_new:Npn\g_automath_primitive_keyval_parent:nn#1#2{
	% Must inherit everything from the parent class
	%\tl_clear_new:c { g_automath_#1_parent }
	%\g_automath_tl_provide:nn { #1 } { parent }
	%IM This should always be declared, so no need for if_provided checks
	%IM This does not work, for unknown reasons:
%	\seq_if_in:NxTF \automath_all_objects_seq { #2 }
%	{	\tl_set:cn { g_automath_#1_parent } { #2 }	}
%	{ \msg_error:nnnn { automath } { parent_not_found } { #2 } { #1 } }
	%IM control if exists!
	\tl_set:cn { g_automath_#1_parent } { #2 }
}

\cs_new:Npn\g_automath_primitive_keyval_keyvals:nn#1#2{
	% Add new keyvals via the interface
	% keyvals={
	%	{key1}{do something with \keyvalue},
	%	{key2}{g=\keyvalue,i=\keyvalue},
	% }
	\g_automath_prop_provide:nn { #1 } { custom_keyvals }
	\clist_map_inline:nn { #2 }{
		\g_automath_keyval_equality_format:nnn{#1}##1
	}
}

\cs_new:Npn \g_automath_keyval_equality_format:nnn#1#2#3{
	%\prop_put:cnn { g_automath_#1_custom_keyvals }{#2}{#3}
	\prop_put:cnn { g_automath_#1_custom_keyvals }{#2}{#3}
	%IM Remove spaces in #2
}

\cs_new:Npn\g_automath_primitive_keyval_singlekeys:nn#1#2{
	% Add sinple keys, taking no values, via the
	% interface
	% singlekeys={
	%	{key1}{print something},
	%	{key2}{g=42,i=42},
	% }
	\g_automath_prop_provide:nn { #1 } { custom_singlekeys }
	\clist_map_inline:nn { #2 }{
		\g_automath_keyval_noequality_format:nnn{#1}##1
	}
}

\cs_new:Npn \g_automath_keyval_noequality_format:nnn#1#2#3{
	\prop_put:cnn { g_automath_#1_custom_singlekeys }{#2}{#3}
}

\cs_new:Npn\g_automath_primitive_keyval_argkeyvals:nn#1#2{
	% Add new keyvals via the interface
	% keyvals={
	%	{key1}{do something with \keyvalue},
	%	{key2}{g=\keyvalue,i=\keyvalue},
	% }
	\g_automath_prop_provide:nn { #1 } { custom_arg_keyvals }
	\clist_map_inline:nn { #2 }{
		\g_automath_arg_keyval_equality_format:nnn{#1}##1
	}
}

\cs_new:Npn \g_automath_arg_keyval_equality_format:nnn#1#2#3{
	\prop_put:cnn { g_automath_#1_custom_arg_keyvals }{#2}{#3}
}

\cs_new:Npn\g_automath_primitive_keyval_argsinglekeys:nn#1#2{
	% Add sinple keys, taking no values, via the
	% interface
	% singlekeys={
	%	{key1}{print something},
	%	{key2}{g=42,i=42},
	% }
	\g_automath_prop_provide:nn { #1 } { custom_arg_singlekeys }
	\clist_map_inline:nn { #2 }{
		\g_automath_arg_keyval_noequality_format:nnn{#1}##1
	}
}

\cs_new:Npn \g_automath_arg_keyval_noequality_format:nnn#1#2#3{
	\prop_put:cnn { g_automath_#1_custom_arg_singlekeys }{#2}{#3}
}

\cs_new:Npn\g_automath_primitive_keyval_symbol:nn#1#2{
	% Sets the value of the symbol
	%\tl_clear_new:c { g_automath_#1_symbol }
	%\g_automath_tl_provide:nn { #1 } { symbol }
	\g_automath_tl_provide:nn { #1 } { symbol }
	\tl_set:cn { g_automath_#1_symbol } { \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_symbol } { #2 }
}

\cs_new:Npn\g_automath_primitive_keyval_slot:nn#1#2{
	% Sets the value of the symbol
	%\tl_clear_new:c { g_automath_#1_symbol }
	%\g_automath_tl_provide:nn { #1 } { symbol }
	\g_automath_tl_provide:nn { #1 } { slot }
	\tl_set:cn { g_automath_#1_slot } { \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_symbol } { #2 }
}

\cs_new:Npn\g_automath_primitive_keyval_symbolputright:nn#1#2{
	% Sets the value of the symbol
%	\tl_if_exist:cTF { g_automath_#1_symbol }
%	{
%		% do nothing
%	}
%	{
%		\tl_set:cn { g_automath_#1_symbol } { \g_automath_tl_get:nn { \g_automath_tl_get:nn { #1 } { parent } } { symbol } }
%	}
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\tl_put_right:cn { g_automath_#1_symbol } { \exp_not:n { #2 } }
}

\cs_new:Npn\g_automath_primitive_keyval_symbolputleft:nn#1#2{
	% Sets the value of the symbol
%	\tl_if_exist:cTF { g_automath_#1_symbol }
%	{
%		% do nothing
%	}
%	{
%		\tl_set:cn { g_automath_#1_symbol } { \g_automath_tl_get:nn { \g_automath_tl_get:nn { #1 } { parent } } { symbol } }
%	}
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\tl_put_left:cn { g_automath_#1_symbol } { \exp_not:n { #2 } }
}

\cs_new:Npn\g_automath_primitive_keyval_command:nn#1#2{
	% Adds one entry on the left of the command
	% sequence to be applied to the symbol
%	\seq_if_exist:cTF { g_automath_#1_commands_sequence }
%	{
%		% do nothing
%	}
%	{
%		\seq_new:c { g_automath_#1_commands_sequence }
%%		%\seq_set_eq:c
%%		%IMplement this
%		\g_automath_seq_get_store:nnc { \g_automath_tl_get:nn { #1 } { parent } } { commands_sequence } { g_automath_#1_commands_sequence }
%	}
	\g_automath_seq_inherit:nn { #1 } { commands_sequence }
	%\seq_put_right:co { g_automath_#1_commands_sequence } { \exp_not:N #2 } %IM maybe \exp_not:n { #2 }?
	\seq_put_right:cn { g_automath_#1_commands_sequence } { #2 } %IM maybe \exp_not:n { #2 }?
	%\seq_put_right:co { g_automath_#1_commands_sequence } { \exp_not:n{\exp_not:N#2} } %IM maybe \exp_not:n { #2 }?
	%\seq_put_right:cn { g_automath_#1_commands_sequence } { \exp_not:N #2 } %IM maybe \exp_not:n { #2 }?
}

\cs_new:Npn\g_automath_primitive_keyval_argwithkeyval:nn#1#2{
	% Sets the argument (printed in parentheses
	% after the symbol)
	\g_automath_arg_keys_set:nn { #1 } {{{ #2 }}}
	%IM for unknown reasons, one needs these extra braces.
}

\cs_new:Npn\g_automath_primitive_keyval_argwithoutkeyval:nn#1#2{
%	\tl_if_exist:cTF { g_automath_#1_arg }
%	{
%		% do nothing
%	}
%	{
%		\tl_new:c { g_automath_#1_arg }
%		\tl_set:cx { g_automath_#1_arg }
%		{ \g_automath_tl_get:nn { \g_automath_tl_get:nn { #1 } { parent } } { arg } }
%		%IM change to :cn if we get a better if_first_arg system
%	}
	\g_automath_tl_provide:nn { #1 } { arg } %IM maybe replace by _x, as above
	%\bool_if:cTF { g_automath_if_first_arg }
	%\g_automath_bool_get:nnTF { #3 } { first_arg }
	\str_case:nnTF { #2 } { { * } { } { - } { } { slot } { } }
	{ \tl_put_right:cx { g_automath_#1_arg } { \exp_not:n { \g_automath_tl_get:nn { #1 } { slot } } } }
	{	\tl_put_right:cn { g_automath_#1_arg } { \exp_not:n { \exp_not:n{#2} } }	}
	%\tl_put_right:cx { g_automath_#1_arg } { #2 }
	%\tl_put_right:cx { g_automath_#1_arg } { \exp_not:n { #2 } }
	%\tl_put_right:cx { g_automath_#1_arg } { #2 }
	%IM :cx should probably be considered, too, at the place
	%IM where arguments are added via keyval.
	%IM THIS IS VERY WEIRD!!!
	\g_automath_primitive_keyval_ifoutput:nn { #1 } { true }
}


%				{ postcommand } {
%					% to be implemented; a command applied to the
%					% entire  
%				}


\cs_new:Npn\g_automath_primitive_keyval_argsep:nn#1#2
{
	%\tl_clear_new:c { g_automath_#1_argsep }
	\g_automath_tl_provide:nn { #1 } { argsep }
	\tl_set:cn { g_automath_#1_argsep } { \exp_not:n { #2 } }
}

\cs_new:Npn\g_automath_primitive_keyval_argdots:nn#1#2
{
	%\tl_clear_new:c { g_automath_#1_argdots }
	\g_automath_tl_provide:nn { #1 } { argdots }
	\tl_set:cn { g_automath_#1_argdots } { \exp_not:n { #2 } }
}


\cs_new:Npn\g_automath_primitive_keyval_output:nn#1#2
{
	% the class that the output of the command has
	%\g_automath_tl_provide:nn { #1 } { output }
	%IM Add this again!!!
	\tl_set:cn { g_automath_#1_output } { #2 }
	%IM check if defined, and also allow output=self for e.g.
	%IM derived functors. RHom should be same class as Hom
	%IM but R(sheaf hom) should be a sheaf.
}

\cs_new:Npn\g_automath_primitive_keyval_nowoutput:nn#1#2
{
	\g_automath_primitive_keyval_parent:nn { #1 } { #2 }
	\g_automath_primitive_keyval_output:nn { #1 } { #2 }
	\g_automath_primitive_keyval_ifoutput:nn { #1 } { true }
}

\cs_new:Npn\g_automath_primitive_keyval_outputoptions:nn#1#2{
	\g_automath_tl_provide:nn { #1 } { output_options }
	%\tl_put_right:cf { g_automath_#1_output_options } { \exp_not:n { #2 } }
	%\tl_put_right:cf { g_automath_#1_output_options } { #2 }
	\tl_put_right:cn { g_automath_#1_output_options } { #2 }
}
				
\cs_new:Npn\g_automath_primitive_keyval_ifoutput:nn#1#2{ %IMPLEMENT THIS
	% tells whether to use the output class or not
	\g_automath_bool_provide:nn { #1 } { output }
	\str_if_eq:nnTF { #2 } { true }
	{
		\bool_set_true:c { g_automath_#1_if_output }
	}
	{
		\str_if_eq:nnTF { #2 } { false }
		{	\bool_set_false:c { g_automath_#1_if_output }	}
		{
			%IM do nothing right now, but should
			%IM probably throw an error
		}
	}
}

\cs_new:Npn\g_automath_primitive_keyval_gradingpos:nn#1#2{
		% tells whether to use upper or lower indices
		\g_automath_bool_provide:nn { #1 } { upper_grading }
		\str_case:nnTF { #2 }
		{
			{ upper }
			{
				\bool_set_true:c { g_automath_#1_if_upper_grading }
			}
			{ lower }
			{
				\bool_set_false:c { g_automath_#1_if_upper_grading }
			}
		}
		{
			% do nohting
		}
		{
			% do nothing at the moment, but should probably throw an error
		}
}

\cs_set_eq:NN \g_automath_primitive_keyval_gradingposition:nn \g_automath_primitive_keyval_gradingpos:nn

\cs_new:Npn\g_automath_primitive_keyval_upper:nn#1#2{
	% adds to the upper index
	\g_automath_tl_inherit_x:nn { #1 } { upper_index }
%	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { #2 } }
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\bool_set_false:c { g_automath_#1_if_first_upper }
}



\cs_new:Npn\g_automath_primitive_keyval_supper:nn#1#2{
	% adds to the upper index
	\g_automath_tl_inherit_x:nn { #1 } { upper_index }
%	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_upper }
	{	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { #2 } }	}
	{
		\tl_put_right:cx { g_automath_#1_upper_index }
		{ \exp_not:n { \g_automath_tl_get:nn { #1 } { uppersep } } }
		\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\bool_set_false:c { g_automath_#1_if_first_upper }
}

\cs_new:Npn\g_automath_primitive_keyval_lower:nn#1#2{
	% adds to the lower index
	\g_automath_tl_inherit_x:nn { #1 } { lower_index }
%	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { #2 } }
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\bool_set_false:c { g_automath_#1_if_first_lower }
}

\cs_new:Npn\g_automath_primitive_keyval_slower:nn#1#2{
	% adds to the lower index
	\g_automath_tl_inherit_x:nn { #1 } { lower_index }
%	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_lower }
	{	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { #2 } }	}
	{
		\tl_put_right:cx { g_automath_#1_lower_index }
		{ \exp_not:n { \g_automath_tl_get:nn { #1 } { lowersep } } }
		\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\bool_set_false:c { g_automath_#1_if_first_lower }
}

\cs_generate_variant:Nn \tl_if_blank:nTF { cTF, vTF }

\cs_new:Npn \g_automath_primitive_upper_lower_auxiliary_first_arg:nn#1#2 { #1 }

\cs_new:Npn \g_automath_primitive_upper_lower_auxiliary_second_arg:nn#1#2 { #2 }

\cs_new:Npn\g_automath_primitive_keyval_uppersep:nn#1#2{
	% adds to the upper index
	\g_automath_tl_inherit_x:nn { #1 } { upper_index }
%	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_upper }
	{	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { \g_automath_primitive_upper_lower_auxiliary_second_arg:nn #2 } }	}
	{
		\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { \g_automath_primitive_upper_lower_auxiliary_first_arg:nn #2 \g_automath_primitive_upper_lower_auxiliary_second_arg:nn #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\bool_set_false:c { g_automath_#1_if_first_upper }
}


\cs_new:Npn\g_automath_primitive_keyval_lowersep:nn#1#2{
	% adds to the lower index
	\g_automath_tl_inherit_x:nn { #1 } { lower_index }
%	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_lower }
	{	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { \g_automath_primitive_upper_lower_auxiliary_second_arg:nn #2 } }	}
	{
		\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { \g_automath_primitive_upper_lower_auxiliary_first_arg:nn #2 \g_automath_primitive_upper_lower_auxiliary_second_arg:nn #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\bool_set_false:c { g_automath_#1_if_first_lower }
}

\cs_new:Npn\g_automath_primitive_keyval_cupper:nn#1#2{
	% adds to the upper index
	\g_automath_tl_inherit_x:nn { #1 } { upper_index }
%	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_upper }
	{	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { #2 } }	}
	{
		\tl_put_right:cn { g_automath_#1_upper_index } { , \exp_not:n { #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\bool_set_false:c { g_automath_#1_if_first_upper }
}


\cs_new:Npn\g_automath_primitive_keyval_clower:nn#1#2{
	% adds to the lower index
	\g_automath_tl_inherit_x:nn { #1 } { lower_index }
%	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_lower }
	{	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { #2 } }	}
	{
		\tl_put_right:cn { g_automath_#1_lower_index } { , \exp_not:n { #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\bool_set_false:c { g_automath_#1_if_first_lower }
}

\cs_new:Npn\g_automath_primitive_keyval_iffirstarg:nn#1#2
{
	\g_automath_bool_provide:nn { #1 } { first_arg }
	\tl_if_eq:nnTF { #2 } { true }
	{	\bool_set_true:c { g_automath_#1_if_first_arg }	}
	{
		\tl_if_eq:nnTF { #2 } { false }
		{	\bool_set_false:c { g_automath_#1_if_first_arg }	}
		{
			%IM Throw error later
		}
	}
}

\cs_new:Npn\g_automath_primitive_keyval_iffirstupper:nn#1#2
{
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\tl_if_eq:nnTF { #2 } { true }
	{	\bool_set_true:c { g_automath_#1_if_first_upper }	}
	{
		\tl_if_eq:nnTF { #2 } { false }
		{	\bool_set_false:c { g_automath_#1_if_first_upper }	}
		{
			%IM Throw error later
		}
	}
}

\cs_new:Npn\g_automath_primitive_keyval_iffirstlower:nn#1#2
{
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\tl_if_eq:nnTF { #2 } { true }
	{	\bool_set_true:c { g_automath_#1_if_first_lower }	}
	{
		\tl_if_eq:nnTF { #2 } { false }
		{	\bool_set_false:c { g_automath_#1_if_first_lower }	}
		{
			%IM Throw error later
		}
	}
}

\cs_new:Npn\g_automath_primitive_keyval_iffirstd:nn#1#2
{
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
	{ \g_automath_primitive_keyval_iffirstupper:nn { #1 } { #2 } }
	{ \g_automath_primitive_keyval_iffirstlower:nn { #1 } { #2 } }
}

\cs_set_eq:NN\g_automath_primitive_keyval_iffirstdeg:nn\g_automath_primitive_keyval_iffirstd:nn

\cs_set_eq:NN\g_automath_primitive_keyval_iffirstdegree:nn\g_automath_primitive_keyval_iffirstd:nn

\cs_new:Npn\g_automath_primitive_keyval_iffirsti:nn#1#2
{
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
	{ \g_automath_primitive_keyval_iffirstlower:nn { #1 } { #2 } }
	{ \g_automath_primitive_keyval_iffirstupper:nn { #1 } { #2 } }
}

\cs_set_eq:NN\g_automath_primitive_keyval_iffirstindex:nn\g_automath_primitive_keyval_iffirsti:nn

\cs_new:Npn\g_automath_primitive_keyval_setuppersep:nn#1#2
{
	\g_automath_tl_provide:nn { #1 } { uppersep }
	\tl_set:cn { g_automath_#1_uppersep } { \exp_not:n { #2 }}
}

\cs_new:Npn\g_automath_primitive_keyval_setlowersep:nn#1#2
{
	\g_automath_tl_provide:nn { #1 } { lowersep }
	\tl_set:cn { g_automath_#1_lowersep } { \exp_not:n { #2 }}
}

\cs_new:Npn\g_automath_primitive_keyval_d:nn#1#2
{
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_upper:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_lower:nn { #1 } { #2 }
	}
}

\cs_set_eq:NN\g_automath_primitive_keyval_deg:nn\g_automath_primitive_keyval_d:nn

\cs_set_eq:NN\g_automath_primitive_keyval_degree:nn\g_automath_primitive_keyval_d:nn

\cs_new:Npn\g_automath_primitive_keyval_sd:nn#1#2
{
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_supper:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_slower:nn { #1 } { #2 }
	}
}

\cs_set_eq:NN\g_automath_primitive_keyval_sdeg:nn\g_automath_primitive_keyval_sd:nn

\cs_set_eq:NN\g_automath_primitive_keyval_sdegree:nn\g_automath_primitive_keyval_sd:nn

\cs_new:Npn\g_automath_primitive_keyval_cd:nn#1#2{ %IM Maybe remove this.
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_cupper:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_clower:nn { #1 } { #2 }
	}
}




\cs_set_eq:NN\g_automath_primitive_keyval_cdeg:nn\g_automath_primitive_keyval_cd:nn

\cs_set_eq:NN\g_automath_primitive_keyval_cdegree:nn\g_automath_primitive_keyval_cd:nn


\cs_new:Npn\g_automath_primitive_keyval_i:nn#1#2{
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_lower:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_upper:nn { #1 } { #2 }
	}
}

\cs_set_eq:NN\g_automath_primitive_keyval_index:nn\g_automath_primitive_keyval_i:nn

\cs_new:Npn\g_automath_primitive_keyval_si:nn#1#2{
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_slower:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_supper:nn { #1 } { #2 }
	}
}

\cs_set_eq:NN\g_automath_primitive_keyval_sindex:nn\g_automath_primitive_keyval_si:nn

\cs_new:Npn\g_automath_primitive_keyval_ci:nn#1#2{
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_clower:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_cupper:nn { #1 } { #2 }
	}
}

\cs_set_eq:NN\g_automath_primitive_keyval_cindex:nn\g_automath_primitive_keyval_ci:nn


\cs_new:Npn\g_automath_primitive_keyval_par:nn#1#2{
	% sets the size of the parentheses
	\tl_set:cn { g_automath_#1_par_size }{ \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_par_size } { \exp_not:N #2 }
	\g_automath_primitive_keyval_ifpar:nn { #1 } { true }
}

\cs_new:Npn\g_automath_primitive_keyval_parsize:nn#1#2{
	% sets the size of the parentheses
	\tl_set:cn { g_automath_#1_par_size }{ \exp_not:n { #2 } }
}

\cs_new:Npn\g_automath_primitive_keyval_leftpar:nn#1#2{
	\tl_set:cn { g_automath_#1_par_open }{ \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_par_open }{ #2 }
	%\tl_set:cx { g_automath_#1_par_open }{ \exp_not:n { \exp_not:n { #2 } } }
	%\tl_set:cx { g_automath_#1_par_open }{ \exp_not:N #2 }
	%\tl_set:cn { g_automath_#1_par_open }{ \exp_not:n{\noexpand#2} }
}

\cs_new:Npn\g_automath_primitive_keyval_rightpar:nn#1#2{
	\tl_set:cn { g_automath_#1_par_close }{ \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_par_close}{ #2 }
	%\tl_set:cn { g_automath_#1_par_close }{ \exp_not:N #2 }
	%\tl_set:cn { g_automath_#1_par_close }{ \exp_not:n{\noexpand#2} }
}

\cs_new:Npn\g_automath_primitive_keyval_ifpar:nn#1#2{ %IMPLEMENT THIS
	% tells whether to use the output class or not
	\g_automath_bool_provide:nn { #1 } { par }
	\str_if_eq:nnTF { #2 } { true }
	{
		\bool_set_true:c { g_automath_#1_if_par }
	}
	{
		\str_if_eq:nnTF { #2 } { false }
		{	\bool_set_false:c { g_automath_#1_if_par }	}
		{
			%IM do nothing right now, but should
			%IM probably throw an error
		}
	}
}



\cs_new:Npn\g_automath_primitive_keyval_spar:nn#1#2
{
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\g_automath_primitive_singlekey_return:n { #1 }
	\tl_set:cx { g_automath_#1_symbol }
	{
		{ \exp_not:n { \exp_not:n { #2 } } }
		{ \g_automath_tl_get:nn { #1 } { spar_open } }
		{ \g_automath_tl_get:nn { #1 } { spar_close } }
		{ \exp_not:v { g_automath_#1_symbol } }
	}
	\tl_put_left:cn { g_automath_#1_symbol }
	{
		\exp_not:N
		\g_automath_symbol_parentheses:nnnn
	}
%	\tl_set:Nn\l__automath_spar_temp
%	{
%		\exp_not:N
%		\g_automath_symbol_parentheses:nnnn
%	}
%	\tl_put_right:Nx\l__automath_spar_temp
%	{
%		{ \exp_not:n { \exp_not:N #2 } }
%		{ \g_automath_tl_get:nn { #1 } { spar_open } }
%		{ \g_automath_tl_get:nn { #1 } { spar_close } }
%		{ \exp_not:v { g_automath_#1_symbol } }
%	}
%	\tl_set_eq:cN { g_automath_#1_symbol } \l__automath_spar_temp
}

\cs_new:Npn\g_automath_primitive_singlekey_spar:n#1{
	\g_automath_tl_inherit:nn { #1 } { spar_size }
%	\g_automath_tl_inherit:nn { #1 } { spar_open }
%	\g_automath_tl_inherit:nn { #1 } { spar_close }
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\g_automath_primitive_singlekey_return:n { #1 }
%	\tl_set:Nn\l__automath_spar_temp
%	{
%		\exp_not:N
%		\g_automath_symbol_parentheses:nnnn
%	}
%	\tl_put_right:Nx\l__automath_spar_temp
%	{
%		{ \exp_not:v { g_automath_#1_spar_size } }
%		{ \g_automath_tl_get:nn { #1 } { spar_open } }
%		{ \g_automath_tl_get:nn { #1 } { spar_close } }
%		{ \exp_not:v { g_automath_#1_symbol } }
%	}
%	\tl_set_eq:cN { g_automath_#1_symbol } \l__automath_spar_temp
	%\tl_set:cx { g_automath_#1_symbol } {\exp_not:V\l__automath_spar_temp}
	\tl_set:cx { g_automath_#1_symbol }
	{
		{ \exp_not:v { g_automath_#1_spar_size } }
		%IM Could replace this by \exp_not:V and a temporary command,
		%IM like in _return
		{ \g_automath_tl_get:nn { #1 } { spar_open } }
		{ \g_automath_tl_get:nn { #1 } { spar_close } }
		{ \exp_not:v { g_automath_#1_symbol } }
	}
	\tl_put_left:cn { g_automath_#1_symbol }
	{
		\exp_not:N
		\g_automath_symbol_parentheses:nnnn
	}
}

\cs_new:Npn\g_automath_auxiliary_first_arg:nn#1#2 { #1 }
\cs_new:Npn\g_automath_auxiliary_second_arg:nn#1#2 { #2 }

%\cs_new:Npn\g_automath_primitive_keyval_otherspar:nn#1#2
%{
%	\g_automath_tl_inherit:nn { #1 } { spar_size }
%	\g_automath_tl_inherit:nn { #1 } { symbol }
%	\g_automath_primitive_singlekey_return:n { #1 }
%%	\tl_set:Nn\l__automath_spar_temp
%%	{
%%		\exp_not:N
%%		\g_automath_symbol_parentheses:nnnn
%%	}
%%	\tl_put_right:Nx\l__automath_spar_temp
%%	{
%%		{ \exp_not:v { g_automath_#1_spar_size } }
%%		{ \g_automath_auxiliary_first_arg:nn#2 }
%%		{ \g_automath_auxiliary_second_arg:nn#2 }
%%		{ \exp_not:v { g_automath_#1_symbol } }
%%	}
%%	\tl_set:cx { g_automath_#1_symbol } { \exp_not:V\l__automath_spar_temp }
%	\tl_set:cx { g_automath_#1_symbol }
%	{
%		%{ \exp_not:c { g_automath_#1_spar_size } }
%		{ \exp_not:n { \use:c { g_automath_#1_spar_size } } }
%		{ \g_automath_auxiliary_first_arg:nn #2 }
%		{ \g_automath_auxiliary_second_arg:nn #2 }
%		{ \exp_not:v { g_automath_#1_symbol } }
%	}
%	\tl_put_left:cn { g_automath_#1_symbol }
%	{
%		\exp_not:N
%		\g_automath_symbol_parentheses:nnnn
%	}
%}

\cs_new:Npn\g_automath_primitive_keyval_otherspar:nn#1#2
{
	\g_automath_primitive_keyval_otherspar_auxiliary:nnn { #1 } #2
}

\cs_new:Npn\g_automath_primitive_keyval_otherspar_auxiliary:nnn#1#2#3
{
	\g_automath_tl_inherit:nn { #1 } { spar_size }
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\g_automath_primitive_singlekey_return:n { #1 }
%	\tl_set:Nn\l__automath_spar_temp
%	{
%		\exp_not:N
%		\g_automath_symbol_parentheses:nnnn
%	}
%	\tl_put_right:Nx\l__automath_spar_temp
%	{
%		{ \exp_not:v { g_automath_#1_spar_size } }
%		{ \g_automath_auxiliary_first_arg:nn#2 }
%		{ \g_automath_auxiliary_second_arg:nn#2 }
%		{ \exp_not:v { g_automath_#1_symbol } }
%	}
%	\tl_set:cx { g_automath_#1_symbol } { \exp_not:V\l__automath_spar_temp }
	\tl_set:cx { g_automath_#1_symbol }
	{
		\exp_not:N
		\g_automath_symbol_parentheses:nnnn
		%{ \exp_not:c { g_automath_#1_spar_size } }
		%{ \exp_not:n { \use:c { g_automath_#1_spar_size } } }
		%{ normal }
		{ \exp_not:n { \exp_not:v { g_automath_#1_spar_size } } }
		{ #2 }
		{ #3 }
		{ \exp_not:v { g_automath_#1_symbol } }
	}
	%\tl_put_left:cn { g_automath_#1_symbol }
	%{
	%	\exp_not:N
	%	\g_automath_symbol_parentheses:nnnn
	%}
}

\cs_new:Npn\g_automath_primitive_keyval_sparsize:nn#1#2{
	% sets the size of the parentheses
	\tl_set:cn { g_automath_#1_spar_size }{ \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_spar_size } { #2 }
	%\tl_set:cx { g_automath_#1_spar_size } { \exp_args:N #2 }
}

\cs_new:Npn\g_automath_primitive_keyval_leftspar:nn#1#2{
	\tl_set:cn { g_automath_#1_spar_open }{ \exp_not:n { \exp_not:n { #2 } } }
	%IM Two \exp_not necessary for unknown reasons
	%IM Doing the same at leftpar yields an error.
}

\cs_new:Npn\g_automath_primitive_keyval_rightspar:nn#1#2{
	\tl_set:cn { g_automath_#1_spar_close }{ \exp_not:n { \exp_not:n { #2 } } }
	%IM Two \exp_not necessary for unknown reasons
	%IM Doing the same at leftpar yields an error.
}


%\def\keyvalue{} % create the command \keyvalue





%\msg_new:nnnn { automath } { singlekey_not_found } { Unknown~key~#1~passed~to~object~#2~on~input~line~\msg_line_number: } {}

\cs_new:Npn \g_automath_keyval:nnnn#1#2#3#4{
	% Takes care of keyvals, keys with a value
	% For the sake of implementation, the arguments
	% come in a strange order
	% #1 = value of key
	% #2 = name of the key
	% #3 = class
	% #4 = object
	\tl_set:Nn\keyvalue{\exp_not:n{#1}} % stores the content of the key in the temporary command \keyvalue
	%\tl_set:Nn\keyvalue{#1}
	%\tl_set:No\keyvalue{\exp_not:n{#1}} % stores the content of the key in the temporary command \keyvalue
	%IM think about using extra {...} to avoid interference with keyval str
	\g_automath_keyval_get:nnNTF { #4 } { #2 } \l_automath_custom_keyval_temp
	{
		\exp_args:Nnx
		%\use:c { g_automath_#4_keys_set:n }
		\g_automath_keys_set:nn { #4 }
		{ \l_automath_custom_keyval_temp }
	}
	{
		\cs_if_exist:cTF { g_automath_primitive_keyval_#2:nn }
		{
			\use:c { g_automath_primitive_keyval_#2:nn }{ #4 }{ #1 }%
		}
		{
			\msg_error:nnnn { automath } { keyval_not_found } { #2 } { #4 }
		}
	}
}

\cs_new:Npn \g_automath_singlekey:nnn#1#2#3
{
	% #1 = name of the key
	% #2 = class
	% #3 = object
%	% takes care of single keys, keys without a value
	\g_automath_singlekey_get:nnNTF { #3 } { #1 } \l_automath_custom_singlekey_temp
	{
		%\exp_args:NNno
		%\exp_args:Nno
		\exp_args:Nnx
		%\use:c { g_automath_#3_keys_set:n }
		\g_automath_keys_set:nn { #3 }
		{
			{ \l_automath_custom_singlekey_temp }
		}
	}
	{
		%\use:c { g_automath_primitive_singlekey_#1:n }{ #3 }%
		%\cs_if_exist:cTF { g_automath_primitive_singlekey_#1:n }
		%{
		%	\use:c { g_automath_primitive_singlekey_#1:n }{ #3 }%
		%}
		\str_case:nnTF { #1 }
		{
			{ return }
			{
				\g_automath_primitive_singlekey_return:n { #3 }
			}
			{ widetilde }
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \widetilde }
				\g_automath_primitive_keyval_command:nn { #3 } { \widetilde }
			}
			{ tilde }
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \widetilde }
				\g_automath_primitive_keyval_command:nn { #3 } { \tilde }
			}
			{ widebar } %IM remove in package
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \widebar }
				\g_automath_primitive_keyval_command:nn { #3 } { \exp_not:N\widebar }
			}
			{ overline }
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \widebar }
				\g_automath_primitive_keyval_command:nn { #3 } { \overline }
			}
			{ smallbar }
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \widebar }
				\g_automath_primitive_keyval_command:nn { #3 } { \bar }
			}
			{ bold }
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \mathbf }
				\g_automath_primitive_keyval_command:nn { #3 } { \mathbf }
			}
			{ upright } %IM remove in package
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \mathup }
				\g_automath_primitive_keyval_command:nn { #3 } { \mathup }
			}
			{ par }
			{
				%\g_automath_primitive_keyval_par:nn { #3 }{ normal }
				\g_automath_primitive_keyval_ifpar:nn { #3 } { true }
			}
			{ nopar }
			{
				%\g_automath_primitive_keyval_par:nn { #3 }{ none }
				\g_automath_primitive_keyval_ifpar:nn { #3 } { false }
			}
			{ spar }
			{
				\g_automath_primitive_singlekey_spar:n { #3 }
			}
			%			{ * } { \g_automath_keyval:nnn { #1 } { n } { \automath_bullet_tl }}
			%			{ ** }{ \g_automath_keyval:nnn { #1 } { n } { \automath_double_bullet_tl }}
			%IM add these again, together with \big, etc., maybe with [auto]
			{ bullet }
			{
				%\g_automath_keyval:nnn { #1 } { n } { \automath_bullet_tl } % bullet in the n-index
				%\g_automath_primitive_keyval_d:nn { #3 } { \automath_bullet_tl }
				\g_automath_keys_set:nn { #3 } { degreedefault = \automath_bullet_tl }
			}
			{ doublebullet }
			{
				%\g_automath_keyval:nnn { #1 } { n } { \automath_double_bullet_tl } % double bullet in the n-index
				%\g_automath_primitive_keyval_d:nn { #3 } { \automath_double_bullet_tl }
				\g_automath_keys_set:nn { #3 } { degreedefault = \automath_double_bullet_tl }
			}
			{ prime }
			{
				%\g_automath_keys_set:nnn { #3 } { upper } { \prime }
				\g_automath_primitive_keyval_upper:nn { #3 } { \prime }
			}
			{ ibullet }
			{
				%\g_automath_keyval:nnn { #3 } { i } { \automath_bullet_tl } % bullet in the i-index
				\g_automath_primitive_keyval_i:nn { #3 } { \automath_bullet_tl }
			}
			{ idoublebullet }
			{
				%\g_automath_keyval:nnn { #3 } { i } { \automath_double_bullet_tl } % double bullet in the i-index
				\g_automath_primitive_keyval_i:nn { #3 } { \automath_double_bullet_tl }
			}
			%			% Some commands to clear some registers:
			{ clearcommand }
			{
				\seq_clear:c { g_automath_#3_commands_sequence }
				%IMplement again
			}
			{ clearkeyvals } %IM also allow removing one keyval etc.
			{
				\tl_clear:c { g_automath_#3_custom_keyvals }
			}
			{ clearsinglekeys }
			{
				\tl_clear:c { g_automath_#3_custom_singlekeys }
			}
			{ clearargkeyvals }
			{
				\tl_clear:c { g_automath_#3_arg_custom_keyvals }
			}
			{ clearargsinglekeys }
			{
				\tl_clear:c { g_automath_#3_arg_custom_singlekeys }
			}
			{ clearupper }
			{
				\tl_clear:c { g_automath_#3_upper_index }
			}
			{ clearlower }
			{
				\tl_clear:c { g_automath_#3_lower_index }
			}
			{ cleararg }
			{
				\tl_clear:c { g_automath_#3_arg }
			}
			{ cleard } %IM clean up
			{
				\bool_if:cTF { g_automath_#3_if_upper_grading }
				{
					\tl_clear:c { g_automath_#3_upper_index }
				}
				{
					\tl_clear:c { g_automath_#3_lower_index }
				}
			}
			{ cleari } %IM clean up
			{
				\bool_if:cTF { g_automath_#3_if_upper_grading }
				{
					\tl_set:cn { g_automath_#3_lower_index } { } %empty
				}
				{
					\tl_set:cn { g_automath_#3_upper_index } { } %empty
				}
			}
			{ clearoutputoptions }
			{
				\tl_clear:c { g_automath_#3_output_options }
			}
		}
		{
			% if true; do nothing
		}
		{
			%\msg_error:nnnn { automath } { singlekey_not_found } { #1 } { #3 }
			%\g_automath_primitive_keyval_i:nn { #3 } { #1 }%
			%\use:c { g_automath_#3_keys_set:n } { default = {#1} }
			\g_automath_keys_set:nn { #3 } { default = { #1 } }
		}
	}
}

%IMplement the same thing for upper, lower

\cs_new:Npn \g_automath_arg_primitive_keyval_sep_auxiliary_function_withsep:nn#1#2
{
	#1#2
}

\cs_new:Npn \g_automath_arg_primitive_keyval_sep_auxiliary_function_withoutsep:nn#1#2
{
	#2
}

\cs_new:Npn \g_automath_primitive_arg_keyval_sep:nn#1#2
{
%	\tl_if_exist:cTF { g_automath_#1_arg }
%	{
%		% do nothing
%	}
%	{
%		\tl_new:c { g_automath_#1_arg }
%		\tl_set:cx { g_automath_#1_arg } { \g_automath_tl_get:nn { \g_automath_tl_get:nn { #1 } { parent } } { arg } }%IM change to :cn if we get a better if_first_arg system
%	}
	\g_automath_tl_inherit_x:nn { #1 } { arg }
	%\bool_if:cTF { g_automath_if_first_arg }
	%\g_automath_bool_get:nnTF { #3 } { first_arg }
	%\tl_if_empty:cTF { g_automath_#1_arg }
	\g_automath_bool_get:nnTF { #1 } { first_arg }
	{
		\tl_put_right:cn { g_automath_#1_arg } { \exp_not:n { \g_automath_arg_primitive_keyval_sep_auxiliary_function_withoutsep:nn #2 } }
		%IM These do not use :x, unlike the ones below
	}
	{
		\tl_put_right:cn { g_automath_#1_arg } { \exp_not:n { \g_automath_arg_primitive_keyval_sep_auxiliary_function_withsep:nn #2 } }
	}
	\g_automath_primitive_keyval_ifoutput:nn { #1 } { true }
	%IM this is not the right place to set this as true; probably it should
	%IM be in the user's setup of the arg key.
	\g_automath_bool_provide:nn { #1 } { first_arg }
	\bool_set_false:c { g_automath_#1_if_first_arg }
}

\cs_new:Npn \g_automath_primitive_arg_keyval_standardsep:nn#1#2
{
%	\tl_if_exist:cTF { g_automath_#1_arg }
%	{
%		% do nothing
%	}
%	{
%		\tl_new:c { g_automath_#1_arg }
%		\tl_set:cx { g_automath_#1_arg } { \g_automath_tl_get:nn { \g_automath_tl_get:nn { #1 } { parent } } { arg } }%IM change to :cn if we get a better if_first_arg system
%	}
	\g_automath_tl_inherit_x:nn { #1 } { arg }
	%\bool_if:cTF { g_automath_if_first_arg }
	%\g_automath_bool_get:nnTF { #3 } { first_arg }
	\g_automath_bool_get:nnTF { #1 } { first_arg }
	{
		%\tl_put_right:cx { g_automath_#1_arg } { \exp_not:n{\exp_not:n { #2 } }}
		\tl_put_right:cx { g_automath_#1_arg } { \exp_not:n { #2 } }
		%IM Recently corrected
	}
	{
		\tl_put_right:cx { g_automath_#1_arg } { \exp_not:n { \g_automath_tl_get:nn { #1 } { argsep } } \exp_not:n { #2 } }
	}
	\g_automath_primitive_keyval_ifoutput:nn { #1 } { true }
	\g_automath_bool_provide:nn { #1 } { first_arg }
	\bool_set_false:c { g_automath_#1_if_first_arg }
}

\cs_new:Npn \g_automath_arg_keyval:nnnn#1#2#3#4
{
	% Takes care of keyvals, keys with a value
	% For the sake of implementation, the arguments
	% come in a strange order
	% #1 = value of key
	% #2 = name of the key
	% #3 = class
	% #4 = object
	\tl_set:Nn\keyvalue{\exp_not:n{#1}} % stores the content of the key in the temporary command \keyvalue
	\g_automath_arg_keyval_get:nnNTF { #4 } { #2 } \l_automath_custom_arg_keyval_temp
	{
		\exp_args:Nnx
		\g_automath_arg_keys_set:nn { #4 } { \l_automath_custom_arg_keyval_temp }
	}
	{
		\cs_if_exist:cTF { g_automath_primitive_arg_keyval_#2:nn }
		{
			\use:c { g_automath_primitive_arg_keyval_#2:nn }{ #4 }{ #1 }%
		}
		{
			\msg_error:nnnn { automath } { arg_keyval_not_found } { #2 } { #4 }
		}
	}
}


\cs_new:Npn \g_automath_arg_singlekey:nnn#1#2#3
{
	% #1 = name of the key
	% #2 = class
	% #3 = object
%	% takes care of single keys, keys without a value
	\g_automath_arg_singlekey_get:nnNTF { #3 } { #1 } \l_automath_custom_arg_singlekey_temp
	{
		%\exp_args:NNno
		%\exp_args:Nno
		\exp_args:Nnx
		%\use:c { g_automath_#3_arg:n }
		\g_automath_arg_keys_set:nn { #3 }
		{
			\l_automath_custom_arg_singlekey_temp
		}
	}
	{
		\str_case:nnTF { #1 }
		{
			{...}{
				\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \g_automath_tl_get:nn { #3 } { argdots } }
				%IMplement the same for symbols
			}
			{-}{
				\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \g_automath_tl_get:nn { #3 } { slot } }
				%IMplement the same for symbols
				%IM Also, allow editing slots
			}
			{*}{
							\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \g_automath_tl_get:nn { #3 } { slot } }
							%IMplement the same for symbols
							%IM Also, allow editing slots
			}
			{slot}{
				\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \g_automath_tl_get:nn { #3 } { slot } }
				%IMplement the same for symbols
			}
		}
		{
			% if true; do nothing
		}
		{
			\g_automath_tl_inherit_x:nn { #3 } { arg }
			%\bool_if:cTF { g_automath_if_first_arg }
			%\g_automath_bool_get:nnTF { #3 } { first_arg }
%			\tl_if_empty:cTF { g_automath_#3_arg }
%			{
%				\tl_put_right:cn { g_automath_#3_arg } { \exp_not:n { #1 } }
%			}
%			{
%				\tl_put_right:cn { g_automath_#3_arg } { \g_automath_tl_get:nn { #3 } { argsep } \exp_not:n { #1 } }
%				%IMplement "arg", similarly to "default"
%				%IMPORTANT: Think about using x-type expansion here,
%				%IM which is done in the other place where arguments are
%				%IM added. This should maybe be the standard.
%			}
%			\g_automath_primitive_keyval_ifoutput:nn { #3 } { true }
			%\exp_args:Nnx\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \exp_not:n { \exp_not:n { #1 } } }
			%\exp_args:Nnx\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \exp_not:n { #1 } }
			%\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { #1 }
			%
			%
			%
			%
			%
			%\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \exp_not:n { #1 } }
			\g_automath_arg_keys_set:nn { #3 } { default={\exp_not:n { #1 } }}
			%\g_automath_arg_keys_set:nn { #3 } { default={#1}}
			%IM THis \exp_not:n was added late, might be needed elsewhere, too.
		}
	}
}

%\tl_new:N\g_automath_automathvariable_parent
%\tl_set:Nn\g_automath_automathvariable_parent { automathvariable }

\g_automath_tl_provide:nn { automathvariable } { output }
\tl_set:Nn\g_automath_automathvariable_output{ automathvariable }


\g_automath_tl_provide:nn { automathvariable } { upper_index }

\g_automath_tl_provide:nn { automathvariable } { uppersep }

\tl_set:Nn \g_automath_automathvariable_uppersep { , }

%IM do the same with all the others, INCLUDING if_upper_grading and symbol
%IM Also, need commands like forgetupperindex, reverting to the class standard

\g_automath_tl_provide:nn { automathvariable } { lower_index }

\g_automath_tl_provide:nn { automathvariable } { lowersep }

\tl_set:Nn \g_automath_automathvariable_lowersep { , }


\g_automath_tl_provide:nn { automathvariable } { preupper }

\g_automath_tl_provide:nn { automathvariable } { postupper }

\g_automath_tl_provide:nn { automathvariable } { prelower }

\g_automath_tl_provide:nn { automathvariable } { postlower }

\g_automath_tl_provide:nn { automathvariable } { prearg }

\g_automath_tl_provide:nn { automathvariable } { postarg }
%IMplement these later

\g_automath_tl_provide:nn { automathvariable } { arg }

\g_automath_tl_provide:nn { automathvariable } { argsep }
\tl_set:Nn \g_automath_automathvariable_argsep {,}

\g_automath_tl_provide:nn { automathvariable } { slot }
\tl_set:Nn \g_automath_automathvariable_slot { \slot }

\g_automath_tl_provide:nn { automathvariable } { argdots }
\tl_set:Nn \g_automath_automathvariable_argdots {\ldots}

\g_automath_tl_provide:nn { automathvariable } { symbol }

\bool_new:N\g_automath_automathvariable_commands_sequence_if_provided
\bool_set_true:N\g_automath_automathvariable_commands_sequence_if_provided
\seq_new:N\g_automath_automathvariable_commands_sequence

%\tl_new:N\g_automath_automathvariable_output_options

\g_automath_bool_provide:nn { automathvariable } { upper_grading }
\bool_set_true:N \g_automath_automathvariable_if_upper_grading

\g_automath_bool_provide:nn { automathvariable } { output }

\g_automath_tl_provide:nn { automathvariable } { output_options }

\g_automath_bool_provide:nn { automathvariable } { first_arg }
\bool_set_true:N\g_automath_automathvariable_if_first_arg

\g_automath_bool_provide:nn { automathvariable } { first_upper }
\bool_set_true:N\g_automath_automathvariable_if_first_upper

\g_automath_bool_provide:nn { automathvariable } { first_lower }
\bool_set_true:N\g_automath_automathvariable_if_first_lower

\g_automath_bool_provide:nn { automathvariable } { par }
\bool_set_true:N\g_automath_automathvariable_if_par




%\tl_set:Nn\g_objectmath_automathvariable_upper_index { hej }
%\tl_set:Nn \g_automathvariable_output { automathvariable }
%\bool_new:N \g_automathvariable_output_if_provided
%\bool_set_true:N \g_automathvariable_output_if_provided


\newvariableclass{automathvariable}[
	%parent=automathvariable,
	symbol=,
	gradingpos=upper,
	%upper=,
	%lower=,
	leftpar=(,
	rightpar=),
	par=normal,
	leftspar=(,
	rightspar=),
	sparsize=normal,
	%arg=,
	ifoutput=false,
	output=automathvariable,
	singlekeys={
		{*}{bullet},
		{**}{doublebullet},
		{smash}{command=\noexpand\smash},
	},
	keyvals={
		{default}{si={\keyvalue}},
		{arg}{argwithkeyval={\keyvalue}},
		{degreedefault}{sd={\keyvalue}},
	},
	argkeyvals={
		{default}{standardsep={\keyvalue}},
	}
	%command=,
]

\ExplSyntaxOff

==> _commands/basics/_basics_1.tex <==
%Basic number sets
%\newcommand\N{\mathbb{N}}
%\newcommand\Z{\mathbb{Z}}
%\newcommand\Q{\mathbb{Q}}
%\newcommand\R{\mathbb{R}}
%\newcommand\C{\mathbb{C}}
%\newcommand\F{\mathbb{F}}
%\newcommand\Zmod[1]{\Z/#1}
%\newcommand\differentialD{d\!}

\newvariableclass{var}[
	parent=automathvariable,
	output=var,
	singlekeys={
		{inv}{upper=-1},
		{conj}{command=\noexpand\overline},
		{varconj}{command=\noexpand\bar},
		{Varconj}{command=\noexpand\widebar},
	},
]

\newvar\vx{x}
\newvar\vy{y}
\newvar\vz{z}

\newvariableclass{classset}[
	parent=var,
	keyvals={
		{power}{upper={\keyvalue}},
		{invar}{upper={\keyvalue}},
		{coinvar}{lower={\keyvalue}},
	},
	singlekeys={
		{closure}{command=\noexpand\overline},
		{varclosure}{command=\noexpand\bar},
		{Varclosure}{command=\noexpand\widebar},
		{interior}{upper=\circ},
	},
]

\newcommand\newdelimsize{\noexpand\automathdelimsize}

\newvariableclass{alg}[
	parent=classset,
	output=alg,
	keyvals={
		{oplus}{upper={\oplus\keyvalue}},
		{coprod}{upper={\smallcoprod\keyvalue}},
		{prod}{upper={\smallprod\keyvalue}},
		{mod}{symbolputright={/\keyvalue}},
		{modn}{symbolputright={/\keyvalue}},
		{shift}{symbolputright={[\keyvalue]}},
		{power}{upper={\keyvalue}},
		{diag}{upper={\keyvalue}},
		{functors}{upper={\keyvalue}},
	},
	singlekeys={
		{pol}{
			nowoutput=algop,
			outputoptions={par,leftpar=\lbrack,rightpar=\rbrack,},
		},
		{field}{
			nowoutput=algop,
			outputoptions={par,leftpar=(,rightpar=),},
		},
		{powerseries}{
			%nowoutput=algop,
			%outputoptions={par,leftpar=\noexpand\llbracket,rightpar=\noexpand\rrbracket,},
			nowoutput=algoppowerseries,
		},
		{freealg}{
			nowoutput=algopfreealg,
			%nowoutput=algop,
			%outputoptions={par,leftpar=\langle,rightpar=\rangle},
		},
		{laurent}{
			nowoutput=algoplaurent,
		},
		%These are for categories:
		{fg}{upper=\mathup{fg}},
		{interiorgroupoid}{upper=\circ},
		{localize}{
			return,
			nowoutput=localizedcategory,
		},
		{fin}{upper=\mathup{fin}},
		{varfin}{upper=\mathup{f}},
		{findim}{upper=\mathup{f}},
		{op}{upper=\mathup{op}},
	},
]


\newalg\N{\mathbb{N}}
\newalg\Z{\mathbb{Z}}
\newalg\Q{\mathbb{Q}}
\newalg\R{\mathbb{R}}
\newalg\C{\mathbb{C}}
\newalg\F{\mathbb{F}}
%\newmap\Zmod{\mathbb{Z}}[
%	%parent=alg,
%	leftpar=/,
%	rightpar=,
%	output=alg,
%]





%\DeclareDocumentCommand\D{sd()mo}{
%	%The first star is pure mark-up; it marks that
%	%the #2 argument is a measure rather than a
%	%variable. It is better to use it, even though
%	%it (with the current settings) has not consequence
%	%for the output.
%	\differentialD
%	\IfNoValueTF{#2}{
%		%do nothing
%	}{
%		^{#2}
%	}
%	#3
%	\IfNoValueTF{#4}{
%		%do nothing
%	}{
%		(#4)
%	}
%}

\begin{comment}
\newcommand\DD{\,\D}
\newcommand\E{e}
\newcommand\I{i}
\newcommand\conj\widebar
\newcommand\subs\subset
\newcommand\sups\superset
\newcommand\propersubs\subsetneq
\newcommand\propersups\supsetneq
\newcommand\inv{^{-1}}
\newcommand\pre{^{-1}}
\newcommand\trans{^{\textup{T}}}
\newcommand\adj{^{*}}
\newcommand\dual{^{*}}
\newcommand\push{_{*}}
\newcommand\pull{^{*}}
\newcommand\units{^{\times}}
\newcommand\op{^{\mathup{op}}}
\newcommand\ort{^{\perp}}

\end{comment}

%\newcommand\sym[1]{\mathfrak{S}_{#1}} % the symmetric group



%\newcommand\iso{\cong}




%\DeclarePairedDelimiter\tup{(}{)} % tuples

\begin{comment}
\newcommand\matlogo{\mathup{M}}
\DeclareDocumentCommand\tempmat{mmm}{
	\matlogo_{#1\times #2}(#3)
}
\DeclareDocumentCommand\tempsqmat{mm}{
	\matlogo_{#1}(#2)
}
\DeclareDocumentCommand\mat{ms}{
	\IfBooleanTF{#2}{Exercise
		\tempmat{#1}
	}{
	\tempsqmat{#1}
}
}
\end{comment}


%\DeclareDocumentCommand\mat{msm}{\mathup{M}_{
%		\IfBooleanTF{#2}{
%			(#1)
%		}{
%			#1
%		}
%		}(#3)}
%
%\DeclareDocumentCommand\matmn{msmsm}{
%	\mat{
%		\IfBooleanTF{#2}{(#1)}{#1}
%		\times
%		\IfBooleanTF{#4}{(#3)}{#3}
%	}{#5}
%}


%\newcommand\der[1]{^{(#1)}} % derivative

%\newcommand\exterior[1]{{\textstyle\bigwedge^{\!\!#1}}} %for exterior powers


\newcommand\smallprod{\mathbin{\text{\rotatebox[origin=c]{180}{$\amalg$}}}}
\newcommand\smallcoprod{\amalg}

\newcommand\smallbullet{\raisebox{-0.25ex}{\scalebox{1.2}{$\cdot$}}}

%\newcommand\comp{^{\smallbullet}} %cocomplexes
%\newcommand\hocomp{_{\smallbullet}} %complexes
%\newcommand\simp{_{\smallbullet}} % complexes
%\let\hocomp=\simp

%\newcommand\bicomp{^{\smallbullet\smallbullet}}
%\newcommand\bihocomp{_{\smallbullet\smallbullet}}
%\newcommand\bisimp{_{\smallbullet\smallbullet}}
%\let\bihocomp=\bisimp

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareMathSymbol{\intprod}{\mathbin}{MnSyC}{'270} %internal product of forms, "into"

==> _commands/categories/_categories_2.tex <==
%\newcommand\categoryformat[1]{\textup{\textbf{#1}}} % no current format

%\newvariableclass{category}[parent=alg,command=\categoryformat]
%\newmapclass{categoryof}[parent=category]

%\newmapclass{category}[parent=alg,command=\categoryformat,output=alg]

%\newmapclass{category}[
%	parent=alg,output=category,
%	]

\newmapclass{localizedcategory}[
	parent=alg,
	leftpar=\lbrack,rightpar=\rbrack,
	argkeyvals={
		{default}{{standardsep={\keyvalue^{-1}}}},
	},
]

\newcommand\categoryformat[1]{\textup{#1}}

\newmapclass{category}[parent=alg,command=\categoryformat]

\newcommand\catxmod[1]{\category{$#1$-mod}}
\newcategory\catRmod{$R$-mod}
\newcategory\catAmod{$A$-mod}

\newcommand\catmodx[1]{\category{mod-$#1$}}
\newcategory\catmodR{mod-$R$}
\newcategory\catmodA{mod-$A$}

\newcommand\catxmodx[2]{\category{$#1$-mod-$#2$}}
\newcategory\catRmodR{$R$-mod-$R$}
\newcategory\catAmodA{$A$-mod-$A$}


\newcommand\catxdgmod[1]{\category{$#1$-dgmod}}
\newcategory\catRdgmod{$R$-dgmod}
\newcategory\catAdgmod{$A$-dgmod}

\newcommand\catdgmodx[1]{\category{dgmod-$#1$}}
\newcategory\catdgmodR{dgmod-$R$}
\newcategory\catdgmodA{dgmod-$A$}

\newcommand\catxdgmodx[2]{\category{$#1$-dgmod-$#2$}}
\newcategory\catRdgmodR{$R$-dgmod-$R$}
\newcategory\catAdgmodA{$A$-dgmod-$A$}


\newcommand\catxcomod[1]{\category{$#1$-comod}}
\newcategory\catRcomod{$R$-comod}
\newcategory\catAcomod{$A$-comod}

\newcommand\catcomodx[1]{\category{comod-$#1$}}
\newcategory\catcomodR{comod-$R$}
\newcategory\catcomodA{comod-$A$}

\newcommand\catxcomodx[2]{\category{$#1$-comod-$#2$}}
\newcategory\catRcomodR{$R$-comod-$R$}
\newcategory\catAcomodA{$A$-comod-$A$}


%\newcategoryof\catvect{Vect}

\newcategory\catset{Set}
\newcategory\cattop{Top}


\newcategory\catvect{Vect}
\newcategory\catcat{Cat}
\newcategory\catab{Ab}
\newcategory\catgrp{Grp}
\newcategory\catcom{Com}
\newcategory\catalg{Alg}

\newcategory\catdgalg{dgAlg}
\newcategory\catainftyalg{$\mathup{A}_{\infty}$Alg}
\newcategory\catdgcat{dgCat}
\newcategory\catainftycat{$\mathup{A}_{\infty}$Cat}


\newcategory\catfun{Fun}
\newcategory\catdgfun{dgFun}
\newcategory\catainftyfun{$\mathup{A}_{\infty}$Fun}


\newmapclass{derivedcategory}[
	parent=alg,
	output=alg,
	singlekeys={
		{b}{upper=b},
		{+}{upper=+},
		{-}{upper=-},
		{+-}{upper=\pm},
		{pm}{upper=\pm},
		{ge0}{upper=\ge0},
		{le0}{upper=\le0},
		{fil}{upper=\mathup{fil}},
	},
]

\newderivedcategory\der{\mathscr{D}}



%\newcommand\category[1]{\textup{\textbf{#1}}}%For categories




%Specific categories


%
%
%\newcommand\catxmod[1]{\category{$#1$-mod}}
%	\newcommand\catRmod{\catxmod{R}}
%	\newcommand\catSmod{\catxmod{S}}
%	\newcommand\catAmod{\catxmod{A}}
%	\newcommand\catBmod{\catxmod{B}}
%\newcommand\catxmodf[1]{\category{$#1$-mod\textsuperscript{f}}}
%	\newcommand\catRmodf{\catxmodf{R}}
%	\newcommand\catSmodf{\catxmodf{S}}
%	\newcommand\catAmodf{\catxmodf{A}}
%	\newcommand\catBmodf{\catxmodf{B}}
%\newcommand\catmodx[1]{\category{mod-$#1$}}
%	\newcommand\catmodR{\catmodx{R}}
%	\newcommand\catmodS{\catmodx{S}}
%	\newcommand\catmodA{\catmodx{A}}
%	\newcommand\catmodB{\catmodx{B}}
%\newcommand\catxmodx[2]{\category{$#1$-mod-$#2$}}
%	\newcommand\catRmodR{\catxmodx{R}{R}}
%	\newcommand\catRmodS{\catxmodx{R}{S}}
%	\newcommand\catAmodA{\catxmodx{A}{A}}
%	\newcommand\catAmodB{\catxmodx{A}{B}}
%\newcommand\catxbimod[1]{\catxmodx{#1}{#1}}
%	\newcommand\catRbimod{\catxbimod{R}}
%	\newcommand\catAbimod{\catxbimod{A}}
%\newcommand\catxdgmod[1]{\category{$#1$-DGmod}}
%	\newcommand\catRdgmod{\catxdgmod{R}}
%	\newcommand\catSdgmod{\catxdgmod{S}}
%	\newcommand\catAdgmod{\catxdgmod{A}}
%	\newcommand\catBdgmod{\catxdgmod{B}}
%\newcommand\catdgmodx[1]{\category{DGmod-$#1$}}
%	\newcommand\catdgmodR{\catdgmodx{R}}
%	\newcommand\catdgmodS{\catdgmodx{S}}
%	\newcommand\catdgmodA{\catdgmodx{A}}
%	\newcommand\catdgmodB{\catdgmodx{B}}
%\newcommand\catxdgcomod[1]{\category{$#1$-DGcomod}}
%	\newcommand\catCdgcomod{\catxcomod{C}}
%\newcommand\catdgcomodx[1]{\category{DGcomod-$#1$}}
%	\newcommand\catdgcomodC{\catcomodx{C}}
%\newcommand\catxdgcontra[1]{\category{$#1$-DGcontra}}
%	\newcommand\catCdgcontra{\catxdgcontra{C}}
%\newcommand\catdgcontrax[1]{\category{dgcontra-$#1$}}
%	\newcommand\catdgcontraC{\catdgcontrax{C}}
%\newcommand\catvect{\category{Vect}}
%\newcommand\catvectf{\category{Vect\textsuperscript{f}}}
%\newcommand\catvectx[1]{\catvect\pars{#1}}
%	\newcommand\catvectk{{\catvectx{k}}}
%\newcommand\catvectfx[1]{\catvectf\pars{#1}}
%	\newcommand\catvectfk{{\catvectfx{k}}}
%\newcommand\catset{\category{Set}}
%\newcommand\catcat{\category{Cat}}
%\newcommand\catab{\category{Ab}}
%\newcommand\catgrp{\category{Grp}}
%\newcommand\catcom{\category{Com}}
%\newcommand\catcomx{\catcom\pars}
%\newcommand\catalg{\category{Alg}}
%\newcommand\catalgx[1]{\category{Alg}\pars{#1}}
%	\newcommand\catalgk{{\catalg{k}}}
%\newcommand\catrng{\category{Rng}}
%\newcommand\cattop{\category{Top}}
%\newcommand\cathot[1]{\category{Hot}\pars{#1}}
%\newcommand\catproj{\category{Proj}}
%\newcommand\catprojx[1]{\catproj\pars{#1}}
%	\newcommand\catprojA{{\catprojx{A}}}
%\newcommand\catinj{\category{Inj}}
%\newcommand\catinjx[1]{\catinj{#1}}
%	\newcommand\catinjA{\catinjx{A}}
%\newcommand\catacycl{\category{Acycl}}
%	\newcommand\catacyclx[1]{\catacycl\pars{#1}}
%	\newcommand\catacyclA[1]{{\catacyclx{A}}}
%\newcommand\catacyclabs{\category{Acycl\textsubscript{abs}}}
%	\newcommand\catacyclabsx[1]{\catacyclabs\pars{#1}}
%	\newcommand\catacyclabsA[1]{{\catacyclabsx{A}}}
%\newcommand\catacyclco{\category{Acycl\textsubscript{co}}}
%	\newcommand\catacyclcox[1]{\catacyclco\pars{#1}}
%	\newcommand\catacyclcoA[1]{{\catacyclcox{A}}}
%\newcommand\catacyclctr{\category{Acycl\textsubscript{ctr}}}
%	\newcommand\catacyclctrx[1]{\catacyclctr\pars{#1}}
%	\newcommand\catacyclctrA[1]{{\catacyclctrx{A}}}
%
%
%\newcommand\Lperp[1]{{}^{\perp}#1}
%\newcommand\lperp[1]{\lperp{(#1)}}
%\newcommand\Rperp[1]{#1^{\perp}}
%\newcommand\rperp[1]{\Rperp{(#1)}}
%
%\newcommand\catderivedD{\mathscr{D}}
%\newcommand\catder[2][]%
%{
%	\catderivedD
%	\ifblank{#1}
%	{
%		% do nothing
%	}
%	{
%		^{#1}
%	}
%	\pars{#2}
%}
%\newcommand\catderp[1]{\catderivedD^{+}\pars{#1}}
%\newcommand\catderm[1]{\catderivedD^{-}\pars{#1}}
%\newcommand\catderpm[1]{\catderivedD^{\pm}\pars{#1}}
%\newcommand\catderb[1]{\catderivedD^{b}\pars{#1}}
%\newcommand\catderabs[1]{\catderivedD^{\mathup{abs}}\pars{#1}}
%	\newcommand\catderabsp[1]{\catderivedD^{\mathup{abs},+}\pars{#1}}
%	\newcommand\catderabsm[1]{\catderivedD^{\mathup{abs},-}\pars{#1}}
%	\newcommand\catderabspm[1]{\catderivedD^{\mathup{abs},\pm}\pars{#1}}
%	\newcommand\catderabsb[1]{\catderivedD^{\mathup{abs},b}\pars{#1}}
%\newcommand\catderco[1]{\catderivedD^{\mathup{co}}\pars{#1}}
%	\newcommand\catdercop[1]{\catderivedD^{\mathup{co,+}}\pars{#1}}
%	\newcommand\catdercom[1]{\catderivedD^{\mathup{co,-}}\pars{#1}}
%	\newcommand\catdercopm[1]{\catderivedD^{\mathup{co,\pm}}\pars{#1}}
%	\newcommand\catdercob[1]{\catderivedD^{\mathup{co,b}}\pars{#1}}
%\newcommand\catderctr[1]{\catderivedD^{\mathup{ctr}}\pars{#1}}
%	\newcommand\catderctrp[1]{\catderivedD^{\mathup{ctr,+}}\pars{#1}}
%	\newcommand\catderctrm[1]{\catderivedD^{\mathup{ctr,-}}\pars{#1}}
%	\newcommand\catderctrpm[1]{\catderivedD^{\mathup{ctr,\pm}}\pars{#1}}
%	\newcommand\catderctrb[1]{\catderivedD^{\mathup{ctr,b}}\pars{#1}}

==> _commands/catlimits/_catlimits_1.tex <==
%Inverse and direct limits that look nicer:

\newcommand\newdirlim[2]{
	%#1 = command name
	%#2 = text name
	\newcommand#1{
		\mathop{
			\smash{
				\operatorname*{#2}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xrightarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#2}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
	}
}

\newcommand\newinvlim[2]{
	%#1 = command name
	%#2 = text name
	\newcommand#1{
		\mathop{
			\smash{
				\operatorname*{#2}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xleftarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#2}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
	}
}



\newdirlim\dirlim{lim}
\newinvlim\invlim{lim}

\newdirlim\holim{holim}
%newinvlim\invholim{holim}


\begin{comment}
\newcommand\dirlim{
	\mathop{
		\smash{
			\lim\limits_{
				{}
				\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$\xrightarrow{\hspace*{1.15em}}$}}
			}
		}
		\vphantom{\textstyle\lim_n}
	}
}

\newcommand\invlim{
	\mathop{
		\smash{
			\lim\limits_{
				{}
				\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$\xleftarrow{\hspace*{1.15em}}$}}
			}
		}
		\vphantom{\textstyle\lim_n}
	}
}
\end{comment}

\begin{comment}
\newcommand\dirlim{
	\mathop{
		\vphantom{g}
		\smash{
			\lim\limits
			_{
				\raisebox{.1em}[0pt][0pt]{$
					\xrightarrow{\hphantom{\hspace*{.95em}}}
					$}
			}
		}
	}
}

\newcommand\invlim{
	\mathop{
		\vphantom{g}
		\smash{
			\lim\limits
			_{
				\raisebox{.1em}[0pt][0pt]{$
					\xleftarrow{\hphantom{\hspace*{.95em}}}
					$}
			}
		}
	}
}
\end{comment}

==> _commands/catlimits/_catlimits_2.tex <==
%Inverse and direct limits that look nicer:

\newcommand\dirlimformat[1]{
	%#1 = text name
		\mathop{
			\smash{
				\operatorname*{#1}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xrightarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#1}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
}

\newcommand\invlimformat[1]{
	%#1 = text name
		\mathop{
			\smash{
				\operatorname*{#1}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xleftarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#1}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
}



%\newdirlim\dirlim{lim}
%\newinvlim\invlim{lim}

%\newdirlim\holim{holim}
%newinvlim\invholim{holim}

\newmapclass{catlim}[
	parent=algop,
	keyvals={
		{diag}{lower={\keyvalue}},
		{default}{diag={\keyvalue}},
		%{weight}{symbolputright={{}^{\keyvalue}},return,command=\mathop,symbolputright=\limits},
		{weight}{return,upper={\keyvalue}},
	},
]


\newcatlim\dirlim{\dirlimformat{lim}}
\newcatlim\invlim{\invlimformat{lim}}
\newcatlim\dirholim{\dirlimformat{holim}}
\newcatlim\invholim{\invlimformat{holim}}



\begin{comment}
\newcommand\dirlim{
	\mathop{
		\smash{
			\lim\limits_{
				{}
				\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$\xrightarrow{\hspace*{1.15em}}$}}
			}
		}
		\vphantom{\textstyle\lim_n}
	}
}

\newcommand\invlim{
	\mathop{
		\smash{
			\lim\limits_{
				{}
				\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$\xleftarrow{\hspace*{1.15em}}$}}
			}
		}
		\vphantom{\textstyle\lim_n}
	}
}
\end{comment}

\begin{comment}
\newcommand\dirlim{
	\mathop{
		\vphantom{g}
		\smash{
			\lim\limits
			_{
				\raisebox{.1em}[0pt][0pt]{$
					\xrightarrow{\hphantom{\hspace*{.95em}}}
					$}
			}
		}
	}
}

\newcommand\invlim{
	\mathop{
		\vphantom{g}
		\smash{
			\lim\limits
			_{
				\raisebox{.1em}[0pt][0pt]{$
					\xleftarrow{\hphantom{\hspace*{.95em}}}
					$}
			}
		}
	}
}
\end{comment}

==> _commands/catlimits/_catlimits_3.tex <==
%Inverse and direct limits that look nicer:

\newcommand\dirlimformat[1]{
	%#1 = text name
		\mathop{
			\smash{
				\operatorname*{#1}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xrightarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#1}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
}

\newcommand\invlimformat[1]{
	%#1 = text name
		\mathop{
			\smash{
				\operatorname*{#1}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xleftarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#1}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
}

%\NewDocumentCommand\dirlimcommand{me{_^}}{%
%	\mathchoice
%		{ \dirlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { {} ^ { #3 } } }
%	    { \dirlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%	    { \dirlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%	    { \dirlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%}

%\NewDocumentCommand\invlimcommand{me{_^}}{%
%	\mathchoice
%		{ \invlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { {} ^ { #3 } } }
%	    { \invlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%	    { \invlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%	    { \invlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%}





%\newdirlim\dirlim{lim}
%\newinvlim\invlim{lim}

%\newdirlim\holim{holim}
%newinvlim\invholim{holim}

\newmapclass{catlim}[
	parent=algop,
	keyvals={
		{diag}{lower={\keyvalue}},
		{default}{diag={\keyvalue},return},
		%{weight}{symbolputright={{}^{\keyvalue}},return,command=\mathop,symbolputright=\limits},
		{weight}{upper={\keyvalue},return},
	},
]


\newcatlim\dirlim{\dirlimformat{lim}}
\newcatlim\invlim{\invlimformat{lim}}
\newcatlim\dirholim{\dirlimformat{holim}}
\newcatlim\invholim{\invlimformat{holim}}


==> _commands/delims/_delims_1.tex <==

% \abs{x} for absolute values:
\DeclarePairedDelimiterX\abs[1]\lvert\rvert{
	\slotifempty{#1}
}

\DeclarePairedDelimiterX\size[1]\lvert\rvert{
	\slotifempty{#1}
}

\newcommand\varsize[1]{\#}

% \norm{x} for norms:
\DeclarePairedDelimiterX\norm[1]\lVert\rVert{ %normer
	\slotifempty{#1}
}
% \inner{u}{v} for inner products:
\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{ %indre produkter
	\slotifempty{#1},\slotifempty{#2}
}

\DeclarePairedDelimiterX\com[2]{[}{]}{ %commutator
	\slotifempty{#1},\slotifempty{#2}
}


%For set notation \Set{ x \in X \given x > 0 }
\newcommand\SetSymbol[1][]{
	\nonscript\:
	#1\vert
	\allowbreak
	\nonscript\:
	\mathopen{}
}
%\providecommand\given{}

\newcommand\where{\errmessage{The command \noexpand\where was used outside an allowed environment on input line \the\inputlineno.}}

\DeclarePairedDelimiterX\Set[1]{\lbrace}{\rbrace}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\set{\lbrace}{\rbrace}{,}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

% Using the same principles, we define \Gen and \gen for algebraic generation,
% using ⟨⟩ and \Altgen and \altgen using ()

\DeclarePairedDelimiterX\Gen[1]{\langle}{\rangle}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\gen{\langle}{\rangle}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

\DeclarePairedDelimiterX\Vargen[1]{(}{)}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\vargen{(}{)}{,}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

%Two commands \Prob{...} og \Mean{...} for probabilities and means. They support the same command \given as before

\DeclarePairedDelimiterXPP\lgen[2]{}{\langle}{\rangle}{_{#1}}{
	#2
}

\DeclarePairedDelimiterXPP\Lgen[2]{}{\langle}{\rangle}{_{#1}}{
	\renewcommand\given{\SetSymbol[\delimsize]}
	\,#2\, %Note that I added the spaces around the inner part
}

\DeclarePairedDelimiterXPP\Prob[1]{P}(){}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}
\DeclarePairedDelimiterXPP\Mean[1]{\mathbb{E}}[]{}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}


\DeclarePairedDelimiterXPP\pol[2]{#1}{[}{]}{}{ % polynomials
	#2
}

\DeclarePairedDelimiterXPP\rat[2]{#1}{(}{)}{}{ % rational functions
	#2
}

\DeclarePairedDelimiterXPP\fal[2]{#1}{\langle}{\rangle}{}{ % free algebra
	#2
}

\DeclarePairedDelimiter\cl{[}{]} % equivalence classes

\newcommand\varcl{\widebar}

% the commands \pars, for the backwards notation \pars{...}[\big] and \pars{...}*

\DeclarePairedDelimiter{\@parentheses}{(}{)}

\DeclareDocumentCommand\parentheses{mso}
{
	\IfBooleanTF{#2}
	{
		\@parentheses*
	}
	{
		\IfNoValueTF{#3}
		{
			\@parentheses
		}
		{
			\@parentheses[#3]
		}
	}
	{
		#1
	}
}

\newcommand\identity[1]{#1}
\newcommand\pars{}

\ExplSyntaxOn



\cs_set:Npn \pars#1{%
	\tl_if_blank:nTF{ #1 }
	{
		% do nothing
	}
	{
		\str_case:nnTF { #1 }
		{
			{.} {}
			{:} {\identity}
			{*} {\parentheses{\slot}}
			{-} {\parentheses{\slot}}
		}
		{
			% do nothing
		}
		{
			\parentheses{#1}%
		}%
	}
}

\ExplSyntaxOff

==> _commands/delims/_delims_2.tex <==

% \abs{x} for absolute values:
\DeclarePairedDelimiterX\abs[1]\lvert\rvert{
	\slotifempty{#1}
}

\DeclarePairedDelimiterX\size[1]\lvert\rvert{
	\slotifempty{#1}
}

\newcommand\varsize[1]{\#}

% \norm{x} for norms:
\DeclarePairedDelimiterX\norm[1]\lVert\rVert{ %normer
	\slotifempty{#1}
}
% \inner{u}{v} for inner products:
\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{ %indre produkter
	\slotifempty{#1},\slotifempty{#2}
}

\DeclarePairedDelimiterX\com[2]{[}{]}{ %commutator
	\slotifempty{#1},\slotifempty{#2}
}


%For set notation \Set{ x \in X \given x > 0 }
\newcommand\SetSymbol[1][]{
	\nonscript\:
	#1\vert
	\allowbreak
	\nonscript\:
	\mathopen{}
}
%\providecommand\given{}

\newcommand\where{\errmessage{The command \noexpand\where was used outside an allowed environment on input line \the\inputlineno.}}

\DeclarePairedDelimiterX\Set[1]{\lbrace}{\rbrace}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\set{\lbrace}{\rbrace}{,}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

% Using the same principles, we define \Gen and \gen for algebraic generation,
% using ⟨⟩ and \Altgen and \altgen using ()

\DeclarePairedDelimiterX\Gen[1]{\langle}{\rangle}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\gen{\langle}{\rangle}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

\DeclarePairedDelimiterX\Vargen[1]{(}{)}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\vargen{(}{)}{,}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

%Two commands \Prob{...} og \Mean{...} for probabilities and means. They support the same command \given as before

\DeclarePairedDelimiterXPP\lgen[2]{}{\langle}{\rangle}{_{#1}}{
	#2
}

\DeclarePairedDelimiterXPP\Lgen[2]{}{\langle}{\rangle}{_{#1}}{
	\renewcommand\given{\SetSymbol[\delimsize]}
	\,#2\, %Note that I added the spaces around the inner part
}

\DeclarePairedDelimiterXPP\Prob[1]{P}(){}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}
\DeclarePairedDelimiterXPP\Mean[1]{\mathbb{E}}[]{}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}


\DeclarePairedDelimiterXPP\pol[2]{#1}{[}{]}{}{ % polynomials
	#2
}

\DeclarePairedDelimiterXPP\rat[2]{#1}{(}{)}{}{ % rational functions
	#2
}

\DeclarePairedDelimiterXPP\fal[2]{#1}{\langle}{\rangle}{}{ % free algebra
	#2
}

\DeclarePairedDelimiter\cl{[}{]} % equivalence classes

\newcommand\varcl{\widebar}

% the commands \pars, for the backwards notation \pars{...}[\big] and \pars{...}*

\DeclarePairedDelimiter{\@parentheses}{(}{)}

\DeclareDocumentCommand\parentheses{mso}
{
	\IfBooleanTF{#2}
	{
		\@parentheses*
	}
	{
		\IfNoValueTF{#3}
		{
			\@parentheses
		}
		{
			\@parentheses[#3]
		}
	}
	{
		#1
	}
}

\newcommand\identity[1]{#1}
\newcommand\pars{}

\ExplSyntaxOn



\cs_set:Npn \pars#1{%
	\tl_if_blank:nTF{ #1 }
	{
		% do nothing
	}
	{
		\str_case:nnTF { #1 }
		{
			{.} {}
			{:} {\identity}
			{*} {\parentheses{\slot}}
			{-} {\parentheses{\slot}}
		}
		{
			% do nothing
		}
		{
			\parentheses{#1}%
		}%
	}
}

\ExplSyntaxOff

==> _commands/delims/_delims_3.tex <==

%% \abs{x} for absolute values:
%\DeclarePairedDelimiterX\abs[1]\lvert\rvert{
%	\slotifempty{#1}
%}
%
%\DeclarePairedDelimiterX\size[1]\lvert\rvert{
%	\slotifempty{#1}
%}
%
%\newcommand\varsize[1]{\#}
%
%% \norm{x} for norms:
%\DeclarePairedDelimiterX\norm[1]\lVert\rVert{ %normer
%	\slotifempty{#1}
%}
%% \inner{u}{v} for inner products:
%\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{ %indre produkter
%	\slotifempty{#1},\slotifempty{#2}
%}
%
%\DeclarePairedDelimiterX\com[2]{[}{]}{ %commutator
%	\slotifempty{#1},\slotifempty{#2}
%}


%%For set notation \Set{ x \in X \given x > 0 }
%\newcommand\SetSymbol[1][]{
%	\nonscript\:
%	#1\vert
%	\allowbreak
%	\nonscript\:
%	\mathopen{}
%}
%\providecommand\given{}

%\newcommand\where{\errmessage{The command \noexpand\where was used outside an allowed environment on input line \the\inputlineno.}}

\newcommand\where{
	\nonscript\:
	\automathdelimsize\vert
	\allowbreak
	\nonscript\:
	\mathopen{}
}

%\DeclarePairedDelimiterX\Set[1]{\lbrace}{\rbrace}{
%	\renewcommand\where{\SetSymbol[\delimsize]}
%	\,#1\, %Note that I added the spaces around the inner part
%}

\newdelimiterclass{delim}[
	parent=var,
	output=var,
	keyvals={
		{ord}{outputoptions={lower={\keyvalue}}}, % for e.g. the n-norm
	},
]

\newdelim\Set{\lbrace}{\rbrace}[
	keyvals={
		{argdefault}{argnokeyval=\,,argnokeyval=\keyvalue,argnokeyval=\,},
	},
	output=classset,
	]


\newtuple\set{\lbrace}{,}{\rbrace}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

\newdelim\Gen{\langle}{\rangle}[
	keyvals={
		{argdefault}{argnokeyval=\,,argnokeyval=\keyvalue,argnokeyval=\,},
	},
	output=alg,
	]


\newtuple\gen{\langle}{,}{\rangle}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}


\newdelim\Vargen{(}{)}[
	keyvals={
		{argdefault}{argnokeyval=\,,argnokeyval=\keyvalue,argnokeyval=\,},
	},
	output=alg,
	]


\newtuple\vargen{(}{,}{)}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

\newdelim\cl{[}{]} % equivalence classes

\newdelim\abs{\lvert}{\rvert}

\newdelim\norm{\lVert}{\rVert}

% Using the same principles, we define \Gen and \gen for algebraic generation,
% using ⟨⟩ and \Altgen and \altgen using ()


\begin{comment}

\DeclarePairedDelimiterX\Gen[1]{\langle}{\rangle}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\gen{\langle}{\rangle}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

\DeclarePairedDelimiterX\Vargen[1]{(}{)}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\vargen{(}{)}{,}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

%Two commands \Prob{...} og \Mean{...} for probabilities and means. They support the same command \given as before

\DeclarePairedDelimiterXPP\lgen[2]{}{\langle}{\rangle}{_{#1}}{
	#2
}

\DeclarePairedDelimiterXPP\Lgen[2]{}{\langle}{\rangle}{_{#1}}{
	\renewcommand\given{\SetSymbol[\delimsize]}
	\,#2\, %Note that I added the spaces around the inner part
}

\DeclarePairedDelimiterXPP\Prob[1]{P}(){}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}
\DeclarePairedDelimiterXPP\Mean[1]{\mathbb{E}}[]{}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}


\DeclarePairedDelimiterXPP\pol[2]{#1}{[}{]}{}{ % polynomials
	#2
}

\DeclarePairedDelimiterXPP\rat[2]{#1}{(}{)}{}{ % rational functions
	#2
}

\DeclarePairedDelimiterXPP\fal[2]{#1}{\langle}{\rangle}{}{ % free algebra
	#2
}

\DeclarePairedDelimiter\cl{[}{]} % equivalence classes

\newcommand\varcl{\widebar}

% the commands \pars, for the backwards notation \pars{...}[\big] and \pars{...}*

\DeclarePairedDelimiter{\@parentheses}{(}{)}

\DeclareDocumentCommand\parentheses{mso}
{
	\IfBooleanTF{#2}
	{
		\@parentheses*
	}
	{
		\IfNoValueTF{#3}
		{
			\@parentheses
		}
		{
			\@parentheses[#3]
		}
	}
	{
		#1
	}
}

\newcommand\identity[1]{#1}
\newcommand\pars{}

\ExplSyntaxOn



\cs_set:Npn \pars#1{%
	\tl_if_blank:nTF{ #1 }
	{
		% do nothing
	}
	{
		\str_case:nnTF { #1 }
		{
			{.} {}
			{:} {\identity}
			{*} {\parentheses{\slot}}
			{-} {\parentheses{\slot}}
		}
		{
			% do nothing
		}
		{
			\parentheses{#1}%
		}%
	}
}

\ExplSyntaxOff

\end{comment}

==> _commands/derivatives/_derivatives_1.tex <==
\begin{comment}
\NewDocumentCommand\dif{D(){}O{}m}{
	\frac{
		\D(#1){#2}
	}{
		\D{#3}
		\IfNoValueTF{#1}{
			%do nothing
		}{
			^{#1}
		}
	}
}

\NewDocumentCommand\tdif{D(){}O{}m}{
	\tfrac{
		\D(#1){#2}
	}{
		\D{#3}
		\IfNoValueTF{#1}{
			%do nothing
		}{
			^{#1}
		}
	}
}

\newcommand*\cont[2][]{
		\ifblank{#1}{
			C(#2)
		}{
			C^{#1}(#2)
		}
	}
\newcommand*\continto[3][]{
	\ifblank{#1}{
		C(#2,#3)
	}{
	C^{#1}(#2,#3)
}
}
\end{comment}

==> _commands/homology/_homology_1.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn { #1 }
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1  {\_homology_parentheses:w{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_big:n #1  {\_homology_parentheses:w[\big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Big:n #1  {\_homology_parentheses:w[\Big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_bigg:n #1  {\_homology_parentheses:w[\bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Bigg:n #1  {\_homology_parentheses:w[\Bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_auto:n #1  {\_homology_parentheses:w*{\_homology_interpret:n{#1}}}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
					%\use:c { _homology_#1_index_go_auto: }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
					%\use:c{ _homology_#1_index_go_auto: }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			%\use:c { _homology_#1_index_go_auto: }
			\tl_put_right:cn { _homology_#1_main_index } { #3 }
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			%\use:c { _homology_#1_index_go_auto: }
			\tl_put_right:cx { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ \big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { * }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { ** }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	%\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }		
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			\use:c { _homology_#1_keys_set:n } { main={#3} }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
	%\group_end:

	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo
		\group_begin:
			\exp_args:Nv
			\_homology_upper_index:n
			{
				_homology_#1_main_index
			}
			%\exp_args:NNNo\exp_args:NNo
			\exp_args:Nv
			\_homology_lower_index:n
			{
				_homology_#1_second_index
			}
		\group_end:
	}
	{
		\group_begin:
			\exp_args:Nv\_homology_upper_index:n
			{
				\group
				_homology_#1_second_index
			}
			\exp_args:Nv\_homology_lower_index:n
			{
				_homology_#1_main_index
			}
		\group_end:
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##3 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ sheaf, indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ sheaf, indextype=upper} { #2 } { #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}




\newcomplex\dif{d}
\newcomplex\pdif{\partial}
\newcomplex\ddif{\delta}

\newsimplex\face{d}
\newsimplex\pface{\partial}
\newsimplex\dface{\delta}


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\ExplSyntaxOff


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/homology/_homology_1000.tex <==
\newcohomologyclass{cohomology}[
	parent=var,
	gradingpos=upper,
	keyvals={
		{shift}{ symbolputright={[\keyvalue]} },
	},
	singlekeys={
		{cech}{ command=\noexpand\check },
		%{cech} { command=\check },
		{hyper}{ command=\mathbb },
	},
	argkeyvals={
		{cover}{ {\keyvalue} },
		{coef}{sep={;}{\keyvalue}},
		{c}{sep={;}{\keyvalue}},
	},
]


\newmapclass{homset}[
	parent=cohomology,
]

\newcomplexclass{complex}[
	parent=cohomology,
]

\newcohomologyclass{homology}[
	parent=cohomology,
	gradingpos=lower,
]


\newcomplexclass{simplex}[
	parent=cohomology,
	gradingpos=lower,
]


\newhomset{\Hom}{\operatorname{Hom}}
\newhomset{\Ext}{\operatorname{Ext}}
\newhomset{\Map}{\operatorname{Map}}

%\newcohomology{homp}{\operatorname{Hom}}
%\let\Hom=\Hompre

%\let\hom=\homp
%\let\Hom=\homp

%\DeclareMathOperator\Extproto{Ext}

%\newcohomology{\ext}{\Extproto}

%\let\Ext=\ext

%\newhomset{\extone}{\Extproto}

\newcomplex\comX{X}
\newcomplex{\comY}{Y}
\newcomplex{\comZ}{Z}
\newcomplex{\comM}{M}
\newcomplex{\comN}{N}
\newcomplex{\comP}{P}
\newcomplex{\comQ}{Q}
\newcomplex{\comI}{I}
\newcomplex{\comJ}{J}
\newcomplex{\comA}{A}
\newcomplex{\comB}{B}
\newcomplex{\comC}{C}
\newcomplex{\comD}{D}
\newcomplex{\comE}{E}
\newcomplex{\comF}{F}
%\end{comment}

%\newcohomology\co{H}
%\newhomology\ho{H}
%
%\newcohomology\coch{C}
%\newhomology\hoch{C}
%
%\newcohomology\cocy{Z}
%\newhomology\hocy{Z}
%
%\newcohomology\coby{B}
%\newhomology\hoby{B}

\begin{comment}

\end{comment}

\ExplSyntaxOn
\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\exp_args:Nc\newcohomology{#1co}{#2}
	\exp_args:Nc\newhomology{#1ho}{#2}[parent=#1co]
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\exp_args:Nc\newhomology{#1hoch}{#3}[parent=#1co]
	\exp_args:Nc\newcohomology{#1coch}{#3}[parent=#1co]
	\exp_args:Nc\newhomology{#1hocy}{#4}[parent=#1co]
	\exp_args:Nc\newcohomology{#1cocy}{#4}[parent=#1co]
	\exp_args:Nc\newhomology{#1hobo}{#5}[parent=#1co]
	\exp_args:Nc\newcohomology{#1cobo}{#5}[parent=#1co]
}
\ExplSyntaxOff


\newhomologytheory{}{H}{C}{Z}{B}

\newhomologytheory{sh}{\mathscr{H}}{\mathscr{C}}{\mathscr{Z}}{\mathscr{B}}

\setupobject\shco{output=sheaf}


\newcohomologyclass{derivedfunctor}[parent=cohomology,nopar,output=map]
\newderivedfunctor\Lder{L}
\newderivedfunctor\Rder{R}




\newcohomology\exterior{\Lambdaup}[upper=\!\!]



\newcohomology\Bar{\operatorname{Bar}}

\newcohomology\Cob{\operatorname{Cob}}

==> _commands/homology/_homology_2.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn { #1 }
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1  {\_homology_parentheses:w{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_big:n #1  {\_homology_parentheses:w[\big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Big:n #1  {\_homology_parentheses:w[\Big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_bigg:n #1  {\_homology_parentheses:w[\bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Bigg:n #1  {\_homology_parentheses:w[\Bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_auto:n #1  {\_homology_parentheses:w*{\_homology_interpret:n{#1}}}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
					%\use:c { _homology_#1_index_go_auto: }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
					%\use:c{ _homology_#1_index_go_auto: }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			%\use:c { _homology_#1_index_go_auto: }
			\tl_put_right:cn { _homology_#1_main_index } { #3 }
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			%\use:c { _homology_#1_index_go_auto: }
			\tl_put_right:cn { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ \big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { * }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { ** }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\bool_new:c { _homology_#1_if_upper_index }
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\str_new:N \_homology_par_size_temp

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }		
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			\use:c { _homology_#1_keys_set:n } { main={#3} }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
	%\group_end:
		\tl_gset:Nv\_homology_main_index_temp { _homology_#1_main_index }
		\tl_gset:Nv\_homology_second_index_temp { _homology_#1_second_index }
		\str_gset_eq:Nc\_homology_par_size_temp { _homology_#1_par_size }
	\group_end:
	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo

			\exp_args:NV \_homology_upper_index:n \_homology_main_index_temp
			\exp_args:NV \_homology_lower_index:n \_homology_second_index_temp
	}
	{
			\exp_args:NV \_homology_lower_index:n \_homology_main_index_temp
			\exp_args:NV \_homology_upper_index:n \_homology_second_index_temp
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:No
				\_homology_parentheses:nn { \_homology_par_size_temp } { ##3 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ sheaf, indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ sheaf, indextype=upper} { #2 } { #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}




%\newcomplex\dif{d}
%\newcomplex\pdif{\partial}
%\newcomplex\ddif{\delta}

%\newsimplex\face{d}
%\newsimplex\pface{\partial}
%\newsimplex\dface{\delta}


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\ExplSyntaxOff


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/homology/_homology_3.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn { #1 }
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


%\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1  {\_homology_parentheses:w{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_big:n #1  {\_homology_parentheses:w[\big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Big:n #1  {\_homology_parentheses:w[\Big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_bigg:n #1  {\_homology_parentheses:w[\bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Bigg:n #1  {\_homology_parentheses:w[\Bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_auto:n #1  {\_homology_parentheses:w*{\_homology_interpret:n{#1}}}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			\tl_put_right:cn { _homology_#1_main_index } { #3 }
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			\tl_put_right:cn { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ \big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { * }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { ** }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\bool_new:c { _homology_#1_if_upper_index }
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\newcommand\homologysetup[2]{
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\str_new:N \_homology_par_size_temp

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }		
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			%\use:c { _homology_#1_keys_set:n } { main={#3} }
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
		\tl_gset:Nv\_homology_main_index_temp { _homology_#1_main_index }
		\tl_gset:Nv\_homology_second_index_temp { _homology_#1_second_index }
		\str_gset_eq:Nc\_homology_par_size_temp { _homology_#1_par_size }
	\group_end:
	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo
		\exp_args:NV \_homology_upper_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_lower_index:n \_homology_second_index_temp
	}
	{
		\exp_args:NV \_homology_lower_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_upper_index:n \_homology_second_index_temp
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \co
	% #2 = name without backshash, e.g. co
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:No
				\_homology_parentheses:nn { \_homology_par_size_temp } { ##3 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=lower, #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \hom
	% #2 = name without backshash, e.g. hom
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower, #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
				\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper, #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \comX
	% #2 = name without backshash, e.g. comX
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper , #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx \_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower , #3 }%
	}
}




%\newcomplex\dif{d}
%\newcomplex\pdif{\partial}
%\newcomplex\ddif{\delta}

%\newsimplex\face{d}
%\newsimplex\pface{\partial}
%\newsimplex\dface{\delta}

\ExplSyntaxOff


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\newcomplex\comX{X}
\newcomplex\comY{Y}
\newcomplex\comZ{Z}
\newcomplex\comM{M}
\newcomplex\comN{N}
\newcomplex\comP{P}
\newcomplex\comQ{Q}
\newcomplex\comI{I}
\newcomplex\comJ{J}
\newcomplex\comA{A}
\newcomplex\comB{B}
\newcomplex\comC{C}
\newcomplex\comD{D}
\newcomplex\comE{E}
\newcomplex\comF{F}


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/homology/_homology_4.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn {{{ #1 }}}%
			% the two extra braces are necessary because \keyval_parse:NNn seems to expand its input twice
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


%\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1
{
	(
		\_homology_interpret:n{#1}
	)
}

\cs_new:Npn \_homology_parentheses_big:n #1
{
	\big(
		\_homology_interpret:n{#1}
	\big)
}

\cs_new:Npn \_homology_parentheses_Big:n #1
{
	\Big(
		\_homology_interpret:n{#1}
	\Big)
}

\cs_new:Npn \_homology_parentheses_bigg:n #1
{
	\bigg(
		\_homology_interpret:n{#1}
	\bigg)
}

\cs_new:Npn \_homology_parentheses_Bigg:n #1
{
	\Bigg(
		\_homology_interpret:n{#1}
	\Bigg)
}

\cs_new:Npn \_homology_parentheses_auto:n #1
{
	\left(
		\_homology_interpret:n{#1}
	\right)
}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			\tl_put_right:cn { _homology_#1_main_index } { #3 }
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			\tl_put_right:cn { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ \big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { * }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { ** }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\bool_new:c { _homology_#1_if_upper_index }
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\newcommand\homologysetup[2]{
	%\exp_args:Nx
	\use:c { _homology_\cs_to_str:N#1_keys_set:n } {
		#2
	}
}

\str_new:N \_homology_par_size_temp

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }		
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			%\use:c { _homology_#1_keys_set:n } { main={#3} }
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
		\tl_gset:Nv\_homology_main_index_temp { _homology_#1_main_index }
		\tl_gset:Nv\_homology_second_index_temp { _homology_#1_second_index }
		\str_gset_eq:Nc\_homology_par_size_temp { _homology_#1_par_size }
	\group_end:
	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo
		\exp_args:NV \_homology_upper_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_lower_index:n \_homology_second_index_temp
	}
	{
		\exp_args:NV \_homology_lower_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_upper_index:n \_homology_second_index_temp
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \co
	% #2 = name without backshash, e.g. co
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:No
				\_homology_parentheses:nn { \_homology_par_size_temp } { ##3 }
			}%
		\group_end:		
	}
}

%\DeclareDocumentCommand{\homologysetup}{argspec}{code}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=lower, #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \hom
	% #2 = name without backshash, e.g. hom
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower, #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper, #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \comX
	% #2 = name without backshash, e.g. comX
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper , #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower , #3 }%
	}
}




%\newcomplex\dif{d}
%\newcomplex\pdif{\partial}
%\newcomplex\ddif{\delta}

%\newsimplex\face{d}
%\newsimplex\pface{\partial}
%\newsimplex\dface{\delta}

\ExplSyntaxOff


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\newcomplex\comX{X}
\newcomplex\comY{Y}
\newcomplex\comZ{Z}
\newcomplex\comM{M}
\newcomplex\comN{N}
\newcomplex\comP{P}
\newcomplex\comQ{Q}
\newcomplex\comI{I}
\newcomplex\comJ{J}
\newcomplex\comA{A}
\newcomplex\comB{B}
\newcomplex\comC{C}
\newcomplex\comD{D}
\newcomplex\comE{E}
\newcomplex\comF{F}


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/homology/_homology_5.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn {{{ #1 }}}%
			% the two extra braces are necessary because \keyval_parse:NNn seems to expand its input twice
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


%\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1
{
	(
		\_homology_interpret:n{#1}
	)
}

\cs_new:Npn \_homology_parentheses_big:n #1
{
	\big(
		\_homology_interpret:n{#1}
	\big)
}

\cs_new:Npn \_homology_parentheses_Big:n #1
{
	\Big(
		\_homology_interpret:n{#1}
	\Big)
}

\cs_new:Npn \_homology_parentheses_bigg:n #1
{
	\bigg(
		\_homology_interpret:n{#1}
	\bigg)
}

\cs_new:Npn \_homology_parentheses_Bigg:n #1
{
	\Bigg(
		\_homology_interpret:n{#1}
	\Bigg)
}

\cs_new:Npn \_homology_parentheses_auto:n #1
{
	\left(
		\_homology_interpret:n{#1}
	\right)
}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			\tl_put_right:cn { _homology_#1_main_index } { #3 }
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			\tl_put_right:cn { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ \big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { * }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { ** }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\bool_new:c { _homology_#1_if_upper_index }
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\newcommand\homologysetup[2]{
	%\exp_args:Nx
	\use:c { _homology_\cs_to_str:N#1_keys_set:n } {
		#2
	}
}

\str_new:N \_homology_par_size_temp

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			%\use:c { _homology_#1_keys_set:n } { main={#3} }
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
		\tl_gset:Nv\_homology_main_index_temp { _homology_#1_main_index }
		\tl_gset:Nv\_homology_second_index_temp { _homology_#1_second_index }
		\str_gset_eq:Nc\_homology_par_size_temp { _homology_#1_par_size }
	\group_end:
	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo
		\exp_args:NV \_homology_upper_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_lower_index:n \_homology_second_index_temp
	}
	{
		\exp_args:NV \_homology_lower_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_upper_index:n \_homology_second_index_temp
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \co
	% #2 = name without backshash, e.g. co
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:No
				\_homology_parentheses:nn { \_homology_par_size_temp } { ##3 }
			}%
		\group_end:		
	}
}

%\DeclareDocumentCommand{\homologysetup}{argspec}{code}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=lower, #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \hom
	% #2 = name without backshash, e.g. hom
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower, #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper, #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \comX
	% #2 = name without backshash, e.g. comX
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper , #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower , #3 }%
	}
}




%\newcomplex\dif{d}
%\newcomplex\pdif{\partial}
%\newcomplex\ddif{\delta}

%\newsimplex\face{d}
%\newsimplex\pface{\partial}
%\newsimplex\dface{\delta}

\ExplSyntaxOff


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\newcomplex\comX{X}
\newcomplex\comY{Y}
\newcomplex\comZ{Z}
\newcomplex\comM{M}
\newcomplex\comN{N}
\newcomplex\comP{P}
\newcomplex\comQ{Q}
\newcomplex\comI{I}
\newcomplex\comJ{J}
\newcomplex\comA{A}
\newcomplex\comB{B}
\newcomplex\comC{C}
\newcomplex\comD{D}
\newcomplex\comE{E}
\newcomplex\comF{F}


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/homology/_homology_6.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn {{{ #1 }}}%
			% the two extra braces are necessary because \keyval_parse:NNn seems to expand its input twice
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


%\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1
{
	(
		\_homology_interpret:n{#1}
	)
}

\cs_new:Npn \_homology_parentheses_big:n #1
{
	\big(
		\_homology_interpret:n{#1}
	\big)
}

\cs_new:Npn \_homology_parentheses_Big:n #1
{
	\Big(
		\_homology_interpret:n{#1}
	\Big)
}

\cs_new:Npn \_homology_parentheses_bigg:n #1
{
	\bigg(
		\_homology_interpret:n{#1}
	\bigg)
}

\cs_new:Npn \_homology_parentheses_Bigg:n #1
{
	\Bigg(
		\_homology_interpret:n{#1}
	\Bigg)
}

\cs_new:Npn \_homology_parentheses_auto:n #1
{
	\left(
		\_homology_interpret:n{#1}
	\right)
}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
				%#1
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
				%#1
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			\tl_put_right:co { _homology_#1_main_index } { #3 } 
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			\tl_put_right:cn { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_bullet: }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { \_homology_double_bullet: }}
		{ indexbullet } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_bullet: }}
		{ indexdoublebullet }{ \_homology_keyval:nnn { #1 } { addsecond } { \_homology_double_bullet: }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\bool_new:c { _homology_#1_if_upper_index }
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\newcommand\homologysetup[2]{
	%\exp_args:Nx
	\use:c { _homology_\cs_to_str:N#1_keys_set:n } {
		#2
	}
}

\str_new:N \_homology_par_size_temp

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			%\use:c { _homology_#1_keys_set:n } { main={#3} }
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
			%\exp_args:Nnno\_homology_keyval:nnn { #1 } { addmain } { \_homology_bullet_if_bar:n { #3 } }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
		\tl_gset:Nv\_homology_main_index_temp { _homology_#1_main_index }
		\tl_gset:Nv\_homology_second_index_temp { _homology_#1_second_index }
		\str_gset_eq:Nc\_homology_par_size_temp { _homology_#1_par_size }
	\group_end:
	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo
		\exp_args:NV \_homology_upper_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_lower_index:n \_homology_second_index_temp
	}
	{
		\exp_args:NV \_homology_lower_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_upper_index:n \_homology_second_index_temp
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \co
	% #2 = name without backshash, e.g. co
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:No
				\_homology_parentheses:nn { \_homology_par_size_temp } { ##3 }
			}%
		\group_end:		
	}
}

%\DeclareDocumentCommand{\homologysetup}{argspec}{code}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=lower, #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \hom
	% #2 = name without backshash, e.g. hom
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower, #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper, #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \comX
	% #2 = name without backshash, e.g. comX
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper , #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower , #3 }%
	}
}




%\newcomplex\dif{d}
%\newcomplex\pdif{\partial}
%\newcomplex\ddif{\delta}

%\newsimplex\face{d}
%\newsimplex\pface{\partial}
%\newsimplex\dface{\delta}

\ExplSyntaxOff


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\newcomplex\comX{X}
\newcomplex\comY{Y}
\newcomplex\comZ{Z}
\newcomplex\comM{M}
\newcomplex\comN{N}
\newcomplex\comP{P}
\newcomplex\comQ{Q}
\newcomplex\comI{I}
\newcomplex\comJ{J}
\newcomplex\comA{A}
\newcomplex\comB{B}
\newcomplex\comC{C}
\newcomplex\comD{D}
\newcomplex\comE{E}
\newcomplex\comF{F}


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/index/_index_1.tex <==
\DeclareDocumentCommand\textdef{som}{% for inline text definitions
	\IfBooleanTF{#1}{%
		\textbf{#3}%
	}{%
	\IfNoValueTF{#2}%
	{%
		\index{#3}%
	}%
	{%
		\index{#2}%
	}%
	\textbf{#3}%
}%
}

==> _commands/intervals/_intervals_1.tex <==
% Commands for intervals


\ifbourbakiintervals
	\newcommand\open\bouropen
	\newcommand\openpm\bouropenpm
	\newcommand\ropen\bourropen
	\newcommand\ropenpm\bourropenpm
	\newcommand\lopen\bourlopen
	\newcommand\lopenpm\bourlopenpm
	\newcommand\closed\bourclosed
	\newcommand\closedpm\bourclosedpm
\else
	\newcommand\open\tradopen
	\newcommand\openpm\tradopenpm
	\newcommand\ropen\tradropen
	\newcommand\ropenpm\tradropenpm
	\newcommand\lopen\tradlopen
	\newcommand\lopenpm\tradlopenpm
	\newcommand\closed\tradclosed
	\newcommand\closedpm\tradclosedpm
\fi

%Traditional notation:

\DeclarePairedDelimiterX\tradopen[2]
	()
	{#1,#2}
\DeclarePairedDelimiterX\tradopenpm[1]
	()
	{-#1,#1}
\DeclarePairedDelimiterX\tradlopen[2]
	(]
	{#1,#2}
\DeclarePairedDelimiterX\tradlopenpm[1]
	(]
	{-#1,#1}
\DeclarePairedDelimiterX\tradropen[2]
	[)
	{#1,#2}
\DeclarePairedDelimiterX\tradropenpm[1]
	[)
	{-#1,#1}
\DeclarePairedDelimiterX\tradclosed[2]
	[]
	{#1,#2}
\DeclarePairedDelimiterX\tradclosedpm[1]
	[]
	{-#1,#1}

% Bourbaki notation:
\DeclarePairedDelimiterX\bouropen[2]
	][ 
	{#1,#2}
\DeclarePairedDelimiterX\bouropenpm[1]
	][
	{-#1,#1}
\DeclarePairedDelimiterX\bourlopen[2]
	]]
	{#1,#2}
\DeclarePairedDelimiterX\bourlopenpm[1]
	]]
	{-#1,#1}
\DeclarePairedDelimiterX\bourropen[2]
	[[
	{#1,#2}
\DeclarePairedDelimiterX\bourropenpm[1]
	[[
	{-#1,#1}
\DeclarePairedDelimiterX\bourclosed[2]
	[]
	{#1,#2}
\DeclarePairedDelimiterX\bourclosedpm[1]
	[]
	{-#1,#1}

==> _commands/lie/_lie_1.tex <==
%Lie stuff:

\newcommand\lieg{\mathfrak{g}}
\newcommand\lieh{\mathfrak{h}}
\newcommand\liegl{\mathfrak{gl}}
\newcommand\liesl{\mathfrak{sl}}
\newcommand\liesu{\mathfrak{su}}
\newcommand\lieso{\mathfrak{so}}

\let\g=\lieg
\let\h=\lieh

==> _commands/maps/maps_11.tex <==
\newmapclass{map}[
	parent=var,
	output=var,
	singlekeys={
		{invim} { upper = -1, nopar, output=sheaf },
		{dirim} { lower={\ast}, nopar, output=sheaf },
		{pull} { upper={\ast} },
		{push}{ lower = {\ast} },
		{shpull}{ upper={\ast}, nopar, output=sheaf },
		{shpush}{ lower={\ast}, nopar, output=sheaf },
		{shriekpush} { lower=!, nopar, output=sheaf },
		{shriekpull} { upper=!, nopar, output=sheaf },
		{!push} { lower=!, nopar, output=sheaf },
		{!pull} { upper=!, nopar, output=sheaf },
		{sharp} { upper=\# },
		{inv} { upper=-1 },
		{pre} { upper=-1 },
%		{shpull} { g=-1 },
		{squared} { upper=2 },
	},
	keyvals={
		{der} { upper = {(\keyvalue)} },
		{res} { return, symbolputright=\vert, lower={\keyvalue} },
		{res} { return, symbolputright=\vert, lower={\keyvalue} },
		{bigres} { return, symbolputright=\big\vert, lower={\keyvalue} },
		{Bigres} { return, symbolputright=\Big\vert, lower={\keyvalue} },
		{biggres} { return, symbolputright=\bigg\vert, lower={\keyvalue} },
		{Biggres} { return, symbolputright=\Bigg\vert, lower={\keyvalue} },
		% Derived functors:
		{Lder} { symbolputleft=L^{\keyvalue}},
		{Rder} { symbolputleft=R^{\keyvalue}},
	},
]

\newmap{\mf}{f}
\newmap{\mg}{g}{}
\newmap{\mh}{h}{}
\newmap{\mphi}{\phi}
\newmap{\mvarphi}{\varphi}
\newmap{\mpsi}{\psi}
\newmap{\mF}{F}
\newmap{\mG}{G}
\newmap{\mH}{H}
\newmap{\mPhi}{\Phi}
\newmap{\mPsi}{\Psi}

\newmap{\dif}{d}[nopar]
\newmap{\pdif}{\partial}[nopar]
\newmap{\ddif}{\delta}[nopar]

%\newmap{\face}{d}[gradingpos=lower,nopar]
%\newmap{\pface}{\partial}[gradingpos=lower,nopar]
%\newmap{\dface}{\delta}[gradingpos=lower,nopar]


%\newcommand\idproto{\mathupright{id}}

\newmap{\id}{\mathup{id}}
\newmap{\bigid}{\mathup{Id}}



\newmap{\Span}{\operatorname{span}}
\newmap{\Ker}{\operatorname{Ker}}
\newmap{\Image}{\operatorname{Im}}
\newmap{\Coker}{\operatorname{Coker}}
\newmap{\Realpart}{\operatorname{Re}}

%\renewcommand*\Im{\operatorname{Im}}
%\renewcommand*\Re{\operatorname{Re}}
\let\Im=\Image
\let\Re=\Realpart

\let\ker=\Ker
\let\coker=\Coker
\let\im=\Im
\let\Id=\id

%\newmap{\End}{\operatorname{End}} % moved to homology
%\newmap{\Hom}{\operatorname{Hom}}
\newmap{\GL}{\operatorname{GL}}
\newmap{\SL}{\operatorname{SL}}
\newmap{\SU}{\operatorname{SU}}
\newmap{\SO}{\operatorname{SO}}
\newmap{\Sym}{\operatorname{Sym}}
\newmap{\Aut}{\operatorname{Aut}}
%\newmap{\Mor}{\operatorname{Mor}
%\newmap{\Fun{Fun}
%\newmap{\Ext{Ext}
%\newmap{\Tor{Tor}

\newmapclass{algop}[
	parent=map,
	output=alg,
	nopar,
]

\newmapclass{algoplaurent}[
	parent=algop,
	par,
	leftpar=(,rightpar=),
	keyvals={
		{arg}{
			argwithoutkeyval={\!\noexpand\automathdelimsize(},
			argwithkeyval={\keyvalue},
			argwithoutkeyval={\noexpand\automathdelimsize)\!},
		},
	},
]

\newmapclass{algopfreealg}[
	parent=algop,
	par,
	leftpar=\langle,rightpar=\rangle,
]

\newmapclass{algoppowerseries}[
	parent=algop,
	par,
	leftpar=\llbracket,rightpar=\rrbracket,
]

\newalgop{\catend}{\int}

\newalgop{\catcoend}{\int}[gradingpos=lower]

\newalgop\Sum{\sum}[
	keyvals={
		{from}{lower={\keyvalue}},
		{to}{upper={\keyvalue}},
	},
]

\newalgop\Int{\int}[parent=Sum]

\newmapclass{calculusdifferential}[
	parent=map,
	argkeyvals={
		{default}{standardsep={d\!\keyvalue}},
	},
	argsep={\,},
	argdots={\cdots},
	ifpar=false,
]

\newcalculusdifferential\intD{}[iffirstarg=false]

\newcalculusdifferential\wedgeD{}[argsep={\wedge}]

==> _commands/operators/operators_1.tex <==
\newvariableclass{automathoperator}[
	parent=var,
	singlekeys={
		{der}{upper=L},
		{bbder}{upper={\noexpand\mathbb{L}}},
		{bder}{upper={\noexpand\mathbf{L}}},
	},
]

\newautomathoperator\tens{\otimes}

\newautomathoperator\fibre{\times}
\newautomathoperator\bigfibre{\amalg}

==> _commands/page/_page_1.tex <==
\newcommand*\mybreak{%for nice breaks in the middle of the text
	\fancybreak{\mbox{}\\*$*\quad *\quad *$\\*\mbox{}}%
}

\NewDocumentCommand\exc{sm}{ % for answers of exercises with the exercise number in the margin
	\IfBooleanTF{#1}{%
		%do nothing
	}{%
	\fancybreak{}%
}\noindent\mbox{}\llap{(#2)\quad}\ignorespaces}

==> _commands/slots/_slots_1.tex <==
\newcommand\slot{\mathord{-}} % for expresseions like \Hom(A,\slot);
								% can be changed to \:\cdot\:

\newcommand\slotifempty[1]{
	\ifblank{#1}{\slot}{#1}
}
\newcommand\bulletifempty[1]{
	\ifblank{#1}{\smallbullet}{#1}
}

==> _commands/smalloperators/_smalloperators_1.tex <==
\newcommand\@sotimes[1]{\vcenter{\hbox{$#1\otimes$}}}

\newcommand{\sotimes}{\mathbin{\mathchoice
  {\@sotimes\scriptstyle}
  {\@sotimes\scriptstyle}
  {\@sotimes\scriptscriptstyle}
  {\@sotimes\scriptscriptstyle}
}}

\newcommand\@soplus[1]{\vcenter{\hbox{$#1\oplus$}}}

\newcommand{\soplus}{\mathbin{\mathchoice
  {\@soplus\scriptstyle}
  {\@soplus\scriptstyle}
  {\@soplus\scriptscriptstyle}
  {\@soplus\scriptscriptstyle}
}}

\newcommand\@stimes[1]{\vcenter{\hbox{$#1\times$}}}

\newcommand{\stimes}{\mathbin{\mathchoice
  {\@stimes\scriptstyle}
  {\@stimes\scriptstyle}
  {\@stimes\scriptscriptstyle}
  {\@stimes\scriptscriptstyle}
}}

\newcommand\@scirc[1]{\vcenter{\hbox{$#1\circ$}}}

\newcommand{\scirc}{\mathbin{\mathchoice
  {\@scirc\scriptstyle}
  {\@scirc\scriptstyle}
  {\@scirc\scriptscriptstyle}
  {\@scirc\scriptscriptstyle}
}}

\begin{comment}

\newcommand\sotimes{\mathbin{\raisebox{0.14ex}{\scalebox{.7}{$\otimes$}}}}
\newcommand\soplus{\mathbin{\raisebox{0.14ex}{\scalebox{.7}{$\oplus$}}}}
\newcommand\stimes{\mathbin{\raisebox{0.14ex}{\scalebox{.7}{$\times$}}}}

\end{comment}

==> _commands/tuples/_tuples_1.tex <==
% The below code defines the macro \newflextuple for defining
% what I call "flextuples", tuple commands that automate
% the typesetting of tuple-like environments. They
% have customizable left and right delimiters, separators
% (i.e. comma for a standard tuple), and dot commands
% (a command that is inserted at all occurrences of "...")
% The flextuples are comma-separated on the syntax level

\ExplSyntaxOn

\clist_new:N \flexsequence_input:
\bool_new:N\flexsequence_if_first:
\cs_new:Npn \flexsequence #1#2#3
{
	% #1 = seperator
	% #2 = "..." replacement
	% #3 = contents
    \group_begin:
	\clist_set:Nn \flexsequence_input: {#3}
	\bool_set_true:N \flexsequence_if_first:
	\clist_map_variable:NNn \flexsequence_input: \flexsequence_var:
	{
		\bool_if:NTF \flexsequence_if_first:
		{
			% do nothing
			\bool_set_false:N\flexsequence_if_first:
		}
		{
			#1
		}
		\str_if_eq:onTF {\flexsequence_var:} {...}
		{
			#2
		}
		{
			\flexsequence_var:
		}
	}
	\group_end:
}

\cs_new:Npn \newflexsequence #1#2#3#4
{
	\newcommand#1[1]{\flexsequence{#2}{#3}{##1}}
}

\cs_new:Npn \newflextuple #1#2#3#4#5
{
	% #1 = name
	% #2 = left delimiter
	% #3 = right delimiter
	% #4 = seperator
	% #5 = "..." replacement
	\cs_new:cpn {\cs_to_str:N #1_process } ##1
	{
		\flexsequence{#4}{#5}{##1}
	}
	\DeclarePairedDelimiterX#1[1]{#2}{#3}{
		\use:c {\cs_to_str:N #1_process } {##1}
	}
}

\ExplSyntaxOff


\newcommand\midsequence[2]{\flexsequence{#1}{\cdots}{#2}}


\newflextuple\tup{(}{)}{,}{\ldots}

==> _commands/tuples/_tuples_2.tex <==
\newtupleclass{tuple}[parent=var,output=var]


\newtuple\tup{(}{,}{)}{\ldots}
\newtuple\pcoor{[}{\mathpunct{:}}{]}{\cdots}

==> _commands/widebar/_widebar_1.tex <==
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}

%\makeatletter
%\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%\newcommand*\widebar[1]{%
%  \begingroup
%  \def\mathaccent##1##2{%
%    \rel@kern{0.8}%
%    \overline{\rel@kern{-0.8}\macc@nucleus\rel@kern{0.2}}%
%    \rel@kern{-0.2}%
%  }%
%  \macc@depth\@ne
%  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
%  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
%  \macc@set@skewchar\relax
%  \let\mathaccentV\macc@nested@a
%  \macc@nested@a\relax111{#1}%
%  \endgroup
%}

==> _commands/wraptext/_wraptext_1.tex <==
\def\putright#1#2{\vskip\parskip
   \hbox to\hsize{\hss
      \vbox to0pt{\kern#1\baselineskip\kern-.8\baselineskip \hbox{#2}\vss}}
   \nobreak\vskip-\parskip\vskip-\baselineskip
} % for wrapping text around figures

==> _preamble/beamertheorems/_beamertheorems_11.tex <==
%\newtheorem{theorem}{Theorem}

\newtheorem{proposition}{Proposition}

==> _preamble/index/_index_1.tex <==
\makeindex


==> _preamble/memoir/_memoir_1.tex <==
%Setup of memoir:
\pagestyle{plain} %change to heading for running headings
\nouppercaseheads %running heads should not be capitalized
\captionnamefont{\small} %captions with small font
\captiontitlefont{\small}
\makeevenhead{headings}{\thepage}{}{\itshape\leftmark} %make headings italic instead of slanted
\makeoddhead{headings}{\itshape\rightmark}{}{\thepage}

\raggedbottomsectiontrue%less harse than \raggedbottom
%\allowdisplaybreaks %long equations may break

==> _preamble/ntheorem/_ntheorem_1.tex <==
%Theorem environments:
\usepackage[thmmarks,amsmath]{ntheorem}

% ntheorem configuration:

\input{_preamble/ntheorem/ntheorem_config/_ntheorem_config_1}



\ifdanish
	\input{_preamble/ntheorem/da/_ntheorem_da_1.tex}
\else
	\input{_preamble/ntheorem/en/_ntheorem_en_1.tex}
\fi

==> _preamble/siunitx/_siunitx_1.tex <==
\usepackage{siunitx}

%Setup of siunitx
\sisetup{
	exponent-product=\cdot,	% uses \cdot (·) as multiplication sign
							% instead \times (×)
	group-separator={\,}, 	% adds spaces after each three digits
	output-decimal-marker={.},
							% decimal marker set to point
	per-mode=symbol, 		% for e.g. m/s instead of \frac{m}{s}
}

==> _preamble/varioref/_varioref_1.tex <==
% Provides the \vref command, for writing e.g. "Chapter~5 on page~123"
\usepackage{varioref}

==> category/category_1.tex <==
\begingroup

\chapter{Tools from general category theory}

We include here some notions and tools from general category theory which we shall make use of in the main body of the text.

\section{Ends and coends}

Let \( \catGamma \) and~\( \catC \) be categories and~\( \mH \colon \catGamma[op] \times \catGamma \to \catC \) a bifunctor. The \textdef{end} of~\( \mH \) is an object
\[
	\End[\catGamma] { \mH } = \End[\vgamma \in \catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\( \catC \), together with morphisms~\(
	%\mvarphi[\vgamma] \colon
	\End[\catGamma] { \mH }
	\to
	\mH { \vgamma , \vgamma }
\) for all~\( \vgamma \in \catGamma \), such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \) the lower right square of the following diagram commutes:
\[\begin{tikzcd}
	A \ar[rd,dashed] \ar[rrd, bend left] \ar[ddr, bend right]
\\[-1em]
	&[-2em]	\End[\catGamma] { \mH } \ar[r] \ar[d]
			& \mH { \vgamma , \vgamma } \ar[d, "\mH { \vgamma , \mf }"]
\\
	&	\mH { \vgamma[prime] , \vgamma[prime] } \ar[r, "\mH { \mf , \vgamma[prime] }"']
			& \mH { \vgamma , \vgamma[prime] }
			\invdot
\end{tikzcd}\]
Furthermore, \( \End[\catGamma] { \mH} \)~is universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( A \to \mH { \vgamma , \vgamma } \) for all~\( \vgamma \), subject to the same commutativity conditions, then these factor through a unique map~\( A\to \End[\catGamma] { \mH } \).
If \( \catC \)~is complete, then clearly
\begin{equation}\label{eq:Equalizer_formula_for_end}
	\End[\catGamma]{ H }
	=
	\Eq[par=\Big] {
		\Prod[ \vgamma \in \catGamma ] { \mH { \vgamma , \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{\mf \colon \vgamma \to \vgamma[prime] } ] { \mH { \vgamma , \vgamma[prime] } }
	}.
\end{equation}
Here, the second product runs over all morphisms~\( \mf \colon \vgamma \to \vgamma[prime] \) in~\( \catGamma \), and the two arrows are given by \( \mH { \vgamma , \vgamma } \xto { \mf[push] } \mH { \vgamma , \vgamma[prime] } \) resp.~\( \mH { \vgamma[prime] , \vgamma[prime] } \xto{ \mf[pull] } \mH { \vgamma , \vgamma[prime] } \).

The dual story is that of a coend: If again \( \mH \colon \catGamma[op] \times \catGamma \to \catC \) is a bifunctor, the \textdef{coend} is an object
\[
	\Coend[\catGamma] { \mH } = \Coend[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\(\catC \), together with morphisms~\(
	\mH { \vgamma , \vgamma } \to \Coend[\catGamma] { \mH }
\)
such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \), the upper left square of the following digram commutes:
\[\begin{tikzcd}
	\mH { \vgamma , \vgamma[prime] }
			& \mH { \vgamma , \vgamma } \ar[l, "\mH { \vgamma , \mf }"']
\\
	\mH { \vgamma[prime] , \vgamma[prime] } \ar[u, "\mH { \mf , \vgamma[prime] }"]
			& \Coend[\catGamma] { \mH } \ar[u] \ar[l]
\\[-1em]
	&	&[-2em] A \ar[ul,dashed] \ar[llu, bend left] \ar[luu, bend right]
\invdot
\end{tikzcd}\]
Furthermore, \( \Coend[\catGamma] { \mH } \) must be universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( \mH { \vgamma , \vgamma } \to A \) for all~\( \vgamma \), then these factor through a unique map~\( \Coend[\catGamma] { \mH } \to A \). If \( \catC \)~is cocomplete, then clearly
\[
	\Coend[\catGamma] { \mH }
	=
	\Coeq[par=\Big] {
		\Coprod[ \mf \colon \vgamma \to \vgamma[prime] ] { \mH { \vgamma , \vgamma[prime] } }
		\rightrightarrows
		\Coprod[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
	},
\]
the maps being defined as before.

\section{Weighted limits}




\section{Kan extensions}




\endgroup

==> category/category_2.tex <==
\begingroup

\chapter{Tools from general category theory}

We include here some notions and tools from general category theory which we shall make use of in the main body of the text.

\section{Ends and coends}

Let \( \catGamma \) and~\( \catC \) be categories and~\( \mH \colon \catGamma[op] \times \catGamma \to \catC \) a bifunctor. The \textdef{end} of~\( \mH \) is an object
\[
	\End[\catGamma] { \mH } = \End[\vgamma \in \catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\( \catC \), together with morphisms~\(
	%\mvarphi[\vgamma] \colon
	\End[\catGamma] { \mH }
	\to
	\mH { \vgamma , \vgamma }
\) for all~\( \vgamma \in \catGamma \), such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \) the lower right square of the following diagram commutes:
\[\begin{tikzcd}
	A \ar[rd,dashed] \ar[rrd, bend left] \ar[ddr, bend right]
\\[-1em]
	&[-2em]	\End[\catGamma] { \mH } \ar[r] \ar[d]
			& \mH { \vgamma , \vgamma } \ar[d, "\mH { \vgamma , \mf }"]
\\
	&	\mH { \vgamma[prime] , \vgamma[prime] } \ar[r, "\mH { \mf , \vgamma[prime] }"']
			& \mH { \vgamma , \vgamma[prime] }
			\invdot
\end{tikzcd}\]
Furthermore, \( \End[\catGamma] { \mH} \)~is universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( A \to \mH { \vgamma , \vgamma } \) for all~\( \vgamma \), subject to the same commutativity conditions, then these factor through a unique map~\( A\to \End[\catGamma] { \mH } \).
If \( \catC \)~is complete, then clearly
\begin{equation}\label{eq:Equalizer_formula_for_end}
	\End[\catGamma]{ H }
	=
	\Eq[par=\Big] {
		\Prod[ \vgamma \in \catGamma ] { \mH { \vgamma , \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{\mf \colon \vgamma \to \vgamma[prime] } ] { \mH { \vgamma , \vgamma[prime] } }
	}.
\end{equation}
Here, the second product runs over all morphisms~\( \mf \colon \vgamma \to \vgamma[prime] \) in~\( \catGamma \), and the two arrows are given by \( \mH { \vgamma , \vgamma } \xto { \mf[push] } \mH { \vgamma , \vgamma[prime] } \) resp.~\( \mH { \vgamma[prime] , \vgamma[prime] } \xto{ \mf[pull] } \mH { \vgamma , \vgamma[prime] } \).

\begin{example}
	Given functors~\( \mF , \mG \colon \catGamma \to \catGamma[prime] \), we obtain a bifunctor
	\[
		\mH = \Hom[ \catGamma[prime] ] { \mF { slot } , \mG { slot } }
		\colon
		\catGamma[op] \times \catGamma \to \catset,
	\]
	and the universal property shows that
	\[
		\End[\catGamma] { \mH }
		=
		\Hom[ \catfun { \catGamma , \catGamma[prime] } ] { \mF , \mG }
	\]
	is the set of natural transformations between \( \mF \) and~\( \mG \).
	%In particular, \( \End[\catGamma] { \Hom[\catGamma] } \)~is the set of natural transformations between the identity functor~\( \id[\catGamma] \) and itself.
	%In general, in understanding the concept of an end, it is useful to regard~\( \mH \) as an enrichment of~\( \catGamma \) over~\( \catC \) and the end as the natural transformations of
\end{example}

The dual story is that of a coend: If again \( \mH \colon \catGamma[op] \times \catGamma \to \catC \) is a bifunctor, the \textdef{coend} is an object
\[
	\Coend[\catGamma] { \mH } = \Coend[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\(\catC \), together with morphisms~\(
	\mH { \vgamma , \vgamma } \to \Coend[\catGamma] { \mH }
\)
such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \), the upper left square of the following digram commutes:
\[\begin{tikzcd}
	\mH { \vgamma , \vgamma[prime] }
			& \mH { \vgamma , \vgamma } \ar[l, "\mH { \vgamma , \mf }"']
\\
	\mH { \vgamma[prime] , \vgamma[prime] } \ar[u, "\mH { \mf , \vgamma[prime] }"]
			& \Coend[\catGamma] { \mH } \ar[u] \ar[l]
\\[-1em]
	&	&[-2em] A \ar[ul,dashed] \ar[llu, bend left] \ar[luu, bend right]
\invdot
\end{tikzcd}\]
Furthermore, \( \Coend[\catGamma] { \mH } \) must be universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( \mH { \vgamma , \vgamma } \to A \) for all~\( \vgamma \), then these factor through a unique map~\( \Coend[\catGamma] { \mH } \to A \). If \( \catC \)~is cocomplete, then clearly
\[
	\Coend[\catGamma] { \mH }
	=
	\Coeq[par=\Big] {
		\Coprod[ \mf \colon \vgamma \to \vgamma[prime] ] { \mH { \vgamma , \vgamma[prime] } }
		\rightrightarrows
		\Coprod[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
	},
\]
the maps being defined as before.

\section{Weighted limits}

Given a functor~\( \mF \colon \catGamma \to \catC \), we may regard~\( \mF \) as a bifunctor~\( \catGamma[op] \times \catGamma \to \catC \),
\( \tup{ \vgamma , \vgamma[prime] } \mapsto \mF { \vgamma[prime] } \), so the first argument is simply discarded. Then it is easy to see that the universal property of~\( \End[\catGamma] { \mF } \) reduces to that of the limit~\( \invlim[\catGamma] { \mF } \), and the equalizer formula~\eqref{eq:Equalizer_formula_for_end} reduces to the familiar formula
\[
	{\textstyle \invlim[\catGamma] { \mF } }
	=
	\Eq[par=\Big] {
		\Prod[\vgamma \in\catGamma] { \mF { \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{ \mf \colon \vgamma\to\vgamma[prime]} ] { \mF { \vgamma[prime] } }
	}.
\]



\section{Kan extensions}




\endgroup

==> category/category_3.tex <==
\begingroup

\chapter{Tools from general category theory}

We include here some notions and tools from general category theory which we shall make use of in the main body of the text.

\section{Ends and coends}

Let \( \catGamma \) and~\( \catC \) be categories and~\( \mH \colon \catGamma[op] \times \catGamma \to \catC \) a bifunctor. The \textdef{end} of~\( \mH \) is an object
\[
	\End[\catGamma] { \mH } = \End[\vgamma \in \catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\( \catC \), together with morphisms~\(
	%\mvarphi[\vgamma] \colon
	\End[\catGamma] { \mH }
	\to
	\mH { \vgamma , \vgamma }
\) for all~\( \vgamma \in \catGamma \), such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \) the lower right square of the following diagram commutes:
\[\begin{tikzcd}
	A \ar[rd,dashed] \ar[rrd, bend left] \ar[ddr, bend right]
\\[-1em]
	&[-2em]	\End[\catGamma] { \mH } \ar[r] \ar[d]
			& \mH { \vgamma , \vgamma } \ar[d, "\mH { \vgamma , \mf }"]
\\
	&	\mH { \vgamma[prime] , \vgamma[prime] } \ar[r, "\mH { \mf , \vgamma[prime] }"']
			& \mH { \vgamma , \vgamma[prime] }
			\invdot
\end{tikzcd}\]
Furthermore, \( \End[\catGamma] { \mH} \)~is universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( A \to \mH { \vgamma , \vgamma } \) for all~\( \vgamma \), subject to the same commutativity conditions, then these factor through a unique map~\( A\to \End[\catGamma] { \mH } \).
If \( \catC \)~is complete, then clearly
\begin{equation}\label{eq:Equalizer_formula_for_end}
	\End[\catGamma]{ H }
	=
	\Eq[par=\Big] {
		\Prod[ \vgamma \in \catGamma ] { \mH { \vgamma , \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{\mf \colon \vgamma \to \vgamma[prime] } ] { \mH { \vgamma , \vgamma[prime] } }
	}.
\end{equation}
Here, the second product runs over all morphisms~\( \mf \colon \vgamma \to \vgamma[prime] \) in~\( \catGamma \), and the two arrows are given by \( \mH { \vgamma , \vgamma } \xto { \mf[push] } \mH { \vgamma , \vgamma[prime] } \) resp.~\( \mH { \vgamma[prime] , \vgamma[prime] } \xto{ \mf[pull] } \mH { \vgamma , \vgamma[prime] } \).

\begin{example}
	Given functors~\( \mF , \mG \colon \catGamma \to \catGamma[prime] \), we obtain a bifunctor
	\[
		\mH = \Hom[ \catGamma[prime] ] { \mF { slot } , \mG { slot } }
		\colon
		\catGamma[op] \times \catGamma \to \catset,
	\]
	and the universal property shows that
	\[
		\End[\catGamma] { \mH }
		=
		\Hom[ \catfun { \catGamma , \catGamma[prime] } ] { \mF , \mG }
	\]
	is the set of natural transformations between \( \mF \) and~\( \mG \).
	%In particular, \( \End[\catGamma] { \Hom[\catGamma] } \)~is the set of natural transformations between the identity functor~\( \id[\catGamma] \) and itself.
	%In general, in understanding the concept of an end, it is useful to regard~\( \mH \) as an enrichment of~\( \catGamma \) over~\( \catC \) and the end as the natural transformations of
\end{example}

The dual story is that of a coend: If again \( \mH \colon \catGamma[op] \times \catGamma \to \catC \) is a bifunctor, the \textdef{coend} is an object
\[
	\Coend[\catGamma] { \mH } = \Coend[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\(\catC \), together with morphisms~\(
	\mH { \vgamma , \vgamma } \to \Coend[\catGamma] { \mH }
\)
such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \), the upper left square of the following digram commutes:
\[\begin{tikzcd}
	\mH { \vgamma , \vgamma[prime] }
			& \mH { \vgamma , \vgamma } \ar[l, "\mH { \vgamma , \mf }"']
\\
	\mH { \vgamma[prime] , \vgamma[prime] } \ar[u, "\mH { \mf , \vgamma[prime] }"]
			& \Coend[\catGamma] { \mH } \ar[u] \ar[l]
\\[-1em]
	&	&[-2em] A \ar[ul,dashed] \ar[llu, bend left] \ar[luu, bend right]
\invdot
\end{tikzcd}\]
Furthermore, \( \Coend[\catGamma] { \mH } \) must be universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( \mH { \vgamma , \vgamma } \to A \) for all~\( \vgamma \), then these factor through a unique map~\( \Coend[\catGamma] { \mH } \to A \). If \( \catC \)~is cocomplete, then clearly
\[
	\Coend[\catGamma] { \mH }
	=
	\Coeq[par=\Big] {
		\Coprod[ \mf \colon \vgamma \to \vgamma[prime] ] { \mH { \vgamma , \vgamma[prime] } }
		\rightrightarrows
		\Coprod[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
	},
\]
the maps being defined as before.

\section{Weighted limits}

Given a functor~\( \mF \colon \catGamma \to \catC \), we may regard~\( \mF \) as a bifunctor~\( \catGamma[op] \times \catGamma \to \catC \),
\( \tup{ \vgamma , \vgamma[prime] } \mapsto \mF { \vgamma[prime] } \), the first argument being simply discarded. Then it is easy to see that the universal property of~\( \End[\catGamma] { \mF } \) reduces to that of the limit~\( \invlim[\catGamma] { \mF } \), and the equalizer formula~\eqref{eq:Equalizer_formula_for_end} reduces to the familiar formula
\[
	{\textstyle \invlim[\catGamma] { \mF } }
	=
	\Eq[par=\Big] {
		\Prod[\vgamma \in\catGamma] { \mF { \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{ \mf \colon \vgamma\to\vgamma[prime]} ] { \mF { \vgamma[prime] } }
	}.
\]

Now suppose that \( \tup { \catV , \tens , \innerhom{ slot , slot } } \)~is a closed, symmetric, monoidal category.
Then one has the usual isomorphism
\[
	\innerhom { \vv[1] , \innerhom{\vv[2] , \vv[3] } }
	\cong
	\innerhom { \vv[2], \innerhom{ \vv[1] , \vv[3] } }
\]
for~\( \vv[1], \vv[2], \vv[3] \in \catV \). This provides a contravariant “action” of~\( \catV \) on itself that we wish to generalize.
A \textdef{powering} of~\( \catV \) on the category~\( \catC \) is a functor
\[
	\catV[op] \times\catC\longto\catC,
	\qquad
	\tup{ \vv, \vc } \longmapsto \vc[powering=\vv]
\]
satisfying
\[d
\]

(other notations include \( \powering { \vv , \vc } \) and~\( \innerhom { \vv , \vc } \)).

\section{Kan extensions}




\endgroup

==> category/category_4.tex <==
\begingroup

\chapter{Tools from general category theory}

We include here some notions and tools from general category theory which we shall make use of in the main body of the text.

\section{Ends and coends}

Let \( \catGamma \) and~\( \catC \) be categories and~\( \mH \colon \catGamma[op] \times \catGamma \to \catC \) a bifunctor. The \textdef{end} of~\( \mH \) is an object
\[
	\End[\catGamma] { \mH } = \End[\vgamma \in \catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\( \catC \), together with morphisms~\(
	%\mvarphi[\vgamma] \colon
	\End[\catGamma] { \mH }
	\to
	\mH { \vgamma , \vgamma }
\) for all~\( \vgamma \in \catGamma \), such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \) the lower right square of the following diagram commutes:
\begin{equation}\label{eq:end_universal_property}
\begin{tikzcd}
	A \ar[rd,dashed] \ar[rrd, bend left] \ar[ddr, bend right]
\\[-1em]
	&[-2em]	\End[\catGamma] { \mH } \ar[r] \ar[d]
			& \mH { \vgamma , \vgamma } \ar[d, "\mH { \vgamma , \mf }"]
\\
	&	\mH { \vgamma[prime] , \vgamma[prime] } \ar[r, "\mH { \mf , \vgamma[prime] }"']
			& \mH { \vgamma , \vgamma[prime] }
			\invdot
\end{tikzcd}
\end{equation}
Furthermore, \( \End[\catGamma] { \mH} \)~is universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( A \to \mH { \vgamma , \vgamma } \) for all~\( \vgamma \), subject to the same commutativity conditions, then these factor through a unique map~\( A\to \End[\catGamma] { \mH } \).
If \( \catC \)~is complete, then clearly
\begin{equation}\label{eq:Equalizer_formula_for_end}
	\End[\catGamma]{ H }
	=
	\Eq[par=\Big] {
		\Prod[ \vgamma \in \catGamma ] { \mH { \vgamma , \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{\mf \colon \vgamma \to \vgamma[prime] } ] { \mH { \vgamma , \vgamma[prime] } }
	}.
\end{equation}
Here, the second product runs over all morphisms~\( \mf \colon \vgamma \to \vgamma[prime] \) in~\( \catGamma \), and the two arrows are given by \( \mH { \vgamma , \vgamma } \xto { \mf[push] } \mH { \vgamma , \vgamma[prime] } \) resp.~\( \mH { \vgamma[prime] , \vgamma[prime] } \xto{ \mf[pull] } \mH { \vgamma , \vgamma[prime] } \).

\begin{example}
	Given functors~\( \mF , \mG \colon \catGamma \to \catGamma[prime] \), we obtain a bifunctor
	\[
		\mH = \Hom[ \catGamma[prime] ] { \mF { slot } , \mG { slot } }
		\colon
		\catGamma[op] \times \catGamma \to \catset,
	\]
	and the universal property shows that
	\[
		\End[\catGamma] { \mH }
		=
		\Hom[ \catfun { \catGamma , \catGamma[prime] } ] { \mF , \mG }
	\]
	is the set of natural transformations between \( \mF \) and~\( \mG \).
	%In particular, \( \End[\catGamma] { \Hom[\catGamma] } \)~is the set of natural transformations between the identity functor~\( \id[\catGamma] \) and itself.
	%In general, in understanding the concept of an end, it is useful to regard~\( \mH \) as an enrichment of~\( \catGamma \) over~\( \catC \) and the end as the natural transformations of
\end{example}

The dual story is that of a coend: If again \( \mH \colon \catGamma[op] \times \catGamma \to \catC \) is a bifunctor, the \textdef{coend} is an object
\[
	\Coend[\catGamma] { \mH } = \Coend[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\(\catC \), together with morphisms~\(
	\mH { \vgamma , \vgamma } \to \Coend[\catGamma] { \mH }
\)
such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \), the upper left square of the following digram commutes:
\[\begin{tikzcd}
	\mH { \vgamma , \vgamma[prime] }
			& \mH { \vgamma , \vgamma } \ar[l, "\mH { \vgamma , \mf }"']
\\
	\mH { \vgamma[prime] , \vgamma[prime] } \ar[u, "\mH { \mf , \vgamma[prime] }"]
			& \Coend[\catGamma] { \mH } \ar[u] \ar[l]
\\[-1em]
	&	&[-2em] A \ar[ul,dashed] \ar[llu, bend left] \ar[luu, bend right]
\invdot
\end{tikzcd}\]
Furthermore, \( \Coend[\catGamma] { \mH } \) must be universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( \mH { \vgamma , \vgamma } \to A \) for all~\( \vgamma \), then these factor through a unique map~\( \Coend[\catGamma] { \mH } \to A \). If \( \catC \)~is cocomplete, then clearly
\[
	\Coend[\catGamma] { \mH }
	=
	\Coeq[par=\Big] {
		\Coprod[ \mf \colon \vgamma \to \vgamma[prime] ] { \mH { \vgamma , \vgamma[prime] } }
		\rightrightarrows
		\Coprod[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
	},
\]
the maps being defined as before.

\section{Weighted limits}

A good reference for this section is \textcite{riehl}.
Given a functor~\( \mF \colon \catGamma \to \catC \), we may regard~\( \mF \) as a bifunctor~\( \catGamma[op] \times \catGamma \to \catC \),
\( \tup{ \vgamma , \vgamma[prime] } \mapsto \mF { \vgamma[prime] } \), the first argument being simply discarded. Then it is easy to see that the universal property of~\( \End[\catGamma] { \mF } \) reduces to that of the limit~\( \invlim[\catGamma] { \mF } \), and the equalizer formula~\eqref{eq:Equalizer_formula_for_end} reduces to the familiar formula
\[
	{\textstyle \invlim[\catGamma] { \mF } }
	=
	\Eq[par=\Big] {
		\Prod[\vgamma \in\catGamma] { \mF { \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{ \mf \colon \vgamma\to\vgamma[prime]} ] { \mF { \vgamma[prime] } }
	}.
\]

%\setupobject\innerhom{outputoptions={\catV}}

Now suppose that \( \tup { \catV , \tens , \innerhom{ slot , slot } , \finalobject } \)~is a unital\fxfatal{Here, unital involves \( \innerhom { \catunit , slot } = \id \); don't know if that's standard. Also, the notation is usually for final object}, closed, symmetric, monoidal category.
Then one has the usual isomorphisms
\[
	\innerhom { \vv[1] , \innerhom{\vv[2] , \vv[3] } }
	\cong
	\innerhom { \vv[2], \innerhom{ \vv[1] , \vv[3] } }
	\qquad\text{and}\qquad
	\innerhom{ \vv[1] \tens \vv[2] , \vv[3] }
	\cong
	\innerhom{ \vv[2] , \innerhom { \vv[1] , \vv[3] } }
\]
for~\( \vv[1], \vv[2], \vv[3] \in \catV \). This provides a covariant as well as a contravariant “action” of~\( \catV \) on itself that we wish to generalize.

Let~\( \catC \) be a category enriched\fxfatal{Be clear somewhere that an enriched category, in our setup, has an underlying category.} over~\( \catV \), and denote the enriched hom space by~\( \Hom[enrich,smash] \). Then a \textdef{powering} of~\( \catV \) on the category~\( \catC \) is a bifunctor
\[
	\catV[op] \times\catC\longto\catC,
	\qquad
	\tup{ \vv, \vx } \longmapsto \vc[powering=\vv]
\]
satisfying
\[
	\Hom[enrich,\catC] { \vy , { \vx[powering=\vv] } }
	\cong
	\innerhom { \vv , \Hom[enrich,\catC] { \vy , \vx } }
\]
for all~\( \vv \in \catV \) and \( \vx , \vy \in \catC \).
(other notations include \( \powering { \vv , \vx } \) and~\( \innerhom { \vv , \vx } \)). Notice that \( \vx[powering=\catunit] = \vx \).
Dually, a \textdef{copowering} of~\( \catV \) on~\( \catC \) is a bifunctor
\[
	\catV \times \catC \longto \catC,
	\qquad
	\tup { \vv , \vx } \longmapsto \vv \tens \vx.
\]
satisfying
\[
	\Hom[enrich,\catC] { \vv \tens \vx , \vy }
	\cong
	\innerhom { \vv , \Hom[enrich,\catC] { \vx , \vy } }
\]
for all~\( \vv \in \catV \) and \( \vx , \vy \in \catC \). Notice that \( \catunit \tens \vx = \vx \).
By the identities above, the inner hom and the tensor product provide a powering resp.\ copowering of~\( \catV \) on itself.

Now\fxfatal{Wait, wait a moment, I have not introduced enriched ends and coends! But then again, the limit should make sense in the classical sense, so I guess really no issues?}
in the above setup, let~\( \catGamma \) be a category and
\(	\mW \colon \catGamma \to \catV \)
a functor. The \textdef{weighted limit} with weight~\( \mW \) of a diagram~\( \mF \colon \catGamma \to \catC \) is given by the end
\[
	\invlim[weight=\mW] { \mF } = \End [ \vgamma\in\catGamma ] { {\mF{\vgamma}[powering=\mW{\vgamma}] } }
\]
By taking~\( \mW \) to be the constant functor at~\( \finalobject \), we obtain \( \invlim[weight=\finalobject] = \invlim \).
Dually, if instead \( \mW \colon \catGamma[op] \to \catV \) is a functor, then
the \textdef{weighted colimit} with weight~\( \mW \) of the diagram~\( \mF \colon \catGamma \to \catC \) is given by the coend
\[
	\dirlim[weight=\mW] { \mF }
	=
	\Coend[\vgamma\in\catGamma] { \mW { \vgamma} \tens \mF { \vgamma } }.
\]
As before, we recover the colimit by~\( \dirlim[weight=\finalobject] = \dirlim \).

\section{Kan extensions}




\endgroup

==> category/category_5.tex <==
\begingroup

\chapter{Tools from general category theory}

We include here some notions and tools from general category theory which we shall make use of in the main body of the text.

\section{Ends and coends}

Let \( \catGamma \) and~\( \catC \) be categories and~\( \mH \colon \catGamma[op] \times \catGamma \to \catC \) a bifunctor. The \textdef{end} of~\( \mH \) is an object
\[
	\End[\catGamma] { \mH } = \End[\vgamma \in \catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\( \catC \), together with morphisms~\(
	%\mvarphi[\vgamma] \colon
	\End[\catGamma] { \mH }
	\to
	\mH { \vgamma , \vgamma }
\) for all~\( \vgamma \in \catGamma \), such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \) the lower right square of the following diagram commutes:
\begin{equation*}%\label{eq:end_universal_property}
\begin{tikzcd}
	A \ar[rd,dashed] \ar[rrd, bend left] \ar[ddr, bend right]
\\[-1em]
	&[-2em]	\End[\catGamma] { \mH } \ar[r] \ar[d]
			& \mH { \vgamma , \vgamma } \ar[d, "\mH { \vgamma , \mf }"]
\\
	&	\mH { \vgamma[prime] , \vgamma[prime] } \ar[r, "\mH { \mf , \vgamma[prime] }"']
			& \mH { \vgamma , \vgamma[prime] }
			\invdot
\end{tikzcd}
\end{equation*}
Furthermore, \( \End[\catGamma] { \mH} \)~is universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( A \to \mH { \vgamma , \vgamma } \) for all~\( \vgamma \), subject to the same commutativity conditions, then these factor through a unique map~\( A\to \End[\catGamma] { \mH } \).
If \( \catC \)~is complete, then clearly
\begin{equation}\label{eq:Equalizer_formula_for_end}
	\End[\catGamma]{ H }
	=
	\Eq[par=\Big] {
		\Prod[ \vgamma \in \catGamma ] { \mH { \vgamma , \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{\mf \colon \vgamma \to \vgamma[prime] } ] { \mH { \vgamma , \vgamma[prime] } }
	}.
\end{equation}
Here, the second product runs over all morphisms~\( \mf \colon \vgamma \to \vgamma[prime] \) in~\( \catGamma \), and the two arrows are given by \( \mH { \vgamma , \vgamma } \xto { \mf[push] } \mH { \vgamma , \vgamma[prime] } \) resp.~\( \mH { \vgamma[prime] , \vgamma[prime] } \xto{ \mf[pull] } \mH { \vgamma , \vgamma[prime] } \).

\begin{example}
	Given functors~\( \mF , \mG \colon \catGamma \to \catGamma[prime] \), we obtain a bifunctor
	\[
		\mH = \Hom[ \catGamma[prime] ] { \mF { slot } , \mG { slot } }
		\colon
		\catGamma[op] \times \catGamma \to \catset,
	\]
	and the universal property shows that
	\[
		\End[\catGamma] { \mH }
		=
		\Hom[ \catfun { \catGamma , \catGamma[prime] } ] { \mF , \mG }
	\]
	is the set of natural transformations between \( \mF \) and~\( \mG \).
	%In particular, \( \End[\catGamma] { \Hom[\catGamma] } \)~is the set of natural transformations between the identity functor~\( \id[\catGamma] \) and itself.
	%In general, in understanding the concept of an end, it is useful to regard~\( \mH \) as an enrichment of~\( \catGamma \) over~\( \catC \) and the end as the natural transformations of
\end{example}

The end is clearly a limit, hence a right adjoint. This adjunction can be spelled out:
\begin{proposition}\label{res:end_adjunction}
	Suppose \( \catC \)~is cocomplete.
	The end fits as the right adjoint of the adjunction
	\[\begin{tikzcd}
		%\catGamma { slot , slot } \times { }
		\Hom[\catGamma] \times\slot
		\colon
		\catC \ar[r, yshift=1pt]
			& \catC[diag=\catGamma[op]\times\catGamma]
			\ar[l,yshift=-1pt]
			\noloc
			\End[\catGamma]\invdot
	\end{tikzcd}\]
	The left adjoint takes~\( \vA \in \catC \) to the bifunctor
	\( \Hom[\catGamma] { slot , slot } \times \vA \colon \catGamma[op]\times\catGamma\to\catC \).
	Here \( \times \)~denotes the canonical copowering by~\( \catset \) on the cocomplete category~\( \catC \).
\end{proposition}

\begin{proof}
	Clear from the definition.
\end{proof}

This is equivalent to the statement that we have an adjunction
\[
	\catset[diag=\catGamma[op]\times\catGamma,par=\big] {
		\Hom[\catGamma] ,
		\catC { \vA , \mF }
	}
	\cong
	\catC[diag=\catGamma[op]\times\catGamma,par=\big] {
		\vA , \textstyle \End[\catGamma] { \mF }
	}
\]
for \( \vA \in \catC \). This says that the end is the weighted limit
\( \End[\catGamma] = \invlim[weight=\Hom[\catGamma],\catGamma[op]\times\catGamma] \)
with weight~\( \Hom[\catGamma] \).


The dual story is that of a coend: If again \( \mH \colon \catGamma[op] \times \catGamma \to \catC \) is a bifunctor, the \textdef{coend} is an object
\[
	\Coend[\catGamma] { \mH } = \Coend[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\(\catC \), together with morphisms~\(
	\mH { \vgamma , \vgamma } \to \Coend[\catGamma] { \mH }
\)
such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \), the upper left square of the following digram commutes:
\[\begin{tikzcd}
	\mH { \vgamma , \vgamma[prime] }
			& \mH { \vgamma , \vgamma } \ar[l, "\mH { \vgamma , \mf }"']
\\
	\mH { \vgamma[prime] , \vgamma[prime] } \ar[u, "\mH { \mf , \vgamma[prime] }"]
			& \Coend[\catGamma] { \mH } \ar[u] \ar[l]
\\[-1em]
	&	&[-2em] A \ar[ul,dashed] \ar[llu, bend left] \ar[luu, bend right]
\invdot
\end{tikzcd}\]
Furthermore, \( \Coend[\catGamma] { \mH } \) must be universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( \mH { \vgamma , \vgamma } \to A \) for all~\( \vgamma \), then these factor through a unique map~\( \Coend[\catGamma] { \mH }[smash] \to A \). If \( \catC \)~is cocomplete, then clearly
\[
	\Coend[\catGamma] { \mH }
	=
	\Coeq[par=\Big] {
		\Coprod[ \mf \colon \vgamma \to \vgamma[prime] ] { \mH { \vgamma , \vgamma[prime] } }
		\rightrightarrows
		\Coprod[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
	},
\]
the maps being defined as before.

The coend is clearly a colimit, hence a left adjoint. This adjunction can be spelled out:

\begin{proposition}
	Suppose \( \catC \)~is complete. The coend fits as the right adjoint of the adjunction
	\[\begin{tikzcd}
		\Coend[\catGamma]
		\colon
		\catC[diag=\catGamma[op]\times\catGamma]
		\ar[r,yshift=1pt]
			& \catC \ar[l,yshift=-1pt]
			\noloc
			\alg{\slot}[powering=\Hom[\catGamma]]
	\end{tikzcd}\]
	The right adjoint takes~\( \vA \in\catC \) to the bifunctor
	\(
		\catA[ powering=\Hom[\catGamma]{ slot , slot } ]
		\colon
		\catGamma[op]\times\catGamma\to\catC
	\).
	Here \( \alg{\slot}[powering=\slot] \)~denotes the canonical powering by~\( \catset \) on the complete category~\( \catC \).\fxfatal{Think about changing the notation to~\( \catGamma\times\catGamma[op] \).}
\end{proposition}

This is equivalent to the statement that we have an adjunction
\[
	\catset[diag=\catGamma[op]\times\catGamma,par=\big] {
		\catC { \vA , \mF } ,
		\Hom[\catGamma]
	}
	\cong
	\catC[diag=\catGamma[op]\times\catGamma,par=\big] {
		\textstyle \Coend[\catGamma] { \mF } , \vA
	}
\]
for \( \vA \in \catC \). This says that the end is the weighted colimit
\( \Coend[\catGamma] = \dirlim[weight=\Hom[\catGamma],\catGamma[op]\times\catGamma] \)
with weight~\( \Hom[\catGamma] \).

\section{Weighted limits}

A good reference for this section is \textcite{riehl}.
Given a functor~\( \mF \colon \catGamma \to \catC \), we may regard~\( \mF \) as a bifunctor~\( \catGamma[op] \times \catGamma \to \catC \),
\( \tup{ \vgamma , \vgamma[prime] } \mapsto \mF { \vgamma[prime] } \), the first argument being simply discarded. Then it is easy to see that the universal property of~\( \End[\catGamma] { \mF } \) reduces to that of the limit~\( \invlim[\catGamma] { \mF } \), and the equalizer formula~\eqref{eq:Equalizer_formula_for_end} reduces to the familiar formula
\[
	{\textstyle \invlim[\catGamma] { \mF } }
	=
	\Eq[par=\Big] {
		\Prod[\vgamma \in\catGamma] { \mF { \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{ \mf \colon \vgamma\to\vgamma[prime]} ] { \mF { \vgamma[prime] } }
	}.
\]

%\setupobject\innerhom{outputoptions={\catV}}

Now suppose that \( \tup { \catV , \tens , \innerhom{ slot , slot } , \finalobject } \)~is a unital\fxfatal{Here, unital involves \( \innerhom { \catunit , slot } = \id \); don't know if that's standard. Also, the notation is usually for final object}, closed, symmetric, monoidal category.
Then one has the usual isomorphisms
\[
	\innerhom { \vv[1] , \innerhom{\vv[2] , \vv[3] } }
	\cong
	\innerhom { \vv[2], \innerhom{ \vv[1] , \vv[3] } }
	\qquad\text{and}\qquad
	\innerhom{ \vv[1] \tens \vv[2] , \vv[3] }
	\cong
	\innerhom{ \vv[2] , \innerhom { \vv[1] , \vv[3] } }
\]
for~\( \vv[1], \vv[2], \vv[3] \in \catV \). This provides a covariant as well as a contravariant “action” of~\( \catV \) on itself that we wish to generalize.

Let~\( \catC \) be a category enriched\fxfatal{Be clear somewhere that an enriched category, in our setup, has an underlying category.} over~\( \catV \), and denote the enriched hom space by~\( \Hom[enrich,smash] \). Then a \textdef{powering} of~\( \catV \) on the category~\( \catC \) is a bifunctor
\[
	\catV[op] \times\catC\longto\catC,
	\qquad
	\tup{ \vv, \vx } \longmapsto \vc[powering=\vv]
\]
satisfying
\[
	\Hom[enrich,\catC] { \vy , { \vx[powering=\vv] } }
	\cong
	\innerhom { \vv , \Hom[enrich,\catC] { \vy , \vx } }
\]
for all~\( \vv \in \catV \) and \( \vx , \vy \in \catC \).
(other notations include \( \powering { \vv , \vx } \) and~\( \innerhom { \vv , \vx } \)). Notice that \( \vx[powering=\catunit] = \vx \).
Dually, a \textdef{copowering} of~\( \catV \) on~\( \catC \) is a bifunctor
\[
	\catV \times \catC \longto \catC,
	\qquad
	\tup { \vv , \vx } \longmapsto \vv \tens \vx.
\]
satisfying
\[
	\Hom[enrich,\catC] { \vv \tens \vx , \vy }
	\cong
	\innerhom { \vv , \Hom[enrich,\catC] { \vx , \vy } }
\]
for all~\( \vv \in \catV \) and \( \vx , \vy \in \catC \). Notice that \( \catunit \tens \vx = \vx \).
By the identities above, the inner hom and the tensor product provide a powering resp.\ copowering of~\( \catV \) on itself.

Now\fxfatal{Wait, wait a moment, I have not introduced enriched ends and coends! But then again, the limit should make sense in the classical sense, so I guess really no issues?}
in the above setup, let~\( \catGamma \) be a category and
\(	\mW \colon \catGamma \to \catV \)
a functor. The \textdef{weighted limit} with weight~\( \mW \) of a diagram~\( \mF \colon \catGamma \to \catC \) is given by the end
\[
	\invlim[weight=\mW] { \mF } = \End [ \vgamma\in\catGamma ] { {\mF{\vgamma}[powering=\mW{\vgamma}] } }
\]
By taking~\( \mW \) to be the constant functor at~\( \finalobject \), we obtain \( \invlim[weight=\finalobject] = \invlim \).
Dually, if instead \( \mW \colon \catGamma[op] \to \catV \) is a functor, then
the \textdef{weighted colimit} with weight~\( \mW \) of the diagram~\( \mF \colon \catGamma \to \catC \) is given by the coend
\[
	\dirlim[weight=\mW] { \mF }
	=
	\Coend[\vgamma\in\catGamma] { \mW { \vgamma} \tens \mF { \vgamma } }.
\]
As before, we recover the colimit by~\( \dirlim[weight=\finalobject] = \dirlim \).

\section{Kan extensions}




\endgroup

==> category/category_6.tex <==
\begingroup

\chapter{Tools from general category theory}

We include here some notions and tools from general category theory which we shall make use of in the main body of the text.

\section{Ends and coends}

Let \( \catGamma \) and~\( \catC \) be categories and~\( \mH \colon \catGamma[op] \times \catGamma \to \catC \) a bifunctor. The \textdef{end} of~\( \mH \) is an object
\[
	\End[\catGamma] { \mH } = \End[\vgamma \in \catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\( \catC \), together with morphisms~\(
	%\mvarphi[\vgamma] \colon
	\End[\catGamma] { \mH }
	\to
	\mH { \vgamma , \vgamma }
\) for all~\( \vgamma \in \catGamma \), such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \) the lower right square of the following diagram commutes:
\begin{equation*}%\label{eq:end_universal_property}
\begin{tikzcd}
	A \ar[rd,dashed] \ar[rrd, bend left] \ar[ddr, bend right]
\\[-1em]
	&[-2em]	\End[\catGamma] { \mH } \ar[r] \ar[d]
			& \mH { \vgamma , \vgamma } \ar[d, "\mH { \vgamma , \mf }"]
\\
	&	\mH { \vgamma[prime] , \vgamma[prime] } \ar[r, "\mH { \mf , \vgamma[prime] }"']
			& \mH { \vgamma , \vgamma[prime] }
			\invdot
\end{tikzcd}
\end{equation*}
Furthermore, \( \End[\catGamma] { \mH} \)~is universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( A \to \mH { \vgamma , \vgamma } \) for all~\( \vgamma \), subject to the same commutativity conditions, then these factor through a unique map~\( A\to \End[\catGamma] { \mH } \).
If \( \catC \)~is complete, then clearly
\begin{equation}\label{eq:Equalizer_formula_for_end}
	\End[\catGamma]{ H }
	=
	\Eq[par=\Big] {
		\Prod[ \vgamma \in \catGamma ] { \mH { \vgamma , \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{\mf \colon \vgamma \to \vgamma[prime] } ] { \mH { \vgamma , \vgamma[prime] } }
	}.
\end{equation}
Here, the second product runs over all morphisms~\( \mf \colon \vgamma \to \vgamma[prime] \) in~\( \catGamma \), and the two arrows are given by \( \mH { \vgamma , \vgamma } \xto { \mf[push] } \mH { \vgamma , \vgamma[prime] } \) resp.~\( \mH { \vgamma[prime] , \vgamma[prime] } \xto{ \mf[pull] } \mH { \vgamma , \vgamma[prime] } \).

\begin{example}
	Given functors~\( \mF , \mG \colon \catGamma \to \catGamma[prime] \), we obtain a bifunctor
	\[
		\mH = \Hom[ \catGamma[prime] ] { \mF { slot } , \mG { slot } }
		\colon
		\catGamma[op] \times \catGamma \to \catset,
	\]
	and the universal property shows that
	\[
		\End[\catGamma] { \mH }
		=
		\Hom[ \catfun { \catGamma , \catGamma[prime] } ] { \mF , \mG }
	\]
	is the set of natural transformations between \( \mF \) and~\( \mG \).
	%In particular, \( \End[\catGamma] { \Hom[\catGamma] } \)~is the set of natural transformations between the identity functor~\( \id[\catGamma] \) and itself.
	%In general, in understanding the concept of an end, it is useful to regard~\( \mH \) as an enrichment of~\( \catGamma \) over~\( \catC \) and the end as the natural transformations of
\end{example}

%The end is clearly a limit, hence a right adjoint. This adjunction can be spelled out:
\begin{proposition}\label{res:end_adjunction}
	Suppose \( \catC \)~is cocomplete.
	The end fits as the right adjoint of the adjunction
	\[\begin{tikzcd}
		%\catGamma { slot , slot } \times { }
		%\Hom[\catGamma] \times\slot
		%\Coprod[ \catGamma { slot , slot } ]
		\Coprod[ \Hom[\catGamma] ]
		\colon
		\catC \ar[r, yshift=1pt]
			& \catC[diag=\catGamma[op]\times\catGamma]
			\ar[l,yshift=-1pt]
			\noloc
			\End[\catGamma]\invdot
	\end{tikzcd}\]
	The left adjoint takes~\( \vA \in \catC \) to the bifunctor
	\( \Coprod[ \Hom[\catGamma] { slot , slot } ] { \vA } \colon \catGamma[op]\times\catGamma\to\catC \).
	%Here \( \times \)~denotes the canonical copowering by~\( \catset \) on the cocomplete category~\( \catC \).
\end{proposition}

\begin{proof}
	Clear from the definition.
\end{proof}

This is equivalent to the statement that we have an adjunction
\[
	\catset[diag=\catGamma[op]\times\catGamma,par=\big] {
		\Hom[\catGamma] ,
		\catC { \vA , \mF }
	}
	\cong
	\catC[diag=\catGamma[op]\times\catGamma,par=\big] {
		\vA , \textstyle \End[\catGamma] { \mF }
	}
\]
for \( \vA \in \catC \). This says that the end is the weighted limit
\( \End[\catGamma] = \invlim[weight=\Hom[\catGamma],\catGamma[op]\times\catGamma] \)
with weight~\( \Hom[\catGamma] \).



The dual story is that of a coend: If again \( \mH \colon \catGamma[op] \times \catGamma \to \catC \) is a bifunctor, the \textdef{coend} is an object
\[
	\Coend[\catGamma] { \mH } = \Coend[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
\]
in~\(\catC \), together with morphisms~\(
	\mH { \vgamma , \vgamma } \to \Coend[\catGamma] { \mH }
\)
such that for any~\( \mf \colon \vgamma \to \vgamma[prime] \), the upper left square of the following digram commutes:
\[\begin{tikzcd}
	\mH { \vgamma , \vgamma[prime] }
			& \mH { \vgamma , \vgamma } \ar[l, "\mH { \vgamma , \mf }"']
\\
	\mH { \vgamma[prime] , \vgamma[prime] } \ar[u, "\mH { \mf , \vgamma[prime] }"]
			& \Coend[\catGamma] { \mH } \ar[u] \ar[l]
\\[-1em]
	&	&[-2em] A \ar[ul,dashed] \ar[llu, bend left] \ar[luu, bend right]
\invdot
\end{tikzcd}\]
Furthermore, \( \Coend[\catGamma] { \mH } \) must be universal with this property, meaning that if \( A \)~is another object of~\( \catC \) with a collection of arrows~\( \mH { \vgamma , \vgamma } \to A \) for all~\( \vgamma \), then these factor through a unique map~\( \Coend[\catGamma] { \mH }[smash] \to A \). If \( \catC \)~is cocomplete, then clearly
\[
	\Coend[\catGamma] { \mH }
	=
	\Coeq[par=\Big] {
		\Coprod[ \mf \colon \vgamma \to \vgamma[prime] ] { \mH { \vgamma , \vgamma[prime] } }
		\rightrightarrows
		\Coprod[\vgamma\in\catGamma] { \mH { \vgamma , \vgamma } }
	},
\]
the maps being defined as before.

The coend is clearly a colimit, hence a left adjoint. This adjunction can be spelled out:

\begin{proposition}
	Suppose \( \catC \)~is complete. The coend fits as the right adjoint of the adjunction
	\[\begin{tikzcd}
		\Coend[\catGamma]
		\colon
		\catC[diag=\catGamma[op]\times\catGamma]
		\ar[r,yshift=1pt]
			& \catC \ar[l,yshift=-1pt]
			\noloc
			%\alg{\slot}[powering=\Hom[\catGamma]]
			\Prod[ \Hom[\catGamma] ]
	\end{tikzcd}\]
	The right adjoint takes~\( \vA \in\catC \) to the bifunctor
	\(
		%\catA[ powering=\Hom[\catGamma]{ slot , slot } ]
		\Prod[ \Hom[\catGamma] { slot , slot } ] { \vA }
		\colon
		\catGamma[op]\times\catGamma\to\catC
	\).
	%Here \( \alg{\slot}[powering=\slot] \)~denotes the canonical powering by~\( \catset \) on the complete category~\( \catC \).\fxfatal{Think about changing the notation to~\( \catGamma\times\catGamma[op] \).}
\end{proposition}

This is equivalent to the statement that we have an adjunction
\[
	\catset[diag=\catGamma[op]\times\catGamma,par=\big] {
		\catC { \vA , \mF } ,
		\Hom[\catGamma]
	}
	\cong
	\catC[diag=\catGamma[op]\times\catGamma,par=\big] {
		\textstyle \Coend[\catGamma] { \mF } , \vA
	}
\]
for \( \vA \in \catC \). This says that the end is the weighted colimit
\( \Coend[\catGamma] = \dirlim[weight=\Hom[\catGamma],\catGamma[op]\times\catGamma] \)
with weight~\( \Hom[\catGamma] \).

\section{Weighted limits}

A good reference for this section is \textcite{riehl}.
Given a functor~\( \mF \colon \catGamma \to \catC \), we may regard~\( \mF \) as a bifunctor~\( \catGamma[op] \times \catGamma \to \catC \),
\( \tup{ \vgamma , \vgamma[prime] } \mapsto \mF { \vgamma[prime] } \), the first argument being simply discarded. Then it is easy to see that the universal property of~\( \End[\catGamma] { \mF } \) reduces to that of the limit~\( \invlim[\catGamma] { \mF } \), and the equalizer formula~\eqref{eq:Equalizer_formula_for_end} reduces to the familiar formula
\[
	{\textstyle \invlim[\catGamma] { \mF } }
	=
	\Eq[par=\Big] {
		\Prod[\vgamma \in\catGamma] { \mF { \vgamma } }
		\rightrightarrows
		\Prod[ \mathclap{ \mf \colon \vgamma\to\vgamma[prime]} ] { \mF { \vgamma[prime] } }
	}.
\]

%\setupobject\innerhom{outputoptions={\catV}}

Now suppose that \( \tup { \catV , \tens , \innerhom{ slot , slot } , \finalobject } \)~is a unital\fxfatal{Here, unital involves \( \innerhom { \catunit , slot } = \id \); don't know if that's standard. Also, the notation is usually for final object}, closed, symmetric, monoidal category.
Then one has the usual isomorphisms
\[
	\innerhom { \vv[1] , \innerhom{\vv[2] , \vv[3] } }
	\cong
	\innerhom { \vv[2], \innerhom{ \vv[1] , \vv[3] } }
	\qquad\text{and}\qquad
	\innerhom{ \vv[1] \tens \vv[2] , \vv[3] }
	\cong
	\innerhom{ \vv[2] , \innerhom { \vv[1] , \vv[3] } }
\]
for~\( \vv[1], \vv[2], \vv[3] \in \catV \). This provides a covariant as well as a contravariant “action” of~\( \catV \) on itself that we wish to generalize.

Let~\( \catC \) be a category enriched\fxfatal{Be clear somewhere that an enriched category, in our setup, has an underlying category.} over~\( \catV \), and denote the enriched hom space by~\( \Hom[enrich,smash] \). Then a \textdef{powering} of~\( \catV \) on the category~\( \catC \) is a bifunctor
\[
	\catV[op] \times\catC\longto\catC,
	\qquad
	\tup{ \vv, \vx } \longmapsto \vc[powering=\vv]
\]
satisfying
\[
	\Hom[enrich,\catC] { \vy , { \vx[powering=\vv] } }
	\cong
	\innerhom { \vv , \Hom[enrich,\catC] { \vy , \vx } }
\]
for all~\( \vv \in \catV \) and \( \vx , \vy \in \catC \).
(other notations include \( \powering { \vv , \vx } \) and~\( \innerhom { \vv , \vx } \)). Notice that \( \vx[powering=\catunit] = \vx \).
Dually, a \textdef{copowering} of~\( \catV \) on~\( \catC \) is a bifunctor
\[
	\catV \times \catC \longto \catC,
	\qquad
	\tup { \vv , \vx } \longmapsto \vv \tens \vx.
\]
satisfying
\[
	\Hom[enrich,\catC] { \vv \tens \vx , \vy }
	\cong
	\innerhom { \vv , \Hom[enrich,\catC] { \vx , \vy } }
\]
for all~\( \vv \in \catV \) and \( \vx , \vy \in \catC \). Notice that \( \catunit \tens \vx = \vx \).
By the identities above, the inner hom and the tensor product provide a powering resp.\ copowering of~\( \catV \) on itself.

Now\fxfatal{Wait, wait a moment, I have not introduced enriched ends and coends! But then again, the limit should make sense in the classical sense, so I guess really no issues?}
in the above setup, let~\( \catGamma \) be a category and
\(	\mW \colon \catGamma \to \catV \)
a functor. The \textdef{weighted limit} with weight~\( \mW \) of a diagram~\( \mF \colon \catGamma \to \catC \) is given by the end
\[
	\invlim[weight=\mW] { \mF } = \End [ \vgamma\in\catGamma ] { {\mF{\vgamma}[powering=\mW{\vgamma}] } }
\]
By taking~\( \mW \) to be the constant functor at~\( \finalobject \), we obtain \( \invlim[weight=\finalobject] = \invlim \).
Dually, if instead \( \mW \colon \catGamma[op] \to \catV \) is a functor, then
the \textdef{weighted colimit} with weight~\( \mW \) of the diagram~\( \mF \colon \catGamma \to \catC \) is given by the coend
\[
	\dirlim[weight=\mW] { \mF }
	=
	\Coend[\vgamma\in\catGamma] { \mW { \vgamma} \tens \mF { \vgamma } }.
\]
As before, we recover the colimit by~\( \dirlim[weight=\finalobject] = \dirlim \).

\section{Kan extensions}




\endgroup
